Automatic Detection of Fake Key Attacks in Secure Messaging

Popular instant messaging applications such as WhatsApp and Signal provide end-to-end encryption for billions of users. They rely on a centralized, application-specific server to distribute public keys and relay encrypted messages between the users. Therefore, they prevent passive attacks but are vulnerable to some active attacks. A malicious or hacked server can distribute fake keys to users to perform man-in-the-middle or impersonation attacks. While typical secure messaging applications provide a manual method for users to detect these attacks, this burdens users, and studies show it is ineffective in practice. This paper presents KTACA, a completely automated approach for key verification that is oblivious to users and easy to deploy. We motivate KTACA by designing two approaches to automatic key verification. One approach uses client auditing (KTCA) and the second uses anonymous key monitoring (AKM). Both have relatively inferior security properties, leading to KTACA, which combines these approaches to provide the best of both worlds. We provide a security analysis of each defense, identifying which attacks they can automatically detect. We implement the active attacks to demonstrate they are possible, and we also create a prototype implementation of all the defenses to measure their performance and confirm their feasibility. Finally, we discuss the strengths and weaknesses of each defense, the overhead on clients and service providers, and deployment considerations.

==> Defense_KT_old.tex <==


%%%%%%%%%%%%%%
%%%%%%%%%%%%%% OLD Section (read-only)
%%%%%%%%%%%%%%
\section{Key Transparency Defense - OLD}

\ks{Kent: I think we can start by first describing what key transparency is for the reader that doesn't have the background. Next we can say why we explore CONIKS and what is new. In CONIKS paper describes a vision where all the secure message providers each maintain a public ledger of their user's keys, user's can communicate with each other within and across providers, and the non-colluding providers audit each other. User's can contact the auditors out of band to detect any equivocation. This is not the model of today's secure messaging providers that currently do not inter-operate. In this section, we consider a slight adaptation of CONIKS to the case of a single identity provider, with the users acting ads auditors. We also assume no out-of-band channel between the user's, so the auditing messages flow through the server that can potentially launch a MITM attack. Assume the server has not compromised the system from the beginning. We begin with a set (size = 1?  k?  a connected graph? well-connected and reasonable diameter) of trusted friends - we have their correct keys. Assume server cannot prevent us from communicating (see our earlier heuristic).  Explain why we need this assumption. We assume synchronized time?}

% While Anonymous Key Retrieval is able to prevent most attacks, it does impose a cost of using Tor in secure messaging clients. We thus explore a different approach based on Key Transparency (KT), an existing approach to defend against fake key attacks. Although Key Transparency is only designed to provide detection of attacks, detection alone is a strong incentive for key servers to behave well and a disincentive for attackers if the detection time is short.




Key Transparency informs users about every public key ever associated with the user's account, preventing the server from distributing a fake public key for a user without detection. 
\st{Although Key Transparency is designed only to detect attacks, detection alone is a strong incentive for key servers to behave well and a disincentive for attackers if the detection time is short.} KT is somewhat analogous to Certificate Transparency (CT) \cite{scheitle2018rise}, an approach for detecting fake  certificates. 


%CT requires web browsers to validate that all website certificates are present in an append-only ledger. 
%If a rogue or hacked Certificate Authority issues a fake certificate and does \textit{not} list the certificate in the ledger, browsers will reject it. 
%If the attacker instead lists the certificate in the ledger, a browser may accept it, but the owner of the domain can detect the malfeasance and seek to have the certificate revoked.

\tarun{
In this section, We describe how to utilize the CONIKS Key Transparency system~\cite{melara2015coniks} to detect fake key attacks in secure messaging. We first explains the use of CONIKS system with multiple auditors scenario and then adapt it for one auditor scenario, where clients act as auditors. The latter is a more realistic scenario and can be deployed today by these messaging applications without waiting for dedicated non-colluding auditors. At the end we present security analysis of these.}
Other KT systems, such as Google Key Transparency [citation?], can similarly detect these attacks.
\ahc{CONIKS was also proposed for authenticating user keys; so what is the delta here? I think a big problem for CONIKS is its reliance on unique names, but I don't see here (or in system model) any discussion of naming. And if we agree that this reliance on unique, known names is problematic, I think we should look for solution much closer to CT than to CONIKS, no? Another problem imho with CONIKS is their assumption that users communicate each epoch, this seems easily avoidable. 
Also in system model we don't discuss having multiple servers and definitely not having any extra entities whose role is to ensure security such as for monitoring/auditing. Ah btw, one reference to CT is RFC6962. 
}
\tarun{Tarun: All the messaging applications that I knwo of rely on the unique names(phone numbers or user names). So, I'm not sure if it's a problem or not, at least for now. I agree with you, if possible we should look it in terms of CT (more generic than CONIKS I believe). }

\ks{Kent: Since messaging clients don't have certificates, I think we want to refer to key transparency instead of certificate transparency. Won't the providers have a ledger of keys instead of a ledger of certificates? https://github.com/google/keytransparency}

%CONIKS commits an identity provider to advertise a single, consistent set of public keys.
%Auditors and key owners monitor the system to detect equivocation. 
%The risk of detection acts as a deterrence for identity providers announcing one public key for Alice but then secretly using another in a MITM attack.


%The rest of this section contains the following: (1) A summary of the CONIKS design, (2) A description of the current CONIKS design for detecting fake key attacks when there are multiple identity providers, (3) A description of our proposal to adapt CONIKS to the single identity provider that exists in current secure messaging systems, and  (4) A security analysis of CONIKS for detecting fake key attacks for the multiple and single identity providers architectures. 



\subsection{CONIKS Background}

CONIKS has three types of actors: (1) \textit{Identity Providers} are key distribution servers that advertise the public keys of their clients. (2) \textit{Clients} run software that relies on public key cryptography, such as a secure email system, and regularly communicate with identity providers to retrieve or monitor keys. (3) \textit{Auditors} verify that identity providers are not equivocating and communicate with each other to ensure global consistency. Clients serve as auditors for their own identity provider. Identity providers can act as auditors for each other. 

Each identity provider maintains a Merkle binary prefix tree containing all of the registered keys of its clients. At regular intervals, called epochs, the identity provider signs the root of the Merkle tree, along with metadata that includes the current epoch and the hash of the previous epoch's signed tree root. This commits the provider to advertising a consistent, linear history of key bindings. 

%When a client requests the public key of a client from the identity provider, it responds with the current signed tree root (STR) and some necessary subset of the Merkle Tree, called the authentication path. The requester places its key as a node in the tree at the appropriate location in the authentication path, then generates the root of the tree and compares this root with the STR given by the provider. Thus, the STR with an authentication path act as a proof of inclusion of the client's public key by the provider. 

Three steps protect against an MKS in CONIKS. First, clients can monitor for spurious keys, ensuring that their identity provider does not advertise a fake key for them. Second, auditors receive the latest STR from each identity provider every epoch and check to ensure they follow a linear history. Third, clients periodically choose a random auditor and ensure the STR it retrieves matches what their provider gave them. \ahc{I think you didn't define  STR. I know STR from KONICS paper (but you can't assume reader does). And you didn't discuss MKS as part of the system model. I'm actually not sure that we need this special term (MKS), why not simply always say something explicit like `rogue server'? I suggest, in any case, making this a macro so it'll be easy to change to whatever we'll decide later.}
\tarun{I agree. Q1) Throughout the paper, should we refer to the attacker as Adversary A1 or rogue server? I'll wait until we decide on one before making changes throughout the paper.}

%If a client discovers misbehavior by a key server, in the form of inconsistent STRs for the same epoch, then they can alert auditors and other clients and include the proof of the inconsistent STRs.


\subsection{Multi-provider scenario}

The CONIKS architecture assumes there are multiple non-colluding identity providers. However, in current secure messaging apps there is only one key server, acting as a single provider.
\ahc{I don't agree; imho CONIKS actually {\em assumes} a single provider per `name space', it just discusses multiple providers since, obviously, the system {\em can} support more than one provider, not since the system {\em assumes} multiple providers.
It is true that CONIKS discusses the use of multiple providers for auditing, but really any parties could act as auditors. I guess if you want interaction btw uses of different providers as with email, then it seems likely that you use your own provider to audit somebody's else provider. But really they just do that imho to get rid of assuming some dedicated monitors, they make big deal of avoiding that (not that I'm convinced). 
}
\tarun{Agree. We should be clear here that they assumes multiple auditors which they do with the help of multiple providers in their scenario. So, either we need multiple providers or dedicated multiple auditors.}

One approach would be for all the secure messaging apps to cooperate by running an identity provider for their users and auditing each other.
In this instance, CONIKS would operate as designed, and 
this approach detects fake key attacks.
%We first describe a hypothetical scenario that assumes the existence of third-party, non-colluding providers that can act as auditors for each other. We describe how automated key verification using CONIKS would work in this case and explain the challenges involved.

%% shortening!

%In this instance, Alice chooses an identity provider and uploads her public key to this provider. The provider updates its Merkle prefix tree to include this new key and generates a fresh STR.  At the next epoch, it publishes this STR so other providers can audit for non-equivocation. The other providers confirm that Alice's provider has correctly signed the STR and that the STR represents a linear history.

%When Bob communicates with Alice, he first performs a key lookup for Alice and also queries several random auditors for the latest STR they received from Alice's providers. Bob audits for non-equivocation by comparing the STR from Alice's identity provider with the STRs provided by auditors. If they match, and Alice's key verifies as part of the identity provider's Merkle tree, then Bob trusts Alice's key and commences encrypted communication with Alice. Additionally, at every epoch, Alice and Bob monitor their own keys to verify that they have not changed without their consent.


% this duplicates what is in the discussion
%However, CONIKS can not distinguish between an MKS that creates a new key for Bob (and does not equivocate), as opposed to Bob changing his key and then falsely accusing the identity provider of being malicious.  There is no cryptographic proof that Bob can offer to others to prove that an identity provider was malicious as opposed to Bob simply reinstalling the application.  CONIKS provides an option requiring Bob to sign a new key with his old key. However, this breaks down if Bob loses his key (.e.g., lost or stolen phone, device crash).

\subsection{Single-provider scenario}
\tarun{TODO: Add the assumption that clients need to have some secure connections at start}
\tarun{TODO: Isolation monitoring analysis to justify that server cannot block STR verification}
Given the current lack of coordination between secure messaging apps, we propose an adaptation of the CONIKS architecture to incorporate it into a single secure messaging app.
We propose delegating the messaging app clients as auditors. At every epoch, a client checks for equivocation by comparing the STR they obtain from the central key server with the STR provided by its contacts. 
Similarly, clients monitor their own keys for inclusion in the Merkle tree advertised by the key server. 

Because there is a single provider, it is essential that clients exchange STRs during every epoch with their contacts. 
\ahc{why the fact we have single provider (per namespace, btw) imposes exchanging STRs with friends every epoch?
Yes, CONIKS assumes you get and check STR every epoch but we can easily avoid that imho by simply requiring always proof-of-consistency from the last STR we have, so that we'll always have all STRs since beginning (or long enough to ensure overlap with any peer). If we focus on single provider, this becomes actually easier than in CONIKS.
}
\tarun{Tarun: Agree. Had similar thought. We should talk about it. I was not sure how to have the latest STR without the rogue server blocking it. One solution is only to retrieve STRs from friends only when Alice starts communication with a new friend or gets a key update for one of her friends. In this case, the rogue server would know that Alice will retrieve STRs as soon as she gets key updates and drop all her messages (assuming them to be STR retrieval messages) to her other friends. Can we assume that the unreachability of all friends be considered as an attack?}

A provider may be able to identify and block STR exchanges if they occur at regular, predictable intervals or have a recognizable signature. \ahc{do you mean such exchanges are done via the providers necessarily? and even if so: can't clients detect if this communication is disabled by provider? I actually think we can easily get away with exchanging STRs only when we communicate with our friends, so that if the provider isn't yet a MitM, they are not able to interfere while providing the communication service. We can discuss. }
To defend against blocking, clients could exchange STRs using randomized delays and random-sized messages. They could also piggyback the STR onto regular messages. \ahc{yes, that's part of the solution, but we should be much more concrete and not leave multiple options and missing details as now. }
\tarun{Agree}

A client should consider the blocking of all auditing messages as malicious behavior because it is unlikely that all of its contacts disconnect from the Internet at the same moment. \ahc{again I'm not sure we need separate auditing messages. IMHO it suffices that the provider has to disconnect a client from other clients if it doesn't have MitM capabilities yet btw them and if it sent non-consistent STRs to them. }

% \tarun{[Make sure it doesn't contradict with previous paragraph. Which one is accurate?]
% From CONIKS "In other words, clients
% need to verify that any provider of interest is maintaining
% a linear STR history. Comparing each observed STR with
% every single other client with which a given client communicates would be a significant performance burden.". One of our contribution is we are only comparing STRs on key updates or new connections.
% }

\ahc{I think the design should described more clearly and in more (full) details. I also think we should completely drop this dependency on CONIKS, esp. as (I think) we shouldn't assume global unique names (as in CONIKS); instead use certificates and assume joint friends - imho, a much more realistic assumption. Yes I know this is the `trust network' solution but I simply can't see how the significant delta from the solution in this section and CONIKS!}
\tarun{TO DISCUSS}
\tarun{In this section, we tried to talk about an existing solutions and modified them a bit to fit in the current messaging application scenario like one auditor scenario. Yes! It would be interesting to see what we can add here by adding the parts of TN here. Let's discuss it and see what benefits we get through (CT + TN) over CONIKS.}

\subsection{Security Analysis}

We now analyze how well Key Transparency protects users from the attacks we have identified. For pair-targeted attacks, we assume a connection between Alice and Bob. For client-targeted attacks, we assume the targeted user is Alice.

For the {\em multi-provider scenario}, we can detect all pair-targeted and client-targeted attacks. The target of the attack can always contact an auditor, independent of its communication with its identity provider, and thus obtain proof of equivocation. We rate these attacks as detected rather than prevented because of the delay imposed by epochs. \ahc{did you discuss multi-providers at all? or auditors?? and, this isn't sufficient as analysis. when are auditors contacted? being to contact isn't enough if you don't contact! }

However, in the {\em single-provider scenario}, all communication occurs through a central key server, which makes its MITM attacks more powerful. We discuss each attack for the single-provider scenario below: \ahc{this looks like a list of specific attacks, but security should be wrt security goals and attacker capabilities, not of specific attack strategies. This will require more careful arguments but is doable. }


\subsubsection{MITM, pair-targeted} Since this attack is pair-targeted, there must exist an STR with the fake keys and another with the real keys. Alice can query any random contact for the latest (real) STR they have received from the central server and compare it to the (fake) STR she receives. She discovers the equivocation and detects this attack.

\subsubsection{MITM, client-targeted, new connections} In launching a MITM attack on Alice, the key server may choose to attack only new connections Alice makes. In this case, (1) the MKS creates a forked history for Alice containing fake keys for her new contacts, (2) a forked history for Alice's new contacts containing Alice's fake key, and (3) keeps all of Alice's existing clients on the original history. Alice can detect this attack by obtaining the latest STR from an existing contact. 
Alice's new contacts may not detect this attack if the MKS gives every client except Alice's existing clients a forked history unless a new contact shares an existing contact with Alice. However, this allows Alice's existing contacts to detect this attack when seeing exchanged STRs from other clients.

\subsubsection{MITM, client-targeted, existing connections} 
The MKS can instead choose to conduct a MITM attack on all of Alice's existing contacts by sending Alice and her contacts fake key updates. The MKS issues a consistent, linear history with the fake key for Alice to all of Alice's contacts while giving Alice a history that includes her real key but fake keys for all of her contacts. 
Key Transparency cannot detect this attack with the MKS performing an active man-in-the-middle attack because any time Alice asks for the latest STR a contact has seen, the MKS can intercept the request and falsify the response. Meanwhile, all of Alice's contacts see the same, consistent history.
To defend against this attack, we use mass key update monitoring heuristic \S\ref{subsec:MassKeyUpdate} from Trust Network defense. It \emph{prevents} naive attacks and \emph{detects} stealthy attacks.

\subsubsection{Impersonation, pair-targeted} Since this attack is pair-targeted, the target of the attack, either Alice or her contact, can query a random contact for the latest STR they have received, compare, and find the equivocation, detecting the attack. 

\subsubsection{Impersonation, client-targeted, new connections} When impersonating new clients to Alice, the MKS creates a forked history for Alice containing fake keys for her new contacts and keeps all existing contacts of Alice on the original history. Alice can detect this attack by obtaining the latest STR from an existing contact. When impersonating as Alice to new contacts, the MKS creates a forked history for her new contacts containing fake keys and keeps Alice on the original history. New contacts can detect this attack by obtaining the latest STR from a mutual contact with Alice (if they have one) or from a random contact if the MKS only gives the forked history to new contacts of Alice. Thus to have a chance of maintaining the attack, the MKS must give the forked history to all of Alice's contacts. 
This forked history allows Alice, her existing contacts, and potentially other clients to identify conflicting STRs since an exchange of conflicting STRs eventually occurs unless there is a complete partitioning of the network.

\subsubsection{Impersonation, client-targeted, existing connections} The MKS can impersonate all of Alice's existing contacts to Alice by giving Alice a history that includes her real key but fake keys for all of her contacts. This attack cannot be detected, because any time Alice asks for the latest STR a contact has seen, the MKS can intercept the request and falsify the response. Alternatively, the MKS can impersonate as Alice to her existing contacts by giving them a history that includes her fake key. This attack cannot be detected by Key Transparency alone because the MKS presents a consistent history to everyone except Alice, who can no longer communicate with anyone.
To defend against this attack, we use some Trust Network monitoring heuristics (\S\ref{sec:heuristics}).
When the MKS impersonates all of Alice's existing connections to Alice, mass key update monitoring prevents naive attacks and detects stealthy attacks. When the MKS impersonates Alice to all of her existing connections, isolation monitoring detects this attack.

% \dev{Dev:Presently, we are referring to monitoring heuristics of \S\ref{sec:heuristics}. Later in next section also we refer to heuristics of the same \S\ref{sec:heuristics}? Thus a question arises, why monitoring heuristics are part of TN, if all solutions require them in detection (or prevention) of some attacks. 
% }
% \ks{I think I noticed that and struck out that text now. Does my strikeout resolve your concern here?}

%Key transparency detects both MitM and impersonation attacks. If an MKS presents a fake key, it is detected at the next epoch through auditing or key monitoring. 
%There are two approaches to auditing. In a multi-provider scenario, the providers perform the auditing, whereas, in a single-provider scenario, the clients perform the auditing. When clients receive an STR from the key server, they request an STR from an auditor (i.e., a provider or another client) to compare with the STR they received. If there is ever a mismatch, then the server has equivocated by giving two entities inconsistent STRs for a given epoch.
%In a single-provider scenario, clients can monitor their own key to detect if a fake key ever appears in the transparency log. There is no evidence to convince third parties that the server has misbehaved, but clients can protect themselves by abandoning the service.

%All pair-targeted and client targeted attacks can be detected by auditing, assuming the key server equivocates to conduct these attacks.
%If an MKS launches a client-targeted impersonation attack on new and existing connections without equivocating by placing a fake key in the log for everyone to see, the client under attack can detect this at the next epoch. The client would have to alert the contacts of the attack out of band. This is not possible for new connections that were established after the attack commenced.


==> Defense_KT_old_2.tex <==
\section{Key Transparency Defense v2 (connected sub-graph)}
{\noindent\bf Definitions}

% Secure connection: Two benign clients have a secure connection if (1) they always have the correct public key for each other, and (2) they have successful bidirectional communication at least once per epoch.

We say that two clients have $\delta$-delay connection in a given epoch (or other time period), if all direct communication between them during this time is reliable with maximal delay $\delta$. 
We say that a pair of clients is {\em secure} during an epoch if they have a $\delta$-delay connection and have the correct public keys for each other for that epoch.

{\noindent\bf Assumptions}

We assume there exists a connected sub-graph in-band at every epoch whose vertices are the set of benign clients, and edges are secure connections. Also, $diam(G)\cdot \delta \leq duration(epoch)$.\\
% \item We assume that the propagation time from one end of the secure connection graph to the other is less than an epoch.
% \ks{Should we define a symbol for the epoch? We can use this symbol in our analysis? Yes. } \ahc{this assumption should be merged with the previous one; all we assume here is that $diam(G)\cdot \delta \leq epoch$, where $epoch$ is the (minimal) length of an epoch.  } 

\ks{I assume these are these the same secure edges in the secure messaging system, not some other secure connections based on other public keys? Does it matter?}

{\noindent\bf Justification of assumptions}

Secure connections assumption: 
Secure connections are formed whenever the server does not attack a connection. Users can verify a secure edge if they manually verify their keys in person or through another communication channel, like reading the numbers over the phone where the \acrshort{ms} is unlikely to be MitM to most of the edges.

$\delta$-delay connection: In a recent study (involving 440 mobile devices)~\cite{bradthesis}, researchers reported that the probability that a disconnected interval for a device lasts for less than one day is 0.998. So, we assume the clients consider longer isolation from a connection an attack and communicate with them out-of-band manually.

Disconnecting Graph: If the graph is connected initially and \acrshort{ms} partitions the graph, the \acrshort{ms} has to keep it partitioned forever and attack all new connections. If any of the new or existing clients ever verify the keys manually, they detect it with \acrlong{pom}.\\

% \tarun{Tarun: TODO- justification for last assumption.}

{\noindent\bf Design}\\
The server maintains a Merkle tree of all the registered client public keys. The tree is constructed as a Merkle binary prefix tree (similar to ~\cite{melara2015coniks}) to ensure that it contains exactly one public key for every client, using a phone number as a unique identifier. At regular intervals (epochs), the server generates a \acrfull{str} by signing the root of the Merkle tree, along with other metadata such as the previous epoch's \acrshort{str}. This commits the server to advertising a consistent, linear history of key bindings. 

\begin{enumerate}
    \item All clients should receive an \acrshort{str} from the server at the beginning of each epoch. If a client does not receive an \acrshort{str}, it is considered an attack and the client disconnects from the server.  
    \item For each new key lookup or key update, the client also obtains a \acrfull{poi} that it uses to verify the key is in the tree. During each epoch, clients obtain an \acrshort{str} and \acrshort{poi} of their public key within the Merkle tree from the server. Clients verify 1) their public key is in the tree using the PoI, 2) the server is publishing a linear history of \acrshort{str}s by comparing the previous \acrshort{str}'s hash in the current \acrshort{str}, and 3) the \acrshort{str}'s signature. \ahc{if checks fails, an attack...}
    % \st{In case a client disconnects and does not receive \acrshort{str}s for some epochs, the server provides the client with the sequence of \acrshort{str}s and corresponding PoIs from the last \acrshort{str} received by the client till the current one.} \ks{Can we remove this last statement because we assume clients communicate during each epoch?}
    % \tarun{makes sense to me. This has been pointed out by Dr. Herzberg earlier and it's an important point if clients disconnects. But in our case we assumes they are available every epoch.}

    \item Clients audit the server for equivocation by sharing \acrshort{str}s with all of their contacts during each epoch, immediately upon receiving it (from the server or from another client).
    If a client detects two conflicting, signed \acrshort{str}s, this constitutes a \acrfull{pom}.
    Clients detecting or receiving a \acrshort{pom}, immediately forward the \acrshort{pom} 
   %equivocation forward the conflicting \acrshort{str}s 
   to all of their contacts so that all clients in the network quickly obtain the \acrshort{pom}. \ahc{rewrote.} %evidence of equivocation.
    % Clients check with their contacts to ensure that a server never equivocates, by sending any of them a different \acrshort{str}.
    % During each epoch, clients use the secure connections to exchange and \acrshort{str}s and verify all of their contacts received the same \acrshort{str} as them. If a client finds conflicting \acrshort{str}s, equivocation is detected. Clients that detect equivocation, i.e., two conflicting \acrshort{str}s for the same period, share the conflicting \acrshort{str}s with all their contacts, proving the misbehavior of the server. Every client, on receiving a \acrfull{pom}, forward it to all of their contacts.  
    
    % To decrease the communication overhead of clients exchanging \acrshort{str}s during each epoch, all clients could sign the \acrshort{str} they obtain and send it back to the server. The server could then deliver all the signed \acrshort{str}s to each client in a single message.  \ahc{I think it may not be worth it to describe this small optimization. but if you guys want to discuss it, we should describe it properly, this description isn't really enough. }

    % \item \tarun{If a client does not receive an \acrshort{str} and \acrshort{poi} from the server during an epoch, the client considers this as misbehavior. The client could choose to stop using the service and alert its contacts. However, there is no proof that the server is misbehaving.} 
    % \ahc{but we assume client can communicate with contacts directly in this case; why not confirm with the contacts that they have the correct \acrshort{poi} for the client? }\\ 
    % \tarun{As the server cannot put a fake key in the tree for a client (according to our assumption), do we need to monitor PoI?}
    % \tarun{[What do we achieve by confirming the contacts for correct \acrshort{poi} for the client? I think in this case the client is going to detect an attack, if server put a fake key for them in the server. However, they still won't be able to prove to others, right? ... The client already know about the server's malicious behavior if it doesn't receive an \acrshort{str} within the epoch. So, what do we get by adding the verification of PoI? ]}\\
    % \tarun{This client obtains \acrshort{str} from contacts and verifies all of its contacts received the same \acrshort{str}. If they are the same, it sends this \acrshort{str} to its contacts as its own. This way, even if multiple subsequent clients don't receive an \acrshort{str} from the server, they propagate \acrshort{str}s between different ends of the network to confirm they are the same.} 
    \item A client that does not receive an \acrshort{str} from the server will receive \acrshort{str}s from its contacts and can forward the \acrshort{str} to its contacts in place of its own. If it receives any conflicting \acrshort{str} later, it can send a \acrshort{pom}. This way, even if multiple subsequent clients also did not receive an \acrshort{str} from the server, \acrshort{str}s propagate between different ends of the network to confirm whether all received \acrshort{str}s are the same. \ahc{isn't this redundant repeat of part of the previous item?}
\end{enumerate}

\begin{enumerate}
    \item All clients receive an \acrshort{str} from the server at the beginning of each epoch. 
    Clients verify the server is publishing a linear history of \acrshort{str}s by confirming the previous \acrshort{str}'s hash is in the current \acrshort{str}, and the \acrshort{str}'s signature is valid.
    If a client does not receive an \acrshort{str} or the \acrshort{str} is invalid, it is considered an attack and the client disconnects from the server.  
    
    \item For each new key lookup or key update, the client receives a \acrfull{poi} that it uses to verify the key is in the tree. During each epoch, clients also receive an \acrshort{str} and \acrshort{poi} to verify that their public is in the tree. 

    \item Clients audit the server for equivocation by sharing \acrshort{str}s with their contacts during each epoch, immediately upon receiving it. A client broadcasts the \acrshort{str} it receives from the server to its contacts. If a client detects two conflicting, signed \acrshort{str}s during an epoch, this constitutes a \acrfull{pom}.
    Clients detecting or receiving a \acrshort{pom}, immediately broadcast the \acrshort{pom} to its contacts so that all clients in the network quickly obtain the \acrshort{pom}.
    If the client does not receive an \acrshort{str} from the server, it broadcasts the first \acrshort{str} it receives from its contacts in place of its own. 
    If it receives any conflicting \acrshort{str} later, it can send a \acrshort{pom}. This way, even if multiple subsequent clients also did not receive an \acrshort{str} from the server, \acrshort{str}s propagate between different ends of the network to confirm whether all received \acrshort{str}s are the same.
\end{enumerate}

{\noindent\bf Relationship to prior work}\\
The KT defense builds on the CONIKS~\cite{melara2015coniks} design.
CONIKS assumes an environment where multiple instant messaging service providers interoperate and audit each other. Our system avoids this assumption, and works with a single provider that is not coordinating with other providers to detect equivocation. The single provider scenario matches the situation today where instant messaging services are walled gardens that do not interoperate. 

In our design the clients act as auditors, instead of the service providers, to detect equivocation. The auditing messages flow through the server like the other messages between clients\ahc{why assume this? why would we care if communication btw clients is direct? we just allow server to be a MitM, no?}, and the server can potentially launch a MITM attack. The threat to auditing messages was not part of the CONIKS threat model.\\

{\noindent\bf Analysis}\\
If the server does not equivocate, then every client in the graph receives the same \acrshort{str} during every epoch. Each client can verify their key is in the \acrshort{str} using the \acrshort{poi}.

If the server equivocates, then at least one pair of clients has conflicting \acrshort{str}s. There is at least one edge in the connected graph that has a secure connection between two clients that receive different \acrshort{str}s. The clients on each secure edge with different \acrshort{str}s will detect the equivocation.
% \ahc{not exactly true. The server may simply not send any \acrshort{str} for some clients, and there may be clients which are only connected to other clients and all of them did not receive any new \acrshort{str}. See solution above...  }
% \tarun{I updated the point above. If a client doesn't receives any \acrshort{str} within an epoch from the server, the client forwards each unique \acrshort{str} to all connections, as soon as it receives. The propagation of these \acrshort{str}s among multiple nodes can happen within one epoch, right? }
% \ahc{that's what I meant. I guess it may make sense to indeed assume that the \acrshort{str} propagation is done within same \acrshort{str}, but then we must add this to our assumptions and use this fact here. Also we should notice that this should be authenticated with the current PKs and that each client also authenticates the keys of its contacts (using PoIs from server). So even if I didn't receive the \acrshort{str} and \acrshort{poi} for my key from the server, I'll get it from my contact. But this may not suffice; maybe my contact also didn't receive PoI? and what if I just get wrong PoI? I guess we can alert our contacts since we assumed connectivity (although that may require broadcast and can only be authenticated with our old pk), but not \acrshort{pom}, and attacker can still impersonate us to new contacts, can't distinguish btw legitimate change of key and attempt to use old key to discredit server.
% We can at least make this detection in one epoch if the server must send (and signs in \acrshort{str}) the entire list of clients that changed their PKs due to reset (without signing them using previous PK). This allows clients to detect from this message (broadcasted) if the server published new PK for them without their authorization; they can then broadcast an `accusation' signed using their old key, but I'm not sure we can do anything more. 
% I think ultimately this may be an unavoidable restriction of our goals, if we agree on this, we should explain properly to the readers. But notice this is a very extreme attack, where server `takes over' benign client who is aware and disconnects from the service. I already referred to this issue in my earlier-posted comment below.}

% \tarun{I think sending list of clients that changed their PKs is too much burden. Can you help me understand what security benefit it gives us?}

% \tarun{I think we cannot allow the client to broadcast the 'accusation', as there is no guarantee that the client is not lying, even if it signs it with previous key. A client, send a key update request to the server, and then later on publish to everyone a fake 'accusation' using previous key. May be I'm not understanding your proposal correctly?}

% \tarun{
% I think these are the three possible attacks in the above scenario. \\
% Attack 1: The server doesn't give \acrshort{str} to a set of clients, but just to disconnect the flow of \acrshort{str}s. These clients are not being attacked in this case. We solve it by making the clients relay the \acrshort{str}s from contacts to other contacts.\\
% Attack 2: The server doesn't give \acrshort{str} to a set of clients because they don't want you to verify the latest contact's keys in the tree.\\
% Attack 3: The server doesn't give \acrshort{str} to a set of clients and server published a fake key for them.\\
% We are handling attack 1, and for the attack 2,3 I think the only client that is under attack is the one who is being denied \acrshort{str}. So, I think assuming an attack if a client doesn't gets an \acrshort{str} should be enough? I am not sure if the client should be allowed to alert or broadcast this alert without proof.\\
% }

The detection of conflicting \acrshort{str}s by a client proves that at least one fake key exists in the system. However, the client cannot determine which keys are fake, only that the server has equivocated.
Only the owners of each key can determine if their key is present in an \acrshort{str}. 

% T2: In the MS model, if an adversary accesses any client messages, and no client receives PoM evidence, then all the victims will detect the attack within one epoch.  (either receive no PoI or an invalid PoI)
\tarun{Tarun: I think we can use the same theorems from previous section exactly. And remove all the below theorems.}

\begin{theorem}
If the \acrshort{ms} \ahc{why use this term for the server?} partitions the graph by attacking some edges, then it is detected with a PoM whenever any pair of clients across the sub-networks, either established or new, verify the key manually.
\end{theorem}
\ahc{I don't think we need this theorem, definitely not as the first claim for KT. We assumed that $G$ is connected , no? so how can this attack happen at all? did you want to discuss the case the assumption does not hold? }

\begin{proof}
If the \acrshort{ms} partitions the graph, by being MITM, the \acrshort{ms} has to keep the established edges partitioned forever and attack all new connections. If any of the new or existing clients verify the keys out-of-band, they detect an attack. Then, they can exchange the conflicting \acrshort{str}s out-of-band for \acrshort{pom}.
\end{proof}


\begin{theorem}
If the \acrfull{ms} sends a fake key for a client to \ahc{any of} its contacts, with a corresponding valid STR, and a valid STR and Poi to the client, then all benign clients in $G$ \ahc{why `in $G$??? remove it, no?}
will receive a \acrfull{pom}.
\end{theorem}
\ahc{why not prove this?}
% \tarun{[Question: Are we going to have a proof for the above theorem or we are considering that an umbrella of 2 lemmas? Also, this is not accurate as we can see in Lemma we detect the attack in 2 epochs. So, saying that the attack is detected within one epoch is incorrect.]}

\begin{lemma}
If the \acrfull{ms} sends a fake key for a client to its contacts and all clients in $G$ receive an \acrshort{str} from the server, then all benign clients in $G$ will receive a \acrfull{pom} within one epoch.
\end{lemma} \ahc{something wrong here; as stated, it's incorrect since MS can send bad STR even to the client (who can only detect not prove); and also, if fixed, wouldn't this lemma just be  part of prev theorem?}

\begin{proof}
\textit{Mass key update monitoring} heuristic ensures that all the established edges of a client are not attacked within an epoch. Then, there is at least one secure edge that connects the client to the graph (G).

If the \acrshort{ms} presents a fake key for a client $C_1$ to a client $C_2$ during an epoch, in the next epoch \acrshort{ms} either 1) put the fake key for $C_1$ in the STR or 2) equivocates and generates two different STRs with correct and fake keys for $C_1$ and $C_2$ respectively. Our assumption of having a securely connected graph prevents \acrshort{ms} from attacking all the client's connections; therefore, the first case is not possible, and we analyze the second case further.

If \acrshort{ms} equivocates, \ie~provides inconsistent \acrshort{str}s in the network, then at least one client has the wrong \acrshort{str}, and this client is connected to the network through at least one secure edge. At least one edge in the connected graph has a secure connection between two clients that receive different \acrshort{str}s. The clients on each secure edge with different \acrshort{str}s will detect the equivocation during the comparison within that epoch.
The detection of an inconsistent \acrshort{str} by a client proves that the server has published at least one fake key (two conflicting \acrshort{str}s). Note that the clients cannot determine which keys are fake, only that the server has equivocated.

Since at least one client detects the equivocation, that client can send the proof of equivocation (two different signed \acrshort{str}s for the same epoch) back to all secure edges. Upon receiving proof of equivocation from a contact, clients forward the proof to all the other contacts. The delay in receiving an equivocation notification for a node depends on its shortest distance from the node that detects equivocation. The maximum distance an equivocation notification needs to travel is the diameter $d$ of the network. From our assumption, the time to propagate a message through $d$ diameter is less than an epoch. Therefore, all the nodes receive equivocation notification within an epoch.  
\end{proof}

\begin{lemma}
Assume a client has $m$ contacts. If the \acrfull{ms} sends a fake key for a client to at most $m-1$ of its contacts and some clients do not receive an \acrshort{str} from the server, then all benign clients in $G$ will receive a \acrshort{pom} within two epochs.
\end{lemma} \ahc{same problem here. }

\begin{proof}
\textit{Mass key update monitoring} heuristic ensures that all the established edges of a client are not attacked within an epoch. Then, there is at least one secure edge that connects the client to the graph (G).

If a client does not receive an \acrshort{str} from the server it stops communicating with it's contacts until they receive \acrshort{poi} and \acrshort{str}. It prevents attacks where the clients who do not receive the \acrshort{str} are the victims. In this case, the server prevents the client from verifying a \acrshort{poi} by not giving them an \acrshort{str}.

If the clients who do not receive an \acrshort{str} from the server during an epoch are not victims, and \acrfull{ms} presents two conflicting \acrshort{str}s. The clients, who do not receive \acrshort{str}, first obtain the \acrshort{str} from (through?) their contacts and then forward it to their remaining contacts.

The maximum distance for these \acrshort{str} to propagate is diameter $d$, when the server does not give an \acrshort{str} to any client on diameter $d$. By our assumption, this propagation of the \acrshort{str} is done within one epoch. If there exists some conflicting \acrshort{str} in any part of the network, it will be detected on at least one edge. The \acrshort{pom} is then propagated back to everyone, which takes one epoch. So the total time to detect the attack is one epoch, and it takes two epochs to alert every client in the system about the attack with the \acrshort{pom}.
\end{proof}

% \begin{theorem}
% If a client is given a fake key for all $m$ of its contacts, the mass key update monitoring heuristic detects it.\\
% \tarun{Alternate: If a client is given a fake key for $m$ of its contacts, within $x$ duration of time the mass key update monitoring heuristic detects it.}
% \end{theorem}
% \tarun{Tarun: TODO remove theorem 5.4 and write mass key history monitoring use in theorem for m contacts attack in proof.}
% \ks{What is x duration of time? x epochs? Since we say we communicate every epoch, server would have to update keys for all contacts within an epoch, so the long stealthy attack can't happen in this case?}

\begin{theorem}
No false Proof of Misbehavior is ever created. If the server is never compromised, no benign client will ever falsely detect that the server is compromised.
\end{theorem}

\begin{proof}
By definition, \acrshort{pom} occurs when a client receives two different \acrshort{str}s for the same epoch. It cannot occur unless the server creates two different Merkle trees and presents conflicting \acrshort{str}s to different clients.

In the case where the server inserts a fake key
\ahc{why do we need this part of the proof? it's not a benign server!}
for a client in the main Merkle tree and presents a consistent \acrshort{str} to everyone, the victim client detects it when verifying the \acrshort{poi} for that \acrshort{str}. 
When the client receives no \acrshort{str} from the server for an epoch, the client considers it an attack. These two client detection scenarios are not examples of \acrshort{pom} because there is no cryptographic proof. 
The current key is not used to sign a key update to avoid losing access to an account if a key is lost and no longer available to authorize a key update.
The client can still accuse the server of a false key update even after a valid key update.
\end{proof}

\ahc{I think we need also a theorem saying basically that all benign clients either are Ok at end of epoch or detect that the server is rogue and (and stop using that server, although still help in broadcasting STRs and PoMs. and then a theorem proving that if all non-detecting client have correct keys in beginning of execution, then same holds always (proof by induction on epochs). }

% \subsection{OLD THEOREMS (TO REMOVE)}

% \begin{theorem}
% No false Proof of misbehavior.
% \end{theorem}

% \begin{proof}
% A proof of misbehavior is the existence of two different \acrshort{str}s for the same epoch. It cannot occur unless the server creates two different Merkle trees and presents conflicting \acrshort{str}s to different clients.
% \end{proof}


% \ahc{The next theorem talks about a critical issue for this (and other) design: the attack where the server just `takes over' the client's identity, not caring that the client would be aware of it. I think we should introduce this threat clearly (earlier, since it applies to all designs), and present this theorem earlier, since it's essentially an easier case than the generation of PoM when server equivocates. Clearly the client can only detect this attack and `accuse' the server. We should prove (for each scheme) that a benign client would never accuse a benign server - that's easy of course (part of correctness, like no PoM against benign server). The theorem should bound the time of issuing such alert - I think in worst case it can take $d$ epochs (although that's a pretty absurd scenario).  }
% \tarun{Reordered. Not sure how can we claim here that the client cannot accuse the server? Cannot a client accuse that they published a fake key for them? As they don't have a proof in this case, at least we can accuse them.
% How does it take $d$ epochs to detect? Shouldn't it be done within one epoch?
% }
% \ahc{We {\em cannot} prevent here false accusations by a {\em rogue} client, but {\em should} claim that a {\em benign} client will never accuse. This is still missing! And, the following theorem should be rephrased; it should say that if a server includes incorrect key for a client, then {\em either} there's a PoM against the server (conflicting \acrshort{str}s), or the client alerts and disconnects from the service.}
% \begin{theorem}
% Clients detect when $A_1$ publishes a fake key for them, but without a cryptographic proof.

% \end{theorem}

% \begin{proof}
% In every epoch, clients verify their key in the Merkle tree using proof of inclusion. If the server includes a client's fake key in the Merkle tree and presents a consistent \acrshort{str} to every client, the owner of the key detects the fake key. However, there is no cryptographic proof of misbehavior.
% \end{proof}


% \ahc{the proof does not analyze properly the case where the server does not send STH (or more precisely, the correct PoI) to a client, and changes the PK of that client. This is the problematic case I referred to above. Seems clients can only alert on this; we can indeed assume these alerts are propagated quickly (but for that we need another assumption; the $d/2$ epochs is if we assume they can communicate only once per epoch, so with the assumption we can idd avoid it). Even to properly detect this (and distinguish from simple failure of communication with the server), I think we need to add the list of client's whose PK changed in this epoch, otherwise how would the client detect from the \acrshort{str} that its key was changed?  }

%\ahc{The theorem should be fixed; the detection can take up to $d/2$ epochs where $d$ is  the diameter of the secure connections graph. And, the theorem should not talk about the attacker behavior, it's better to talk about the {\em impact}, i.e., in this case, if we have an epoch in which the attacking server can be MitM btw two users. Of course, this requires the server to give them equivocating \acrshort{str}s but the claim is stated in terms of the undesirable outcome and not by term of attacker behavior  or strategy. }
% \tarun{Why the detection takes up to d/2 epochs? Atleast one edge would have conflicting \acrshort{str} within one epoch and the nodes corresponding to that edge detects equivocation.
% Regarding second point, should we say MITM or impersonation attack? MITM can happen either by equivocating or by presenting fake to everyone (without equivocating). Here in this theorem we are trying to only capture the case where they equivocate. Should we write something like "If the server executes MITM by by distributing conflicting \acrshort{str}s during an epoch, ..."
% }

% \ahc{I removed above comments since I think the theorem below is now Ok, but notice it's weak, since it refers to specific attack behavior. So it looks more like a lemma; we should really have theorem which states what the protocol ensures against arbitrary attack strategy.}

% \begin{theorem}
% \st{If the server equivocates by distributing conflicting STRs during an epoch, the equivocation is detected by at least one node within that same epoch that now has a cryptographic proof of the misbehavior.}
% If the server executes MITM by distributing conflicting \acrshort{str} during an epoch, the equivocation is detected by at least one node within that same epoch with a cryptographic proof of the misbehavior.

% \end{theorem}


% \begin{proof}
% If the server equivocates, \ie~provides inconsistent \acrshort{str}s in the network, then at least one client has the wrong \acrshort{str}, and this client is connected to the network through at least one secure edge. At least one edge in the connected graph has a secure connection between two clients that receive different \acrshort{str}s. The clients on each secure edge with different \acrshort{str}s will detect the equivocation during the comparison within that epoch.
% The detection of an inconsistent \acrshort{str} by a client proves that at least one fake key exists in the system (two conflicting \acrshort{str}s). Note that the clients cannot determine which keys are fake, only that the server has equivocated.
% \end{proof}

% \ahc{the theorem below should be improved by adding that this is done within either one epoch or a given number of epoch since sending the conflicting STHs. This simply depends if we want to assume that these PoMs and detections are done quickly within same epoch or assume one communication per epoch. 
% Once this is determined, the theorem need to be modified; and the proof, in any case, simplified, simply use the diameter $d$ of the graph of secure connections. 
% I comment-out earlier comments. }

% \ahc{this theorem should also be improved, this time the claim is weaker than what it should be! in reality we can bound the time that all clients receive the PoM to  $d$, the diameter of the secure connections graph.
% But I think the claim should also be made clearer; currently it isn't clear what does the time count begin. I understand the idea was to count from detection, but I think it'll be better to simply bound the time from the epoch in which the server equivocated (so total time will be $\frac{3d}{2}$).
% }

% \tarun{Agree. we can update it once we decide on how long does it take to detect equivocation. look at previous comment before Theorem 1. I think we can propagate the proof(contradicting \acrshort{str}s) within one epoch after detection, unless the epoch is too small. The total edges/steps are bound to d. }

% \begin{theorem}
% All the nodes in the graph will be made aware of the misbehavior by a proof of equivocation.
% \end{theorem}

% \begin{proof}
% Since at least one client detects the equivocation, that client can send the proof of equivocation (two different signed \acrshort{str}s for the same epoch) back along all secure edges. Upon receiving proof of equivocation from a friend, clients forward the proof to all the other secure friends. The delay in receiving an equivocation notification for any node $i$ in the network depends on the shortest distance $d_i$ from a node that detects equivocation. 
% All nodes will be notified of the equivocation within $max(d_i)$ steps. 
% \end{proof}





















% \section{Key Transparency Defense (Old)}

% The goal of the Key Transparency (KT)~\cite{melara2015coniks,chaseseemless}
% \ahc{I suggest removing these citations from here; it isn't clear what it means, i.e., is this solution taken from there (as is)? I think we should discuss the relationships more clearly (and probably after presenting the design, making it easy for us to explain what we took and what we did differently. For readers that may know CONIKS, we could also say up front that the design is based on the CONIKS design, with citations, and mention we compare later.}
% defense is to detect the distribution of a fake key by the server to a client. 
% \ahc{isn't the above goal shared by all defenses? if so, I guess we better remove it from here. }
% KT utilizes an append-only ledger for storing public keys. 
% \st{The server maintains a Merkle tree of all the registered client public keys. At regular intervals (epochs), the server signs the root of the Merkle tree, along with metadata that includes the current epoch and the hash of the previous epoch's STR.} 
% \tarun{The server maintains a Merkle tree of all the registered client public keys. At regular intervals (epochs), the server generates \acrshort{str} by signing the root of the Merkle tree, along with metadata like previous epoch's \acrshort{str}.}
% \ahc{don't we want the server to also share this \acrshort{str} with all clients? also, clarify what's an \acrshort{str}: just the signature over the root, or (more likely...) the value of the root, the metadata and the signature over them? }
% \tarun{Updated.}
% This commits the server to advertising a consistent, linear history of key bindings. 
% \st{A client can audit the server to confirm that its public key and the public keys for its contacts are contained in the Merkle tree.}
% \ahc{that's right except: (1) it isn't optional; in every epoch the client should receive that epoch's \acrshort{str} from the server (as we just said...) so it should do this validation (and I'm not sure we should refer to this as audit; audit is usually an active, optional check); (2) to do the validation, we should specify that the server should provide each client with a \acrshort{poi} of that client's public key in the tree; I know you refer to this later, but...don't split.  (3) for this to work we must make sure that the tree cannot contain another public key for the same subject, e.g., by organizing it like in CONIKS (or similarly). 
% (4) why use the term ledger? it isn't a blockchain, and let's only terms we need and define without multiple terms. Here it should simply be `tree' (or, add `Merkle'). 
% }
% Clients receive the latest \acrshort{str} from the server and can verify a linear history of \acrshort{str}s. 
% \ahc{note that this also requires that if a customer was disconnected and did not receive \acrshort{str}s of some epochs, the server will provide them with the sequence of \acrshort{str}s from the one they have till the current one.}
% \ks{Yes, notice assumption 2 below that we assume clients communicate during each epoch, so they also communicate with the server. Should we add an explanation here to summarize your point, or make this explicit in the assumptions?} \ahc{I think it's better to {\em begin} each the three designs with a brief introduction of the relevant unique aspect of the system model, i.e., assumptions required for this design. }
% Clients check with their contacts to ensure that a server never equivocates by presenting any of them a different \acrshort{str}. 

% \ahc{I think we better completely describe our design and only then discuss differences from previous work (in this case, mostly CONIKS). Also, above you already described part of the design, and now you break and later begin again, with some repetition... really better if you describe it all together and at the beginning (after assumptions though).}
% Our assumptions differ from the CONIKS design in three ways. 
% (1) We assume a single provider that is not coordinating with other providers to detect equivocation. 
% This matches the situation today where instant messaging services are walled gardens that do not interoperate. CONIKS assumes an environment where there are multiple instant messaging service providers that interoperate and audit each other. \ahc{it's not that we assume a single provider! our solution can clearly be used separately by multiple providers! it is just that we {\em avoid} the CONIKS assumption, which isn't simply that there are multiple providers, but also that they cooperate - indeed a problematic assumption!}
% (2) The clients act as auditors, instead of the service providers, to detect equivocation. \ahc{that's a difference but in the design not in the assumptions. }
% (3) We do not rely on an out-of-band channel between the clients, so the auditing messages flow through the server that can potentially launch a MITM attack. 
% Our assumptions raise new security issues not addressed in the original CONIKS paper. \ahc{what do you mean?? which issues? }

% % Meeting notes 4/1/2021. %%%%%%%%%%%%%%%%%%%%%%%%%%
% % Upfront mention that each design will have its own assumptions.
% % Compare all the solutions in the end.
% % Communicate within a bounded delay delta
% % Diameter is bounded then attacker can impersonate at the end of the graph - be certain we can detect in certain amount of time

% Our KT defense has the following assumptions:
% \begin{enumerate}
% \item The system is modeled as a well-connected graph $G$ with $k$ nodes representing the clients and a set of edges $E$. Each edge represents a secure connection between two clients (\ie~they have each other's correct public key). Secure edges are formed whenever the server does not attack a connection. The existence of a secure edge can be verified if the participants manually verify their keys.
% \ahc{this assumption should be rephrased. First we should define the notion of a secure edge: we say that two clients have a secure connection if (1) they always have the correct public keys of each other, and (2) they have  successful bidirectional  communication at least once in every epoch - via the server, or, if this fails, using a different communication service. Then we should state the assumption, i.e., that the graph whose nodes are the benign clients and whose edges are the secure connections, which I suggest we call by some term such as the {\em secure connections graph}, is a connected graph. (btw, why `well connected'? it's not a directed relationship, is it?) Ah and I think we should separate btw the assumptions and the justifications for the assumptions. }
% % \tarun{If a client has atleast two secure friends initially, the mass key monitoring heuristic ensures that all of their connections cannot be compromised within an epoch. Assume a connected messaging network, not attacked by server, and every client has atleast two friends. The mass key monitoring heuristic ensure that there will always be secure connected  }
% % \item \st{The communication between these secure $E$ edges happens within every epoch. The isolation monitoring detects communication blocking with secure friends.}
% \item The clients are able to communicate along each secure edge during every epoch. In a recent study (involving 440 mobile devices) [25], researchers reported that the probability that a disconnected interval for a device lasts for less than one day is 0.998. So, we assume the clients consider longer isolation from a secure connection an attack and communicate to them out-of-band manually. \ahc{I think this is just part of the same assumption and not a separate one; and while the justification is nice, I still think we should separate btw assumption and justification. }
% \end{enumerate}

% % The isolation monitoring detects communication blocking with secure friends, and mass key monitoring detects if the server compromises all the friends of a client during the same epoch.
% % \ks{Do we need to state this in this section? During the security analysis?}

% The client monitoring works as follows:
% % \begin{enumerate}
% % \item During each epoch, clients obtain an \acrshort{str} and proof of inclusion from the server and verify that their public key is in the ledger.
% % \item During each epoch, clients randomly request an \acrshort{str} from a random friend. If a response is not timely, the client randomly requests an \acrshort{str} from other friends until a response is received. These requests and responses for \acrshort{str}s may be piggybacked on normal communications between clients.

% % Have to compare to the good edge. Compare with all of your friends. What about efficiency. 
% % Every epoch you give server a signed statement, server hands them out, or you compare directly with each friend.
% % Once per epoch the graph is well-connected.

% % \end{enumerate}

% \begin{enumerate}
% \item During each epoch, clients obtain an \acrshort{str} and proof of inclusion from the server and verify that their public key is in the ledger.
% \ahc{better describe all checks (correct previous ledger, correct signature).}
% \item During each epoch, clients use the secure messaging provider
% \ahc{which `secure messaging provider'?? again: use consistent terms!!}
% to exchange and compare \acrshort{str}s with all of their friends. If a mismatch occurs, equivocation is detected. Following detection, a client shares proof of the equivocation (two different \acrshort{str}s within same epoch signed by the server) with all its secure friends. \ahc{remove `secure' - we'll share it with everyone for sure...}\\
% To decrease the communication overhead of clients exchanging \acrshort{str}s during each epoch, all clients could sign the \acrshort{str} they obtain and send it back to the server. The server could then deliver all the signed \acrshort{str}s to each client in a single message.  \ahc{I think it may not be worth it to describe this small optimization. but if you guys want to discuss it, we should describe it properly, this description isn't really enough. }
% % Compare \acrshort{str} with all secure friends every epoch
% % 		may be get it signed by friends and send it to server, and server sends secure friends signed \acrshort{str}s

% \ahc{you didn't describe how we handle the case where we do not receive the \acrshort{str} from the server. In this case, we kind of detect immediately a problem but have no proof; we should wait to receive the \acrshort{str} from one of our secure connections. Notice this may take few rounds; we should propagate in such cases all \acrshort{str}s that our peer (in the secure connection) did not receive. This will ensure that if the server equivocated, eventually we'll get a PoM. Ah, and the protocol should also propagate PoM to all clients!!}
% \tarun{Why it takes few rounds? Cannot it happen in just one epoch if epoch isn't too short.}

% \ahc{Also notice we {\em could} add an `alert' mechanism where a client informs her peers that they didn't receive any \acrshort{str} from the server - which, if the client is benign, implies that the server is rogue. The problem is that the peer cannot really propagate this (even if we assume you trust your securely-connected peer, we surely don't want to assume this is transitive so everyone is trusted...). So I think this doesn't give much benefit cf to the PoM and I tend to think we shouldn't get into this at all. 
% }

% % \ks{
% % \item [Revise prior item for review] During each epoch, clients exchange and compare \acrshort{str}s with all of their friends. If a mismatch occurs, equivocation is detected. Following detection, a client shares proof of the equivocation (two different \acrshort{str}s within same epoch signed by the server) with all its friends.\\
% % To decrease the communication overhead of clients exchanging \acrshort{str}s during each epoch, all clients could sign the \acrshort{str} they obtain and send it back to the server. The server could then deliver all the signed \acrshort{str}s to each client in a single message. 
% % }
% \end{enumerate}

% If the server does not equivocate, then every client in the graph receives the same \acrshort{str} during every epoch. Each client can verify their key is in the \acrshort{str} using a proof of inclusion.

% If the server equivocates, then at least one client has the wrong \acrshort{str}. 
% \ahc{what does it mean `the wrong \acrshort{str}'?? there are simply two conflicting (equivocating) \acrshort{str}s, I don't think we can call one of them `wrong' !}
% There is at least one edge in the connected graph that has a secure connection between two clients that receive different \acrshort{str}s. The clients on each secure edge with different \acrshort{str}s will detect the equivocation.
% \ahc{not exactly true. The server may simply not send any \acrshort{str} for some clients, and there may be clients which are only connected to other clients and all of them did not receive any new \acrshort{str}. See solution above...  }

% The detection of an inconsistent \acrshort{str} by a client proves that at least one fake key exists in the system. However, the client cannot determine which keys are fake, only that the server has equivocated.
% Only the owners of each key can determine if their key is present in an \acrshort{str}. 

% %%%%%%%% NOTES
% % Theorem - argument form
% % Detection if provider is providing inconsistent \acrshort{str}s, some node will detect it within the same epoch with a proof of misbehavior (conflicting \acrshort{str}s).

% % Within diameter of the network, all benign nodes will become aware of the misbehavior

% % If provider is benign, never have a proof of misbehavior. No false positives.

% % What if provider doesn't hand out \acrshort{str}s? We can detect but not prove to others.

% % What about detecting your own key for yourself?
% % Clients can change keys?
% % Some users can detect an attack but cannot prove it to others

% % We can have a stronger property if we require user to sign key changes with old key

% % Need good edges for those not detecting immediately

% % Assumption about good clients which are not immediately raising an alert.

% \ahc{The theorem should be fixed; the detection can take up to $d/2$ epochs where $d$ is  the diameter of the secure connections graph.
% And, the theorem should not talk about the attacker behavior, it's better to talk about the {\em impact}, i.e., in this case, if we have an epoch in which the attacking server can be MitM btw two users. Of course, this requires the server to give them equivocating \acrshort{str}s but the claim is stated in terms of the undesirable outcome and not by term of attacker behavior  or strategy. 
% }
% \begin{theorem}
% If the server equivocates by distributing conflicting \acrshort{str}s during an epoch, the equivocation is detected by at least one node within that same epoch that now has a cryptographic proof of the misbehavior.
% \end{theorem}

% \begin{proof}
% If the server equivocates, \ie~provides inconsistent \acrshort{str}s in the network, then at least one client has the wrong \acrshort{str}, and this client is connected to the network through at least one secure edge. At least one edge in the connected graph has a secure connection between two clients that receive different \acrshort{str}s. The clients on each secure edge with different \acrshort{str}s will detect the equivocation during the comparison within that epoch.
% The detection of an inconsistent \acrshort{str} by a client proves that at least one fake key exists in the system (two conflicting \acrshort{str}s). However, the clients cannot determine which keys are fake, only that the server has equivocated.
% \end{proof}

% \ahc{this theorem should also be improved, this time the claim is weaker than what it should be! in reality we can bound the time that all clients receive the PoM to  $d$, the diameter of the secure connections graph.
% But I think the claim should also be made clearer; currently it isn't clear what does the time count begin. I understand the idea was to count from detection, but I think it'll be better to simply bound the time from the epoch in which the server equivocated (so total time will be $\frac{3d}{2}$).
% }

% \begin{theorem}
% All the nodes in the graph will be made aware of the misbehavior by a proof of equivocation.
% \end{theorem}

% \begin{proof}
% Since at least one client detects the equivocation, that client can send the proof of equivocation (two different signed \acrshort{str}s for the same epoch) back along all secure edges. Upon receiving proof of equivocation from a friend, clients forward the proof to all the other secure friends. The delay in receiving an equivocation notification for any node $i$ in the network depends on the shortest distance $d_i$ from a node that detects equivocation. 
% All nodes will be notified of the equivocation within $max(d_i)$ steps. 

% \end{proof}

% \ahc{I think the next proof- which I think we should call `no false PoM' or `no false positives' - should appear first, before the theorems about the attacks. also , let's consistently use `proof of misbehavior' (PoM)... }

% \begin{theorem}
% If the server is benign, a proof of equivocation does not exist.
% \end{theorem}

% \begin{proof}
% A proof of equivocation is the existence of two different \acrshort{str}s for the same epoch. It cannot occur unless the server creates two different Merkle trees and presents conflicting \acrshort{str}s to different clients.
% \end{proof}

% \ahc{The next theorem talks about a critical issue for this (and other) design: the attack where the server just `takes over' the client's identity, not caring that the client would be aware of it. I think we should introduce this threat clearly (earlier, since it applies to all designs), and present this theorem earlier, since it's essentially an easier case than the generation of PoM when server equivocates. Clearly the client can only detect this attack and `accuse' the server. We should prove (for each scheme) that a benign client would never accuse a benign server - that's easy of course (part of correctness, like no PoM against benign server). The theorem should bound the time of issuing such alert - I think in worst case it can take $d$ epochs (although that's a pretty absurd scenario).  }

% \begin{theorem}
% Clients can detect when $A_1$ publishes a fake key for them, but there is no cryptographic proof to convince a third party.
% \end{theorem}

% \begin{proof}
% In every epoch, clients verify their key in the Merkle tree using proof of inclusion. If the server includes a client's fake key in the Merkle tree and presents a consistent \acrshort{str} to every client, the owner of the key detects the fake key. However, there is no cryptographic proof of misbehavior.
% \end{proof}

% \dz{I like the direction toward more formalism here. The cynic in me would counter that by assuming every client has one or two secure connections to other clients (connections that can't be tampered with by the provider), you are essentially assuming the problem away. The hard problem seems to be ensuring that this actually is the case. Do we need to spend more time talking about how to ensure this, as opposed to assuming it?}

% \ks{
% We believe there is justification for the assumption that the network graph remains well-connected for detecting an attack even in the face of attacks from $A_1$. 
% We are not assuming that there are secure connections the provider cannot attack. 
% The defense works as long as $A_1$ does not attack {\em all} the connections for a client. 
% Recall that we assume the system is not compromised from the beginning, so the graph is well-connected in advance of any attack.
% Most user's have more than one contact, so the graph remains well-connected for pair-targeted attacks unless a client has only one connection.
% The defense does not protect a client with only one contact.
% If all edges for a user are compromised, mass key update monitoring detects it.
% One way to strengthen the assumptions is for each user to manually confirm one secure connection when they join, and let KT approach detect subsequent attacks. 
% This places a much lighter burden on users compared to expecting them to manually verify all key updates. Is this last item an important point for the conclusions if we agree it makes sense?
% Basically, if we will all verify one contact, KT will help us detect any future attacks on the network. Also, as long as the system wasn't compromised from the beginning, these automated defenses do provide some guarantees to detect attacks.
% }
% \ahc{I also think this is actually a reasonable assumption - and it seems unavoidable for this solution, anyway... Notice the assumption does not assume secure connectivity via the (rogue) server, it can be connectivity in some other way. Now, your software should alert you that you lost all connectivity to your provider - that's pretty alarming already - and our assumption is basically that users will have some alternate connection via which they can exchange the PKs and in fact the \acrshort{str}s one of them got (from server or from another secure contact). I think in reality, your software should do all this communication using a direct peer-to-peer connection, not via the provider. So it seems quite reasonable to me.  }




==> Defense_TN.tex <==
\section{Trust Network Defense}

The Trust Network (TN) defense relies on the clients in the secure messaging network to cooperate in detecting fake key attacks.
TN does not rely on any third-party infrastructure like Tor in AKM. One limitation of relying on an anonymous system like Tor is that it is blocked by certain countries and organizations, which limits its applicability.
TN also does not depend on any out-of-band channels but uses the existing secure communication channels between clients that flow through the server.
Given these simpler deployment requirements, the challenge is to determine how well a system can defend against fake key attacks when the server observes all messages and is an on-path attacker.

%\ks{If a closed group (company, political campaign, activists) want to secure their communications using Signal, could TN be deployed without any changes to the server if contact lists and key requests do not need to be kept private? Do we need the signed timestamp on verification bundles?}

%\ks{One motivation for TN is that Tor is blocked by countries and organizations. Not relying on a third party means it can be everywhere.}

%\tarun{Connected graph assumption can be feasible in case of SIGNAL APP because they do not have information about contacts and the graph, hence cannot partition graph}

% \ks{The hash of the identity. We've talked about this being phone numbers. Isn't it fairly easy to brute force all possible phone numbers? Is it worth having this privacy feature? We should introduce it as a privacy feature, I believe.}
% \tarun{Yes! These can be brute forced if they are phone numbers. But the identifier can be username, email addresses or other identifier which could be harder to brute force than phone numbers. But I agree it's not a strong defense. Are you proposing in our design we do not talk about hashing and at the end explain this privacy feature?}
% \ks{Not sure about moving it, but we should mention the limitation for reviewer so they know we are aware.}

%Trust Network is more usable than KT as it tells exactly which keys are fake in the system, and TN is more usable and deployable than AKM, as it does not require any third-party support.

{\noindent\bf Additional adversary model (Malicious Client)}

Since TN depends on other clients to verify keys for a client $i$ and these clients do not need to be direct connections, we have to consider a malicious client. A Malicious Client (MC) has access to its long-term private key of a client. The MC does not control or collude with the server
\ahc{can't we avoid this strong assumption? it makes this model less interesting, for the goal of disrupting monitoring. Unless the goal is specifically to disrupt monitoring for a benign server. Not clear. }.
\tarun{Yes! The goal of the MC is to disrupt monitoring for a benign server.}

% The MC's goal is to identify all of Bob's contacts. The second goal is to disrupt the communication of other contacts (by lying to them during key verification).

MCs goal is to 1) identify all of the victim's contacts and 2) to disrupt the overall monitoring of the system and interfere with a specific client's monitoring by blocking messages or presenting fake messages. 

{\noindent\bf Definitions}
% We say that two clients have a $\delta$-delay connection over a channel in a given epoch (or other time period), if all communication between them during this time is reliable with maximal delay $\delta$. \ahc{already defined/assumed, no?}

We say that a pair of clients have a {\em secure in-band} connection  if they have a $\delta$-delay communication \textit{through the server} and have the correct public keys for each other throughout that epoch. 
% \ahc{during entire epoch, or only at beginning of epoch?}



% The degree of separation ($s$) is the number of hops to reach from one client to any other client. In 2016, Facebook network has a $3.57$ degree of separation on average  \dev{it should be a citation or a footnote} [https://research.fb.com/blog/2016/02/three-and-a-half-degrees-of-separation/]

    
{\noindent\bf Assumptions}

In every epoch $e$ there exists a well-connected graph $G$ whose vertices are all of the benign clients and whose edges are {\em secure in-band} connections. 
\ahc{that's a weird assumption, since the server can introduce delays for connections going through it.} \tarun{All the communication through them is normal messaging communication. So, we are assuming they do not randomly delay those messages between clients. Is that an unreasonable assumption?}
Also, the server has $\delta/2$-delay connections with all clients. 
\tarun{TODO: Put the assumption that directly connected MC does not interefere with monitoring process?}

% Also, $diam(G)\cdot \delta \leq duration(epoch)/2$.\\
% \dev{The rationale behind the preeceding equation is not explained.}\\


    % \item The server doesn’t do collateral damage. i.e it doesn’t block normal communication messages to block the verification messages.
    % \item The server does not completely block communication between two nodes for longer than an epoch.

    % \item Epoch $e$ is long enough such that messages travel from every client to every other client in the network within $diam(G)$ epochs using secure connections. 
    % \item We assume keys are distributed by the server using a push-based model.



{\noindent\bf Justification of Assumptions}\\
The justification for the $\delta$-delay connection assumption is the same as presented in section ~\ref{connection-justification}.

% However, in unlikely cases, the detection might take longer depending on the duration of client disconnections. For simplicity, we assume that all the clients are online every epoch.

Since it is unlikely that a secure messaging system is compromised from the beginning, the existing secure connections form the well-connected graph $G$ before any fake key attack. The assumption will continue to hold for each epoch until the \acrshort{ms} attacks enough connections to partition the graph, and maintains the attack indefinitely to defeat the detection method. 
The TN defense significantly raises the bar for the attacker compared to current systems. 

% Traffic assumption: In the WhatsApp network of 1.6 billion active users monthly, 65 billion messages are sent every day.\\

{\noindent\bf Design}
We first present the high-level design and explain the details in later subsections: 
\begin{itemize}
    \item  Once per epoch, every client $c_1$ randomly {\em monitors their key} through a \textit{proxy} to ensure the server is consistently distributing their key. The \textit{proxy} is a random client 
\ahc{random: uniformly selected among all clients? how can a client uniformly-randomly select such proxy?  do you assume server does not control (e.g., invent) clients? If server controls clients, maybe WHP a random client is controlled by server?}   
\tarun{Clients randomly select one of their edges at every relay. So, we assume they are random enough? Yes! The server can introduce such clients. But they have to be connected to some clients. Even if that is done, the clients only need half of the monitoring to be successful. Look at the monitoring through a proxy section. }    in the graph $G$ that receives the monitoring request from $c_1$ in a way that makes it hard for the server to predict on whose behalf the proxy is making the request.
     
    \item Clients verify keys for new connections and key updates through mutual friends. 
    % Our simulation results (simulation setup is described in section~\ref{simulation_setup}) show that around 59\% of connections have at least one mutual friend.
    Evidence from our analysis of a Facebook subnetwork suggests that it may be common for two contacts in the network to have a mutual friend. \tarun{TODO:<cite the appendix>}
    % \ahc{I'm not sure, how the percentage of mutual friends in simulation is relevant. Do we make some corresponding assumption?} \tarun{No! We use mutual friends in our design. These results provides usefulness of this part of the design, where we can use a mutual friend.}
    
    
    
    
    \item Every client $c_1$ randomly {\em monitors keys for new connections and key updates} through a \textit{proxy} for $n$ epochs after receipt of a new key.
    % \item Clients monitor a new contact's key and recent key updates for multiple epochs by requesting the contact’s key through a relay of friends.
    % \item Clients monitor their key every epoch by requesting their key through a relay of friends.

\tarun{TODO: Tarun switch 2 and 3 here. And switch sections.}
\end{itemize}


\subsection{Mutual Contact}
% \tarun{TODO: Explain how to use PSI for finding contacts intersection and limit privacy leak.}
% \ks{I think we need a PSI solution or limit the proposal to send the hash of public key so only mutual contacts are discovered. Periodically refresh the database to discover new mutual contacts. The privacy leak is too big a target for reviewers, I fear, unless we believe there are important subsets that would use this. But those subsets would work with the hash of the key instead of phone number.}


\label{mutual_contact}

% \begin{figure}
% 	\centering
% Eddie	\includegraphics[width=0.4\textwidth]{images/Mutual_Contact_Updated.pdf}
% 	\caption{Mutual Contact: (1) Alice's contacts share the verification bundle of their contacts with Alice. She maintains a database of her contacts' contacts verification bundle. (2) Alice queries the server for Bob's key. The server responds with Bob's verification bundle. Alice compares the two sets of keys (\emph{i.e.,} 1 and 2). If a key mismatch is found, an attack is detected. 
% 	\ahc{Comments: 1. I suggest you use names for Alice's contact, not A, B and C. 2. the entity in the middle is the server, right? so just write this next to it. 3. I believe Alice get's only bundles for contacts she shares with A, B or C; and if Alice just connected to Bob in step 2, then it wouldn't receive Bob's bundle after doing the PSI (i.e. at step 1). 3. why do you use number 2 for all three flows? (I also think it'll be better to use 1A, 1B and 1C for the three `step 1').  }\\
% 	\tarun{I propose we remove this figure as we are short on space. If we really want to keep this figure, I'll update it for only one contact and to include PSI part.}
% % 	\ahc{how? what does Alice do in such case? and isn't it possible that the key changed legitimately?}} \tarun{Explained these in the text. Do we want to explain it here too?} \ks{What does "for the same timestamp" mean? How would there be two keys with the exact same timestamp? Is that in the text?
% }
% 	\label{fig:MutualFriend}
% \end{figure}



The key server generates a long-term asymmetric key pair and distributes the public key to clients at the time of registration. Whenever Alice requests her contact Bob's public key, the key server responds with Bob's signed public key and the signed \textit{verification bundle}. A verification bundle contains Bob's identity (\emph{e.g.} phone number), a hash of Bob's public key, the current timestamp when the verification bundle is created and a timestamp indicating the time when Bob pushed his public key to the key server.
% \tarun{Updated sentence} A verification bundle contains Bob's public key and the current timestamp when the verification bundle is created and a timestamp indicating the time when Bob pushed his public key to the key server. The verification bundle is encrypted by Bob's identity (\emph{e.g.} phone number) as key. As the encrypted content is random enough, it is infeasible to perform a brute force attack to find the identity.

% \tarun{TODO: 1) Do PSI first. 2) Exchange verification bundle = public key + timestamp.}

% \tarun{New para}
% To identify the list of shared contact's verification bundle, clients use Diffie-Hellman based Private Set Intersection (PSI) protocol (such as~\cite{huberman1999enhancing}~\cite{de2010linear}). These protocols use a simple modification of the Diffie-Hellman key agreement protocol to achieve PSI. 
% \begin{align*}
% verificationBundle = Enc_{identity}(PublicKey|timestamp)
% \end{align*}
% \begin{align*}
%     sig_{serverkey}(verificationBundle)
% \end{align*}
% \tarun{New para}
% Alice and Bob use PSI on their contact identity sets to identify shared contacts. After finding the identities of the shared connections, they can decrypt the verification bundle and retrieve the corresponding public key and timestamp. The identity is not revealed through the verification bundles until the clients perform a PSI on the identities and then decrypt the verification bundle.

Whenever two clients start communication for the first time, they both perform Private Set Intersection (PSI) on their contact's set to identify a list of shared contact's verification bundles. 
\ahc{there's a potential privacy exposure here, you know. we need at least to acknowledge it. } \tarun{Privacy exposure of Mutual friends, right? We have presented it at the end of this subsection. Is there anything we are missing?}
The PSI protocol helps two parties identify the intersection of two sets without informing them about the whole sets. Clients use Diffie-Hellman-based Private Set Intersection (PSI) protocol (such as~\cite{huberman1999enhancing}~\cite{de2010linear}), which use a simple modification of the Diffie-Hellman key agreement protocol to achieve PSI. Then, both the clients' exchange shared contacts' verification bundles as shown in Figure \ref{fig:MutualFriend}. Alice verifies the server's signature on each verification bundle to ensure that Bob does not forge his contact' keys. Alice maintains a database of the verification bundles of her mutual contacts. Whenever Alice obtains a key update message from the server for her contact, she sends a \textit{database update message}, to all her contacts who are mutual friends with Bob, with the new verification bundle for Bob. Assuming all clients do this, Alice can maintain the latest verification bundle of her two-hop contacts. When Alice starts communicating to a new client, she performs PSI for that identity with all of her contacts' contacts identity to find a shared friend. \ahc{how can we deal with a server dropping such PSI request with a particular contact to foil this check? also, there's further privacy exposure here: your contacts learn immediately whenever you connect with a new contact. } \tarun{PSI is happening with secure friends. So, it is a secure channel, and the server has no way to know which of the communication between two clients is of PSI. The clients learn when you communicate to a new client, but not whom you communicate to, right? However, that's an interesting point. They could know the total number of my contacts. That's what you want to say?}


% \tarun{New paragraph} When Alice starts communication with Charlie or gets a key update for Charlie, she checks whether Charlie's verification bundle exists in the database. If it exists, Alice compares Charlie's key received from the server with the key in the verification bundle. In case of timestamp matches, and if the keys also match, it is a legal key; otherwise, it is an attack. In case of timestamp mismatches, Alice asks for a verification bundle update from all the contacts who sent her Charlie's verification bundle. Those contacts wait for $\delta$ time, where $\delta$ is the maximum time it takes to receive an updated key from the server. And then contacts returns either the updated response or the same key with the previous timestamp. If the key and the timestamp match, Alice marks the key as secure otherwise it considers it an attack, and Alice notifies the contact that helped detect this attack. Here, Alice trusts her mutual contact to give her key updates instead of lying that they did not receive them.

 When Alice starts communication with Bob or gets a key update for Bob, she checks whether Bob's verification bundle exists in her database. If it exists, Alice compares Bob's key received from the server with the key in the verification bundle. If both the timestamp and key match, it is a legal key. If the timestamps match and the keys do not, it is an attack. In case the timestamps do not match, Alice requests a verification bundle update from all the contacts who previously sent her Bob's verification bundle. Those contacts wait for $\delta$ time, where $\delta$ is the maximum time it takes to receive an updated key from the server. The contacts reply with either an updated bundle or the previous bundle. If the key and the timestamp match, Alice marks the key as secure, otherwise it considers it an attack, and Alice notifies the contact that helped detect this attack. Alice trusts her mutual contact to give her the most recent key update instead of lying that they did not receive it. \ahc{so what prevents the server from changing the key for {\em all} mutual contacts? and what do you mean that we trust the mutual contact ? what do we do if the mutual contact says it received no response to the request for update bundle?}

{\noindent\bf Privacy leak:} The mutual contact approach introduces a privacy concern since it leaks contact information. Some applications are not suitable for this approach, while others may value its strong detection capabilities without adding new infrastructure. For example, LinkedIn shows shared connections, and their documentation says \textit{"No matter which setting you select, your 1st-degree connections will always be able to see shared connections."}~\cite{linkedinHelp}.

\begin{lemma}
If the \acrfull{ms} sends Bob's fake key to Alice, and Alice shares a mutual contact with Bob, and both Alice and mutual contact have a secure connection with that Bob, then Alice detects the fake key with $6\dot\delta$ and prevents the attack.
\tarun{@Dr. Seamons please review the updated lemma and proof.}
\end{lemma}

\begin{proof}
    All clients perform PSI and maintain a database of their contacts' mutual contacts key. If Alice gets a key update for mutual contact, Charlie, Alice first verifies the key in the database and detects the attack instantly if there is a mismatch. Suppose Charlie's key in the database is outdated (key upload timestamp of the database mismatches). In that case, Alice asks the mutual contact to retrieve the updated Charlie's key and return it to her. This takes up to $3\dot\delta$ delay to detect the attack.
    
    If Alice starts communicating with a new contact, Bob, Alice performs PSI with all of her contacts to find if Bob is in contact with any of her contacts. This PSI process takes $2\dot\delta$ delay. If there is a mutual friend, they share the verification bundle, which takes $\delta$ time. If the verification bundle is outdated, it takes an additional $3\dot\delta$ time to get an updated verification bundle. So, the maximum delay the detection can take is $6\dot\delta$.  \\
    
    
    % \ahc{that doesn't seem to match the claim of the lemma! }
\end{proof}


%  Suppose the key in the database for the new contact is outdated (key upload timestamp of the database key does not match with key retrieved from the server), and the mutual contact is offline to verify the latest key. In that case, it can take longer to detect the attack. Until then, the contacts are marked as neutral and can be verified using monitoring.

\ahc{I'll stop reading this section here since already the scheme as described so far (the simpler version) appears complex and problematic, and since I can't see the motivation: this doesn't seem compatible with existing servers, so what's the advantage over KT? }


\subsection{Key monitoring through a proxy}

% \ks{Thinking about terminology. Not sure I like relay of contacts. Considering terms like "forwarding a request through a series of contacts", random forwarding, ForwardingCount. Instead of "relaying the requests" we could say "forwarding the requests".  "relay key monitoring" change to "forward key monitoring", don't like that change. Maybe instead "Alice uses forwarding to monitor her own key"? Or maybe "Alice forwards key requests to monitor her key". Maybe the 6.2 section title should be "Key monitoring using forwarding".} \tarun{Let's use forwarding if you prefer that. The actual meaning we need here is that we are forwarding/relaying request to a client who makes the request. And I think either term should be fine. Let me know if you agree and I'll replace it.}
% \tarun{Last client who makes a request: use that as "proxy"  and use term "relaying the request to proxy.". the proxy position makes the request to the server indistinguishable.}

Clients monitor their keys, keys of new contacts, and key updates of existing contacts. 
Monitoring requests are not sent directly from Alice to the server because the server can more easily launch fake key attacks when it knows the identity of the requestor. 
Instead, Alice forwards her request through a relay of contacts to a random client that acts as a proxy and sends her request to the server. 
To prevent the tracking of monitoring requests by the \acrshort{ms}, Alice also sends a random-sized dummy monitoring message to all her other contacts in every epoch.
The design of our approach makes it difficult for the server to determine the origin of a monitoring request, and it is highly unlikely that the server can equivocate (i.e., provide a different key in response to requests for the same identifier) without being detected.

\paragraph{Relay key monitoring request to a proxy}
To monitor Bob's key for an epoch, Alice generates a random session key, concatenates it to Bob's identity, and encrypts the resulting string using the server's public key so that relays do not learn which key Alice is monitoring.
The \texttt{Identity} is the identifier (\eg~phone number) for the user. 
The server uses the \texttt{SessionKey} to encrypt its response so it is kept confidential between Alice and the server. A malicious client does not learn the origin of the request and thus cannot block only responses destined for a specific client. A random symmetric key does not reveal Alice's identity to the server.

\ahc{This seems problematic. 1. it seems quite likely that a request may reach  a corrupt client that cooperates with corrupt server, and may be able to deanonymize and return wrong value. 2. the anonymity here seems to be completely vulnerable to eavesdropper. 3. overeall the design is basically of an anonymous relay; why re-invent it? just use AKM! 4. what's to prevent a rogue client from dropping the requests it receives from peers?? in fact, what's motivating clients to spend their resources relaying requests? 5. what about DoS abuse? so again I'll quit reviewing rest of this section. }

\begin{align}
	KeyReq = Enc(K_{ServerPubKeyEnc}||Identity||SessionKey)
\end{align}

Next, Alice generates a monitoring request that includes the key request just described and \texttt{RelayCount}, which is the total number of hops the request is forwarded before a relay sends the monitoring request to the server.
% a, and (2) \texttt{RelaySet} contains $n$ random indices indicating at which hops along the forwarded requests will $n$ relays send the monitoring request to the server on behalf of Alice.

\begin{align}
    	MonitoringReq = ReqId||KeyReq||RelayCount
\end{align}

Suppose Alice sends the monitoring request to one of her contacts, Carol. When Carol receives this message, in the next epoch, she decrements \texttt{RelayCount} and, if it is still greater than zero, selects a random contact to forward the request to. 

\paragraph{Proxy retrieves key}
When a client receives the request with a \texttt{RelayCount} value of 1, they act as a proxy for that request, send the embedded request to the server and relay the \texttt{Response} back to Alice. If every client makes a monitoring request through a proxy that is at least $diam(G)$ hops away from them, the \acrshort{ms} cannot determine the origin of the monitoring request since the relayed request could have originated from any client in $G$. Therefore, a client acts as a proxy only after a request is relayed $diam(G)$ times. Thus, $RelayCount\geq diam(G)$.

% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.48\textwidth]{images/PostKeyRetrieval.pdf}
% 	\caption{Contact acts as a relay (for existing connections): Alice randomly selects one of her contacts (Carol) and sends an sealed sender key retrieval request for Bob's key bundle. Carol, after some delay, relays the request (as a sealed sender) to one of her contact Ed  and so on. The last relay would ask the server for Bob's key bundle and relays the response back to Alice (as sealed sender request).}
% 	\label{fig:PostKey}
% \end{figure}


% When Carol receives this message, in the next epoch, she decrements the \texttt{RelayCount} and, if it is still greater than zero, selects a random contact to forward the request to in. If she chooses a new contact David, then she forwards the $MonitoringReq$ that is now encrypted with a shared symmetric key she shares with David. \ahc{I don't think we've setup (or used) such symmetric keys so far. }

% When a relay receives the monitoring request and current \texttt{RelayCount} is in \texttt{MonitoringRelaySet}, then the relay sends the embedded request to the server. The server's response is:

% Since a relay may be offline at any moment, a client may take multiple epochs to forward the request. A relay that is online either appends the monitoring request with the regular message or selects a random time in the epoch to forward the request. From previous research, the probability that a disconnected interval for a device lasts for less than one day is 0.998. Therefore, if epochs are one day long, all clients will likely be online for at least some duration in the epoch. \ks{This is the same .998 mentioned in section 3. Probably refer back to that assumption rather than repeat the data here.}


\paragraph{Relay key monitoring response back to Alice}

\begin{multline}
	Response = ReqId||Sign(K_{ServerPrivKeySign},\\Enc(K_{SessionKey},KeyBundle_{Bob}||\\VerificationBundle_{Bob}))
\end{multline}


The $Response$ is relayed back along the same path used for the request, one hop per epoch. To achieve this, clients maintain a table of all requests that contains $ReqId$, $cameFrom$ and $forwardedTo$. When a client receives a response, it forwards it to the $cameFrom$ client and removes the entry.

The server signs the request so that it cannot be tampered with or falsified by a malicious client. Encrypting the response with  \texttt{SessionKey} ensures confidentiality between the server and Alice. If Alice sends a monitoring request for a contact's key to $n$ proxies and does not receive a response from at least $n/2$ proxies, it considers it as an attack. The threshold of $n/2$ proxies helps to ensure that Alice does not get a false positive because of a few malicious clients in the system. A malicious client is one of the relays or proxies in the monitoring process, and they can try to interfere with the monitoring process by dropping a request/response.

Alice uses proxy key monitoring to monitor her own key, new contact's key, and a key update. If Alice wants to monitor a key for $n$ epochs starting at epoch $e_1$, she initiates a monitoring request for every epoch from $e_1$ to $e_1+n$ epochs. The requests flow through the graph $G$ for diam(G) epochs before being sent to the server, and the response flows for diam(G) epochs before being received by Alice. Therefore, the monitoring responses are received by Alice in epochs $e_1+2\cdot diam(G)$ through $e_1+n+2\cdot diam(G)$.

\begin{theorem}
If the \acrfull{ms} sends a fake key for client $i$ to $c$ contacts during an epoch, then client $i$ detects the attack within $2.(diam(G)+n)$ epochs with probability $1- (1/(c+1))^{n/2}$, where $n$ is the number of monitoring requests from each contact following a key update. 
\end{theorem}

\begin{proof}
Clients monitor their key every epoch and monitor any new/updated contact's key for $n$ epochs. If the \acrshort{ms} presents a fake key to a client Alice for her contact Bob, it has to present the correct key to Bob when he monitors his key and a fake key to Alice for all $n$ of her monitoring requests. 
The monitoring requests from both Alice and Bob are first relayed through $diam(G)$ relay nodes before a request is sent to the server. Once Alice starts monitoring, it takes $n$ epochs for her to send all of her relay monitoring requests, up to $2\cdot diam(G)$ epochs for her to receive the first monitoring response, and up to $2\cdot diam(G) + n$ epochs for her to receive the last monitoring response. As $diam(G)$ is the maximum distance that is required to reach from a client to any other client in the network; therefore the \acrshort{ms} cannot distinguish between the monitoring request from the owner (Bob) and the contact (Alice) based on the position of the proxy client in the network. A request could have originated from any other client in the network. Therefore, the probability of correctly predicting the request is $1/2$. If $c$ contacts, including Alice, receive key updates for Bob, they monitor Bob's key, and the server has to present the real key to Bob and fake keys to Bob's $c$ contacts. There are $c+1$ possible combinations of giving a real key to 1 client and $c$ fake keys to the remaining clients. Thus, if Alice receives a response from at least $n/2$ proxies, the probability of detecting a fake key distribution is $1-(1/(c+1))^{n/2}$.

In case Alice does not receive a response from at least $n/2$ proxies out of $n$ proxies, Alice considers it as an attack. Therefore, the attack is detected within $2\cdot diam(G) + n$, which is the maximum time the last response takes to come back from the $n^{th}$ proxy.
\end{proof}

% \tarun{Add details of mutual contact if timestamp mismatch}
% \tarun{mutual contact: server give Bob's fake key to Alice for timestamp t1, contacts do not send update but give new key update for t2 for Bob. how we handle? }

==> Defense_TN_Old.tex <==


\section{Trust Network Defense (Old)}
\label{subsec:TN}

\ahc{rephrased this parag.}
The KT and AKM defenses both require adoption and involvement by the service provider. In contrast, the Trust Network (TN) defense is designed for client devices to automatically verify keys on their own, using only the existing secure messaging infrastructure, i.e., without any support from the service provider. 
%In contrast to the first two defenses, TN requires no new third-party infrastructure.
\st{This applies to the current situation, where a new client application could be designed with additional functionality, using the existing central server of the messaging company.}

The basic idea of the TN defense is that Alice uses a set of \textit{trusted contacts} to verify whether they have the same key for Bob that she received from the server. Trusted contacts are those contacts whose keys Alice has previously verified with this method.
Alice automatically verifies the authenticity of Bob's public key with these trusted contacts whenever she
receives Bob's public key from the server, either for a new contact or a key update.
This defense is able to \emph{prevent} some attacks and \emph{detect} all of them.
% It requires Alice to trust the key for her first contact until she has other contacts to assist with key verification.

The deployment benefit of no new infrastructure comes with a privacy cost because TN leaks mutual friends information. 
%\st{As an example the linkedIn shows shared connection and in their documentation it says \textit{"No matter which setting you select, your 1st-degree connections will always be able to see shared connections."~\cite{linkedinHelp}.}}

\ahc{I think we can adopt a different assumption / justification. Assume that a user identifies its friends by `nicknames', 
which are {\em shared} with one (or some threshold) shared-friends. 
I think this is a very common situation. So we can't identify a specific person such as Alice Smith or Bob Jones by a globally-unique name - I bet these are not unique - but if we're both their friends, we may know that these are Alice and Bob when we communicate btw us. Right? Now, I think it is likely that {\em all} persons are connected in this way - and, for a popular messaging platform, this even holds considering friends on same platform. I think that's all we need! BTW, this concept is a bit similar to the `petname' concept proposed ages ago, maybe some of the old-timers remember it (and I guess Google scholar surely remembers it).  }
\tarun{TO DISCUSS}



% \tarun{The new attack vectors on TN defense introduces a new adversary A2. The following section explains the new adversary model, the TN design, and security analysis.}


% \paragraph{Adversary model (A2)}
% \tarun{Adversary A2 has control over at least one of the Alice's friend's client or has one of her friend's long-term private identity Key. The adversary A2 doesn't have any control over the server. A2's goal is to 1) identify all Alice's friends and 2) disrupt the communication of the friends of the compromised client. (by using false attack alerts)}


{\noindent\bf Assumptions}

\begin{enumerate}

\item Every client has at least one secure connection\ahc{define!}. The mass key update monitoring heuristic ensures that $A_1$ cannot compromise all clients within a short duration and isolation monitoring ensures that every client can communicate with at least one connected secure edge. Together, these heuristics ensure that every client is able to communicate securely with at least one other client. \ahc{separate assumptions from justifications}

\item A client (Alice) can send an {\em anonymous verification message} to another client (Bob) via the server where the server learns only the recipient but not the sender. 
This assumption matches the {\em sealed sender} capability recently added to the Signal protocol~\cite{ndss2021}. 
The adversary $A_1$ does not learn the sender's identity from the application layer data \st{or the sender's IP address from the network layer.}
\ahc{this seems like a pretty major assumption on the server to me - which contradicts the goal of no support by the server.}

\item The server has a long-term public key that is made available to clients during registration with the service when the app is installed. The purpose of this key is to sign public keys before delivering them to clients so that clients can reliably share and compare public keys they receive and trust that they are from the legitimate server.
\ahc{again an assumption about the server... }

\item The server supports a push-based key distribution model. When Alice's key changes, a key update is pushed to all of Alice's contacts. \ks{Can we give example of a current system that does this? Didn't Devashish once say that WhatsApp pushes keys to clients?} \ahc{another assumption...}

\item We assume that enough clients are behind the NAT to it infeasible for the server to deanonymize the sender conclusively based on the IP address. Many ISPs across the globe have deployed Carrier-grade NAT (CGN) devices~\cite{livadariu2018inferring, rytilahtiusing}. Ritchter et al.~\cite{richter2016multi} reported that CGN deployment is ubiquitous in cellular networks, with more than $90\%$ of all cellular ASes deploying CGNs. Thus, in a well-established social network, many users are likely behind the same NAT device. \ahc{true, but it's another - huge - assumption. Specifically, most NATs are cone-NATs which means that the server usually would be able to trivially identify the client (if it also communicates to it in non-anonymous manner, which is necessary). }
\end{enumerate}

% {\noindent\bf Anonymity of Verification Messages }
% We assume adversary $A_1$ cannot deanonymize the sender's identity at the IP layer from a verification message. Currently, deanonymization based solely on IP addresses may lead to inaccurate inferences because many ISPs across the globe have deployed Carrier-grade NAT (CGN) devices~\cite{livadariu2018inferring, rytilahtiusing}. Ritchter et al.~\cite{richter2016multi} reported that CGN deployment is ubiquitous in cellular networks, with more than $90\%$ of all cellular ASes deploying CGNs. Thus, in a well-established social network, many users are likely behind the same NAT device, making it hard for $A_1$ to identify Alice among other NAT clients accurately.

% Anonymity could also be achieved by using a popular VPN or an anonymizing proxy such as Tor [45], [19]. For this paper's purposes, we assume that users who wish to remain anonymous to the provider can use such proxies (e.g., Orbot [2]) for verification messages. \ks{Doesn't this contradict our first statement that TN does not rely on 3rd party infrastructure?} In terms of impact, we note that a recent study suggests as many as 15\% of mobile users already use VPNs every day [28]; this prevalence is even higher in east Asia and, presumably, among vulnerable user populations. 

{\noindent\bf Adversary Model}
Adversary $A_1$ is still the primary adversary that TN is designed to defend against.
Since TN adds new messages between clients to detect fake key attacks, this introduces the risk of a new adversary $A_2$ that controls Alice's client or has compromised her long-term private key. $A_2$ can intercept or inject messages on Alice's client. $A_2$ does not control the server. 
$A_2$'s goals are to 1) identify Alice's contacts' contacts, and 2) give false attack alerts to Alice's contacts. \ahc{this A2 adversary isn't clear to me. }

To defend against adversary A2, TN ensures that Alice's contacts cannot falsify Bob's keys by having  the server sign each key that it distributes to clients. \ahc{huge assumption; does it hold for current services? if it does (which I doubt), I think it may allow a better solution (avoiding these anonymity assumptions - esp. problematic on the server). 
One way would be to use separate, independent key-validation server(s) that a client can contact anonymously to confirm the (server-signed) pk for any client, where a conflict is a PoM against the service provider. So this is like the AKM just w/o the change to the server. In fact I think I can further improve this to even work without the signatures by the service provider (providing only prevention/detection, no PoM, though), by using `attestations' from `trusted friends' for each entity. We can discuss. 
}
Whenever a client requests a contact's public key, the server responds with a signed public key and a signed \textit{verification bundle}.
The verification bundle contains the hash of the identity (\emph{e.g.} phone number) of the contact, the hash of the contact's public key, and a timestamp that indicates the time at which Bob pushed his public key to the server.
Clients can't forge or replay these verification bundles, and their purpose is to detect equivocation.

% \tarun{TAKEN FROM OTHER PAPER(NDSS 2021): Can we use it for TN approach? We note that the service provider could infer a sender’s identity from network metadata such as the IP address used to send a sealed sender message. However, this is a problem that could be solved by using a popular VPN or an anonymizing proxy such as Tor [45], [19]. For the purposes of this paper, we assume that users who wish to remain anonymous to Signal can use such proxies (e.g. Orbot [2]) when sending sealed sender messages (and, in our solution, when receiving messages to ephemeral mailboxes), and we do not use network metadata in our attack. In terms of impact, we note that a recent study suggests as many as 15\% of mobile users already use VPNs every day [28]; this prevalence is even higher in east Asia and, presumably, among vulnerable user populations.}

% \ks{Will this become the justification for the requirement here that we assume adversary cannot correlate layer 3 packets? We can make this connection and cite the NDSS paper for the idea.}
% \tarun{Yes! That's the plan.}







%\st{To initialize this set, Alice can perform manual key verification with several contacts.} \ks{NOTE: I think we should remove this prior sentence and discuss the issue in the security analysis. If the network is not compromised, the first fake key attack can be detected. What if Alice has no other contacts? She can either trust on first use or do the key ceremony. I don't think t works for most users to assume they will conduct the ceremony so I think a TOFU approach is also possible.} \tarun{agree with it.}

% \tarun{In some situations, the attack detection could take longer in order of days or a couple of weeks. We believe even in these situations the TN could be of great value for most of the users who never do manual authentication []. One key point to note is that it's easy to detect when an MKS stops an attack and gives the correct key of the contacts as shown in ~\ref{subsec:KeyHist}. So, in general, our goal is to detect the never-ending attacks, and we believe it's better to detect an attack than never.}

%{\bf TBD/KS: Discuss in security analysis: If the network is not compromised, the first fake key attack can be detected. What if Alice has no other contacts? She can either trust on first use or do the key ceremony. I don't think it works for most users to assume they will conduct the ceremony so I think a TOFU approach is also possible.}
%\tarun{yes! TN doesn't helps in initial connection. We have to careful while explaining TOFU, such that readers don't misinterpret it as TOFU for all the keys.}
%\ks{If Alice has no contacts, when she adds her first contact she doesn't have a mutual contact to prevent the attack, nor any other contacts to request the key. She has to trust on first use. As contacts are added, she gradually gains the benefits of the TN approach. So a mutual contact added later can help her detect an earlier attack.}

%Later, when she wishes to establish a secure connection with a new user (say Bob), her client attempts to identify some trusted mutual contacts between Alice and Bob.
%If there exist some trusted mutual contacts between them, her client directly confirms from them, whether the received identity keys (of Bob) are correct.
%If there does not exist any mutual contact, she randomly selects any of her trusted contacts (\emph{e.g.} Carol) to ask for Bob's key on her behalf.
%If MKS was launching fake key attacks (\emph{e.g.,} pair-targeted attacks) only for Alice and Bob, MKS would present correct keys of Bob to Carol' client. Alice's client on receiving the correct keys from Carol' client, would detect that Alice is under attack.

% \paragraph{Malicious contacts}

{\noindent\bf How TN Works}
There are two mechanisms the Trust Network defense uses to verify keys:
(1) mutual contacts to prevent fake-key attacks, and 
(2) random contacts to detect fake-key attacks, 
In this section, we describe each mechanism along with a security analysis.

%\tarun{[Alternate 2] There are three mechanisms the Trust Network uses to verify keys---
%1) uses mutual contacts to prevents equivocation,
%2) uses random contacts as relays to detect equivocation,
%3) uses heuristics based on the server's malicious behavior to detect fake key distribution to everyone in the system.
%In this section, we describe each mechanism and provide a security analysis.}

%\ks{Looking over these two options. Is (1) more correct because it does prevent pair-targeted attacks so we should be specific? Or is it more general than that so equivocation is accurate?}
%\tarun{According to our threat model, Alternate 1 is more specific. ALternate 2 is trying to generalize.}

% TN \textit{assumes} that Alice already has few secure connection with some of her contacts (after she initially joined the app's network). Assuming there is a pair-targeted attack on Alice and Bob by the MKS --- when Alice requests Bob's identity key, the MKS responds with fake keys to impersonate Bob. Presently, apps relying on Signal protocol uses manual key verification (as already explained in Subsection \ref{}). However, with the trust network based approach --- Alice automatically queries her contacts\footnote{Only those clients are considered with whom she already has established E2EE connections.} to determine if they have the same identity key for Bob. If so, Alice assumes she is safe and not under attack.
%We now describe our Trust Network defense strategy in detail \dev{(along with the use of Verification bundle)}.

% \noindent \textit{Assumption}:
% We assume that, a user's few initial E2EE connections would be secure after they join app's network.
% We suggest users resorting to manual key verification to have such secure E2EE connections.\\
% With few secure E2EE connections apriori, TN can defend against fake key attacks as follows:


% \noindent \textit{The Trust Network Approach}:

\subsection{Mutual Contact}
\label{mutual_contact}

\ks{I think we should modify Figs 4-5 to be generic and not use Signal terminology. Change Sealed request to anonymous request, change key bundle to verification bundle.}

Whenever Alice starts communicating with a new user Bob, he sends Alice all of his contacts' verification bundles. The bundles provide Alice the hash of the identifier and public key of all of her two-hop contacts (her contacts' contacts), as shown in Figure \ref{fig:MutualFriend}.
\dev{Dev: Why we selected only two hop contacts for storing verification bundles? If we go upto 'n' hops the detection probability will increase. I guess the reason is trade-off between database increase and detection probability. I think, we can briefly mention about this trade-off here and discuss later in the \S\ref{subsec:compare}. Moreover, if Bob is sending not only his contacts, rather its contacts' contacts to Alice, privacy leak could be reduced as well. It would become hard for Alice to distinguish among the received contacts from Bob, who are mutual contacts with Bob.}
\tarun{By two-hop, we mean friends' friend. We already have keys for one hop (i.e., direct friends of a client). Yes, in the end, we can explain that the clients can go 3; it would prevent privacy issues and could be more preventive but would take more space.}
%Alice can then compare the hashes of the identity keys of her contacts with those in the received verification bundles, identifying mutual contacts.

The hash of the identifier prevents a client from knowing their friend's complete friends list. The client can only know about the mutual friends it has with their friends by comparing the hashes it receives with the hashes it has.

\begin{figure}
	\centering
	\includegraphics[width=0.4\textwidth]{images/Mutual_Contact_Updated.pdf}
	\caption{Mutual Contact: (1) Alice's contacts share the verification bundle of their contacts with Alice. She maintains a database of her contacts' contacts verification bundle. (2) Alice queries the server for Bob's key. The server responds with Bob's verification bundle. Alice compares the two set of keys (\emph{i.e.,} 1 and 2). If a mismatch is found, an attack is prevented.}
	\label{fig:MutualFriend}
\end{figure}

Alice maintains a database that contains the verification bundle of her two-hop contacts.
Whenever Alice obtains a key update message from the server (a push notification) regarding Bob, she sends a \textit{database update message} to all her contacts with a new verification bundle for Bob. Assuming all clients do this, Alice can maintain the latest verification bundle of her two-hop contacts.

\begin{theorem}
    If $A_1$ delivers a fake key update for Bob's key to Alice, and they share a mutual contact Carol that is not under attack by $A_1$, Alice can immediately determine the key is fake and prevent the attack.
\end{theorem}

\begin{proof}
To check whether a fake key attack is in progress, Alice compares the hash of Bob's identity to the hashed identity keys in the verification bundles in her database. Assume they share a mutual contact Carol. Now Alice compares the timestamp (t1) and the hash of the key from Bob's verification bundle that Carol sent with the timestamp (t2) and the hash of the key provided by server. If they match, Alice trusts the key; if timestamp t1 is equal to or greater than t2 but there is a key mismatch, a fake key is detected  else, if timestamp t1 < t2, Alice contacts Carol for an updated key verification for Bob.
\end{proof}

\begin{lemma}
If $A_1$ delivers a fake key update for Bob's key to Alice, and they share a mutual contact Carol, the only time Carol is unable to confirm Bob's valid key for Alice is when $A_1$ is impersonating Bob to all his friends. When that happens, isolation monitoring will detect the attack.
\end{lemma}

\begin{proof}
Given a system that is not under attack from the beginning, $A_1$ can launch a pair-targeted attack on Alice and Bob, or launch a client-targeted attack on Bob. In the case of a pair-targeted attack, their mutual contacts will have their correct keys to compare to to prevent the attack from succeeding. In the case of a client-targeted attack where $A_1$ impersonated Bob to all of his contacts, all of Bob's contacts, including any mutual contacts with Alice, will also have the fake key from $A_1$. The TN defense cannot detect or prevent that attack. It will be detected by the isolation monitoring heuristic when Bob discovers he cannot communicate with any of this contacts because
\end{proof}

% \st{There is no data available from current secure messaging systems
% to determine the probability that two  users share a mutual contact.
% To gain insight into this question, we analyzed a Facebook dataset[], explained in []. We found that an average user has at least one mutual friend for 59 percent of their connections, and the average number of mutual friends is 4.46.}

%The database update message contains:
%   \begin{multline}
%       Verification\_bundle_{Contact1}:\\Verification\_bundle_{Contact2}:\\Verification\_bundle_{Contact3}...
%   \end{multline}

%        %\textcolor{brown}{(Add keys from 2 level of contacts.)}
%        Here Alice sends a standard key retrieval request to the MKS represented as ``\textit{Request}''. MKS responds with a standard response, which has Bob's key bundle, represented as ``\textit{Response}''.

%        \begin{equation}
%            Request: request
%\end{equation}

%       \begin{multline}
%            Response: Key Bundle_{Bob} ||\\ Verification Bundle_{Bob}
%        \end{multline}


\subsection{Random Contact}

If Alice does not have a mutual contact with Bob, her client randomly selects any one of her contacts, \textit{e.g.} Carol, to act as a proxy for her. Alice asks Carol to obtain Bob's verification bundle from the server on her behalf.
Carol may relay this request to additional random contacts.
Once Alice receives a key from a relay, Alice compares this key with the one provided directly by the server. On successful match, Alice trusts the key, otherwise an attack is detected.

\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{images/PreKeyRetrieval.pdf}
	\caption{Contact acts as a relay (for new connections): Alice randomly selects one of her contacts and sends an encrypted key retrieval request for Bob's key bundle. The contact relays the request to the server and relays the response back to Alice.}
	\label{fig:PreKey}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{images/PostKeyRetrieval.pdf}
	\caption{Contact acts as a relay (for existing connections): Alice randomly selects one of her contacts (Carol) and sends an sealed sender key retrieval request for Bob's key bundle. Carol, after some delay, relays the request (as a sealed sender) to one of her contact Ed  and so on. The last relay would ask the server for Bob's key bundle and relays the response back to Alice (as sealed sender request).}
	\label{fig:PostKey}
\end{figure}

\subsubsection{Basic Mechanism}

When Alice needs to retrieve Bob's keys from a contact, her client generates a new \texttt{SessionKey} that it appends with the request, then encrypts this combination with the public key\footnote{When we refer to encrypting with a public key, we mean encrypting with a symmetric key and then encrypting the symmetric key with the public key.} of the server:

\begin{align}
	Request = Enc(K_{ServerPubKey},Identity||SessionKey)
\end{align}

The \texttt{Identity} is the identifier (\eg~phone number) for Bob. The request is encrypted with the server's public key so that relays do not learn who Alice is communicating with. The server will later use the \texttt{SessionKey} to encrypt its response so the response is also kept confidential between Alice and the server. A symmetric key does not reveal Alice's identity to the server.

%\todo{Devashish: I feel the SessionKey requires more explanation. DZ: Can you clarify what you feel needs more explanation?}

%\textcolor{magenta}{In any case the Request is being encrypted by the $KS_{PubKey}$; in one sense confidentiality is being achieved at this step also. However when last hop would receive the response from the MKS, in absence of session key, he could infer the contact with whom Alice wishes to communicate. We are providing confidentiality to the response from \textbf{only the last hop.}....If its obvious we can ignore this.}

%DZ: I think I clarified this well enough.

Next, Alice's client sends the request anonymously to one of her contacts so that the server only knows the recipient's identity and not the sender's identity.
The way that Alice sends this request depends on whether Bob is a new connection or an existing connection.

\subsubsection{New Connections}

For new connections, Alice's client first sends this request to Carol, and Carol retrieves Bob's keys from the server and then relays them to Alice. After this, Alice's client requests Bob's key directly from the server and compares keys (shown in Figure \ref{fig:PreKey}).
%  \begin{multline}
%       \textbf{Sealed\hspace{1mm}Request:}\\Enc(Enc(request||SessionKey)_{KSPubKey}\\||identity)_{Key\_Alice\_Carol}
%  \end{multline}
%  \begin{multline}
%   \textbf{ Response\hspace{1mm}to\hspace{1mm}Carol:}\\
%     Enc(Enc(KeyBundle_{Bob}||\\Verification\_Bundle_{Bob})_{SessionKey})_{KSPrivKey}
%   \end{multline}
%   \begin{multline}
%   \textbf{Response\hspace{1mm}to\hspace{1mm}Alice:}\\
%     Enc(Enc(Enc(KeyBundle_{Bob}||\\Verification\_Bundle_{Bob})_{SessionKey}\\)_{KSPrivKey})_{RelayKey}
% \end{multline}


\subsubsection{Existing Connections}

% \tarun{[]I think we can mention here that contact relay would work effectively on existing connection when the delay is in order of days or weeks.]}

% \tarun{One fact to note is that the response of the contact relay is sealed sender, so KS would not be able to differentiate between a contact relay request/forward/response.}



When Alice has an existing connection with Bob, then she may receive a key update message from the server. Alice needs to have some other client request Bob's key as well, so she can verify it, but this needs to be done without the server being able to correlate that this client is asking on behalf of Alice.
Thus, Alice sends a request to Carol for Bob's key, as above, and also includes additional metadata:
\begin{align}
    	Request||Identity||RelayCount||RelayKey
\end{align}
% \begin{multline}
% 	Request||Identity||RelayCount||RelayKey
% 	%   Enc(K_{Alice\_Carol},Enc(K_{KSPubKey},request\\||SessionKey) ||Identity||RelayCount||RelayKey)
% \end{multline}
Here, \texttt{Identity} is the identifier (\eg~phone number) of Alice, \texttt{RelayCount} is the number of relays to use, and \texttt{RelayKey} is a symmetric key to use for encrypting the response.

When Carol receives this message, she decrements the \texttt{RelayCount} and, if it is still greater than zero, selects a random contact to forward the request to. If she chooses a new contact David, then she forwards the message that is now encrypted with a shared, symmetric key she shares with David. At each hop between relays the message is sealed by the sender. Since a relay may be offline at any moment, this process may incur delay on the order of hours or days. A relay that is online adds some random delay to prevent the server from being able to correlate the timing of the messages and determine the request is from Alice.

Once the \texttt{RelayCount} reaches zero, then last recipient sends the embedded request to the server (as shown in Figure \ref{fig:PostKey}). The server's response is:
\begin{multline}
	Response = Sign(K_{ServerPrivKey},Enc(K_{SessionKey},\\KeyBundle_{Bob}||VerificationBundle_{Bob}))
\end{multline}
The server signs the request so that it cannot be tampered with or falsified by adversary $A_2$. The \texttt{SessionKey} ensures confidentiality between the server and Alice. Upon receiving a response, that client forwards the response to Alice using an anonymous verification message:
\begin{align}
	Enc(K_{RelayKey},Response)
\end{align}

Here we assume that any client can send a message to another client without having to establish an end-to-end connection. This allows a relay to send the response to Alice without having to first establish a connection, and avoids a recursive key validation problem.
\st{By also using sealed sender, the server is not able to know who is communicating with Alice.}

%she would first request MKS for Bob's key bundle and later she asks Carol to relay her sealed request to the next relay. In turn, Carol would select (her contact) Ed as a relay and the process continues. \textit{All these messages are sealed by the sender and at every relay change considerable amount of delay is added (in hours/days)}.
%    Now the last relay would retrieve the Bob's key on behalf of Alice.
%    Post-key retrieval is used when Alice's client has an established E2EE connection with Bob's client and her client received a key update notification from MKS.\\


%    In post-key retrieval, Alice's client appends some additional information in the sealed message.
%that is sent to Carol's client
%    --- a number \textit{RelayCount} and a new session key \textit{RelayKey}.
%    \textit{RelayCount} is a counter that depicts the total number of relays that the sealed message would be forwarded to. Every relay would decrement its value by one. The relay for which its value reaches zero (the last relay), would ask the MKS for Bob's key bundle on behalf of Alice.
%    After obtaining the key bundle, the last relay would use the \textit{RelayKey} to seal the message and sends it to the Alice as a sealed message. \\


%    Finally the sealed request that Alice sends to her relays can be represented as:
%     \begin{multline}
%          \textbf{Sealed\hspace{1mm}Request:}\\Enc(Enc(request||SessionKey)_{KSPubKey}\\||identity||RelayCount||RelayKey)_{Key\_Alice\_Carol}
%    \end{multline}
%    The last relay would send a standard key retrieval request to the key server \emph{i.e.}
%     \begin{multline}
%          \textbf{Request\hspace{1mm}to\hspace{1mm}MKS:}\\Enc(request||SessionKey)_{KSPubKey}
%    \end{multline}
%    On reception of key server would encrypt the response with the session key that was embedded in the request. It sends the encrypted response to the last relay.
%   \begin{multline}
%      \textbf{ Response\hspace{1mm}to\hspace{1mm}last\hspace{1mm}relay:}\\
%       Enc(Enc(KeyBundle_{Bob}||\\Verification\_Bundle_{Bob})_{SessionKey})_{KSPrivKey}
%   \end{multline}
%   Finally, the last relay would forward the MKS response to Alice as a sealed message.
%   \begin{multline}
%     \textbf{Response\hspace{1mm}to\hspace{1mm}Alice:}\\
%       Enc(Enc(Enc(KeyBundle_{Bob}||\\Verification\_Bundle_{Bob})_{SessionKey}\\)_{KSPrivKey})_{RelayKey}
%   \end{multline}

%\subsection{Design Choices}

We use multiple relays for existing connections to avoid timing attacks by $A_1$. Without this protection, $A_1$ could send a fake key update to Alice, then watch for a message from Alice to a relay Carol, followed by Carol asking for Bob's key bundle. All of these messages would occur within a short time period and all pass through $A_1$. This would allow $A_1$ to present a fake key bundle to Carol's client, thwarting the defense. By adding multiple relays, with a random delay incurred at each step, it is more difficult for $A_1$ to correlate that the last relay is asking for Bob's key bundle on behalf of Alice.

\begin{theorem}
    If $A_1$ delivers a fake key update for Bob's key to Alice, and none of Bob's other contacts are under attack, Alice will detect the attack using another contact as a relay.
\end{theorem}

\begin{proof}
If none of Bob's other contacts are under attack, $A_1$ is conducting a pair-targeted attack against Alice and Bob. Everyone else except Alice will be given Bob's valid key. When Alice's contact requests Bob's key, they will be given Bob's valid key and return it to Alice. Alice will detect that she was given a fake key.
\ks{We may need to argue the chance of the server guessing when Alice's contact is requesting Bob's key is negligible.}
\end{proof}

\begin{lemma}
If $A_1$ delivers a fake key update for Bob's key to Alice, the only time Alice is not able to detect the attack using her other contacts as a relay is when $A_1$ is attacking all of Bob's contacts. In this case, Alice's contacts will request Bob's key and be given the fake key instead. 
When this happens, isolation monitoring will detect the attack.
\end{lemma}

\begin{proof}
Given a system that is not under attack from the beginning, $A_1$ can launch a pair-targeted attack on Alice and Bob, or launch a client-targeted attack on Bob. In the case of a pair-targeted attack, any of Alice's contacts that request Bob's key will receive Bob's valid key and return it to Alice, who will detect the attack. In the case of a client-targeted attack where $A_1$ impersonates Bob to all of his contacts, any of Alice's contacts that request Bob's key will receive the fake key and return it to Alice, who will not detect the attack. The TN defense cannot detect or prevent that attack. It will be detected by the isolation monitoring heuristic when Bob discovers he cannot communicate with any of his contacts because $A_1$ is impersonating him to all of his contacts.
\end{proof}

%Our design raises several questions --- in sealed request, why we include a SessionKey, why we require assymetric key pair for key server and why we use multiple relays in post key retrieval \emph{etc.}
%We now explain our the rationale behind our design choices.\\

%\noindent \textbf{Use of multiple relays in post key retrieval:}
%\label{subsec:MultipleRelays}
%Post-key retrieval might be susceptible to a timing correlation attack by MKS.
%(1) MKS sends a fake key update to Alice. (2) Next, Alice sends a sealed message to Carol. (3) Later, Carol asks MKS for Bob's key bundle.
%All the three messages are relayed via the MKS; additionally MKS has a complete information about who are the Alice's contacts. Even if the message from Alice's client to Carol's client are sealed, still a determined MKS can observe a correlation in the aforementioned messages and might present fake key bundle to Carol's client.
%Thus, to defend against such attacks we need to obfuscate the previous message patterns.
%To do so, Alice's client involves multiple other users' clients as relays, which forward the Alice's client's initial message.
%All these messages are sealed by the relay
%and at every relay change considerable amount of
%delay is added (in hours/days). Now the last relay
%would retrieve the Bob’s key on behalf of Alice
%This would make it extremely difficult for MKS to correlate that the last relay is asking for Bob's key bundle on behalf of Alice.\\

%\noindent \textbf{Use of asymmetric key pair by the key server:}
%As already described, both in pre and post key retrieval, Alice's client's key retrieval request its response from key server are served by other users' clients.
%It can be argued that other user could be malicious. He can present Bob's fake key to Alice to annoy her with false ``attack warning''. To thwart this situation,
% the key server generates a long-term asymmetric key pair and sends the public key to the clients at the time of registration.
%the key server signs the key retrieval response with its private key.
%Whenever Alice retrieves Bob's keys from Carol, she first verifies the key server signature with corresponding public key (of the key server) she owns. This prevents her malicious contacts from presenting a fake key.\\


%\noindent \textbf{Use of SessionKey in sealed request:}
%Since the key retrieval response to Alice's client comes from a some other user's client (say Carol),
%Carol can identify with whom Alice would communicate by reading the Alice's request or Key server's response. Henceforth,
%When Alice would relay her query via Carol, she would first generate a session key at her end only. Next, she would append the session key with the request $(request||SessionKey)$ and eventually encrypting it with public key of the key server.
%When Carol would relay this encrypted message to key server, she could not decrypt it. However, key server can successfully decrypts it. In return, key server would encrypt the response with the session key that was embedded in the request.
%This would prevent Carol from deciphering the response.

% \textit{In order to make relay request indistinguishable from normal request, all the Signal clients would include a self-generated session key in normal requests for key bundle as well}.
% \textcolor{olive}{Alternate: Direct key retrieval requests is also done in a similar way($Enc(request||SessionKey)_{KSPublicKey}$) as relay key retrieval requests to make them indistinguishable.}





% \noindent\textbf{\textit{Assumptions:}} (1)
% % We assume there are few initial secure connections for a user after joining the app's network.
% We first assume that, a user's few initial E2EE connections would be secure after they join app's network.
% % We assume a user would have few secure connections after joining the app network.
% % We assume there are few initial secure E2EE connections for a user who just joins the app's network.
% %When a user would join the app's network he would build few (atleast one) secure E2EE connections.
% We suggest users resorting to manual key verification to have such secure E2EE connections.\\
% (2) Moreover, we assume that MKS would refrain from dropping standard communication messages of non-victim app users.

% If MKS drops standard communication messages of multiple non-victim users. It could drop all the standard messages of Alice to all friends except Carol. Now, Alice is out
% % However, in extreme, it may drop few messages considering them potential verification messages by the app's clients.

% \input{Defense_heuristics.tex}




==> Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{Proof of an Attack}
\label{proof_of_attack}

The detection of conflicting \acrshort{str}s in the KT defense is the only case where there is \acrfull{pom}.
In all other cases, even though Alice and Bob have evidence that they are under attack, they cannot provide irrefutable evidence to a third party that the server is malicious. 
In these cases, Alice and Bob could be colluding to damage the reputation of the server. 
One approach to overcoming this limitation is for Alice and Bob to sign any key update with their previous key.
However, this introduces new challenges when their key is lost or compromised.
Thus, it is impossible to distinguish between an MKS that creates a fake key for Bob and a legitimate key change by Bob, who then falsely accuses the server of being malicious.

\subsection{User Notifications}
\label{user_notifications}
Secure messaging applications typically alert users whenever a key update occurs for one of their contacts. This alert occurs when a contact re-installs the messaging application, perhaps due to obtaining a new phone. 
The adoption of the defenses presented here would allow the option for key updates due to re-installations no longer generating an alert message. Fewer alert messages may be suitable for most users that are not a member of a vulnerable population. This would result in fewer alerts arriving, with greater confidence that an attack is in progress, providing new opportunities for tailoring alert messages to reflect the actual risk that the user is under attack. 
A redesign of the alert messages that would accompany the defenses presented in this paper is an open research challenge that deserves further study.


\input{Defense_heuristics}

%\ks{ Does Signal have to select one of the three defense and support it? Can the options co-exist? Does it still work if only part of the user base adopts it? We would have to decide on a pull or push model - you couldn't have both happening simultaneously, could you? Does the paper need to make a clear point about these issues?}



%\textcolor{teal}{Dev: Some thoughts...}
%\deva{
%As already mentioned (ref. Subsection \ref{subsec:compare}), different approaches have their own pros and cons, and thus can be deployed independently in different settings. Existing (or future) Signal based apps can use any of the three approaches for the automated defense. However, with respect to immediate deployment, among all the three proposed approaches, AKR can be deployed even if there is less participation from the Signal users. Assuming only Alice and Bob (who are friends with each other), would like to adopt an automated key verification scheme. With AKR, if only these two users adopt anonymous key monitoring and key retrieval, they can safeguard against the attacks. However, for TN and key transparency, we require cooperation from as many participants as we can. In TN, we require users to share their contacts information with each other; key transparency requires multiple users to be auditors etc.
%}




% \subsection{Exhaustion of one-time pre-keys}
% In our approaches, key bundle request is sent multiple times (for key monitoring). This might lead to exhaustion of one-time pre-keys in the bundle. To avoid such a situation there are two options: (1) Alice must periodically upload new one-time pre-keys to the key server or (2) she could generate a session key with only identity key and signed pre-key and (without using one-time pre-keys).
% In (1) there would be an undue burden on the client app and server app to periodically maintain the one-time pre-keys keys, whereas option (2) cannot ascertain complete security guarantees.
% Thus, in our design, we used the following approach: Initially Alice generates a session key based on only identity key and signed pre-key; encrypts the first message and send it to Bob. In the same message Alice piggybacks her one-time pre-keys to Bob. 
% Bob also generates a session key (same as Alice) based only on identity key and signed pre-key; decrypts the first message, obtains the Alice's one-time pre-keys. In the second message Bob also piggybacks his one-time pre-keys keys with the message and encrypts it using the initial session key. On reception, Alice decrypts the second message; obtains the one-time pre-keys keys of Bob. Now, both Alice and Bob, have each others all the three keys. They generate a new session keys and encrypt the further communication with the new key.
% [It must be noted that, one-time pre-keys are \textit{optional} by the signal protocol description itself. In the existing Signal protocol, if for Bob, key server does not have any one-time pre-keys left, key server would return Bob's identity key and signed pre-key only, as a key bundle. The session keys would be generated based on the aforementioned two keys only. However, in our proposed approach, except for the first two messages, all the subsequent messages would be encrypted the session key that has been generated from all the three keys.]

\subsection{Likelihood of false positives}

A false positive is the misclassification of a legitimate key update as a fake key attack. 
KT and AKR do not suffer from false positives.
In KT, the most recent STR reflects all key updates, so a legitimate key update cannot be mistaken for an attack. 
In AKR-basic, a key update is considered valid until anonymous monitoring reveals the server is equivocating. In AKR-advanced, a key update is reliably obtained for new or existing connections and confirmed by monitoring. Once a legitimate key change occurs, the owner's Tor hidden service becomes defunct and is replaced by a new service, so the old service cannot be a source of false positives.

However, false positives are possible with the Trust Network.
If Alice receives a valid key update for Bob, but all her mutual contacts with Bob are offline and most recently gave Alice Bob's old key, then this appears to be an attack. To prevent a false positive, Alice's client may need to wait to confirm the attack until she has a recent update from at least one of her mutual contacts whenever a mismatch occurs.
%If mutual contacts are online, then a Signal client verifies the key bundle provided by the MKS to the one obtained from mutual contacts or contact relays.
%In both cases, the keys a client retrieves have a timestamp associated with them, which is the time the user uploaded her key to the key server.
%The two sets of key bundles---one from the MKS and other from contacts, are considered a match if they contain the same timestamp value. Thus, it prevents false positives.
%\ks{What about when Alice gets a key update K2 for Bob, and her two mutual contacts are offline and have K1 as Bob's key in Alice's database? An attack is detected (false positive) when her mutual contacts are not online to immediately confirm the key change.}

%\textcolor{olive}{In this case the timestamp of K1 and K2 will be a mismatch, therefore Alice would not consider K1 for verification. }

False positives are also possible, though unlikely, with the mass key update and isolation monitoring heuristics since they assume Alice is under attack when multiple contacts update their key or there is no response from the server.

%\subsection{Exhaustion of one-time pre-keys}

%The addition of key monitoring to deter fake key attacks increases the number of key bundle requests, leading to an exhaustion of one-time pre-keys. One-time pre-keys are \textit{optional} in the  Signal protocol; clients will compute session keys using only the identity key and signed pre-key. The primary impact is to forward secrecy.  There are two options to address this: (1) Alice must upload new one-time pre-keys to the key server more frequently, or (2) Alice could send an additional one-time pre-key in a subsequent message and trigger renegotation of the secret key.


%It is important to note that one-time pre-keys are \textit{optional} in the  Signal protocol. If the key server runs out of pre-keys for Bob, the server returns only Bob's identity key and signed pre-key in the key bundle. When this occurs, the session keys are generated using only the two keys returned. 


%We propose a modification to Signal that leverages optional pre-keys. When Alice sends her first message to Bob she generates a session key based only on Bob's identity key and signed pre-key. Alice encrypts the first message using this session key and also includes her one-time pre-keys. Bob also generates a session key based only on an identity key and signed pre-key; this enables Bob to decrypt the first message and obtain Alice's one-time pre-keys. In his response, Bob also piggybacks his one-time pre-keys keys with the message and encrypts it using the first session key. Now, both Alice and Bob have three types of keys from each other and can generate subsequent session keys to encrypt their data according to the current protocol specification that provides forward secrecy. The session key in the initial one-round message exchange is unique and is not reused.

% \subsection{Pull vs Push based approaches}

% A popular messaging apps like WhatsApp (that has billions of users) have implemented Signal protocol with push based model \emph{i.e.} whenever a key server would receive a new key bundle for any signal user (\emph{e.g.} Alice) it would automatically send a key update message to all of Alice's contacts. In this paper, we also assume a push based model for analysis. The push model not only aids our detection strategies, but it is more efficient --- all the contacts of Bob would have the latest keys of the Bob (nearly) at the same time. Legitimate key updates do not occur very often; \textit{only} when a client re-installs the app. Hence, push notifications save resources at both the client and the server (compared to a pull-based model).

% There also exist apps like signal messenger that uses pull based approach wherein clients pull key updates on-demand from the server. Whenever Alice opens a chat window to communicate with Bob, her client issues a pull request to the server for Bob's key bundle. Pull requests ensure that Alice obtains Bob's current key before sending the message. The pull model means that some of Bob's keys stored on clients may be out-dated for anyone that hasn't recently communicated with Bob. Our defensive approaches can also be tailored for pull-based model, and we tend to explore this in our future work.

\subsection{Partial client-targeted attacks}
\label{partial_client_targeted_attacks}
%In our threat model, we identify two types of scenarios--- pair-targeted attacks (two specific Signal users Alice and Bob) and client-targeted attacks (Alice and \textit{all} of her contacts). 
% Both types of attacks and their mitigation strategies are analyzed in Section \ref{sec:analysis}. 
Our threat model includes two attack modes: pair-targeted and client-targeted attacks.
A variant of the second attack is a partial client-targeted attack where the MKS attacks Alice and \textit{some} of her contacts.
For the Trust Network, partial client-targeted attacks are less stealthy. If the MKS attacks only some of Alice's existing contacts, then the contacts that are not targeted can provide the correct key, either as a mutual contact or as a relay.
Anonymous Key Retrieval is unaffected by partial attacks since anonymity makes it difficult for the server to present fake keys consistently to only some users.
For Key Transparency, the multi-provider scenario detects any client-targeted attacks, whether partial or full. In the single-provider scenario, partial attacks are \textit{more} easily detected since the server will provide inconsistent STRs. Attacks that target all contacts are more stealthy since the server can present a consistent history of STRs.




% \subsection{Attacks on multiple clients}

% In our threat model, we have considered broadly two type of scenarios --- pair targeted attacks (target are only two specific Signal users \emph{i.e.} Alice and Bob) or client targeted (target is only Alice and \textit{all} of its contacts). Both type of attacks and their mitigation strategies have been explained in Section \ref{}.
% Bit, it can be argued that a third scenario also exists --- MKS may wish to launch the attacks against Alice and \textit{few} of its contacts.

% For a third scenario MKS has two options; either (1) it provide fake key updates for few of Alice's contacts to Alice or (2) its sends a fake key update of all most all of Alice's contacts to Alice.

% With first option, (assuming TN defense strategy), Alice would have multiple contacts left whose keys have not been changed. Lets assume Alice has $10$ contacts and she obtains a key update message for $4$ contacts. She could verify keys of these $4$ from rest of the $6$ contacts if some of the remaining $6$ are mutual contacts with the Alice and the $4$ clients. If not, she could use any of the $6$ clients as contact as relay (ref. Subsection \ref{subsec:TN}).

% For the second option, let us assume Alice receive fake key updates of its $8$ contacts. If she receives key updates simultaneously, attack can be easily detected using our heuristic burst of key updates. However, if MKS wishes to present these fake keys to Alice gradually; before it presents all, the attack would be detected by the Alice as it would become pair-targeted attack for Alice.

% With AKR based approach, clients would ask keys anonymously; a targeted attack for Alice and its specific contacts is not trivial as it is hard to distinguish one anonymous client from other. 
% Assuming MKS decides to randomly provide fake keys for some X new connections, it could be easily detected. Alice can anonymously ask for its own keys from the MKS. Thus, if among those X requests (for Alice's key bundle), there is request from Alice herself; the attack would be detected if MKS provided fake key bundle to all the X requests. (Alice could verify the mismatch between her uploaded key bundle and the one that was provided).





%However, if the MKS wishes to present these fake keys to Alice gradually, the attack would be detected as a series of pair-targeted attacks. For example, assuming the TN defense strategy, Alice would have multiple contacts left whose keys have not changed. Let's assume Alice has $10$ contacts, and she obtains a key update message for $4$ contacts. She could verify the $4$ keys from the remaining $6$ contacts if some of them are mutual contacts with the Alice and the $4$ clients under attack. If not, she could use any of the $6$ clients as a relay (ref. Subsection \ref{subsec:TN}).

% Partial attacks may affect the effectiveness of mass key update monitoring, depending on the thresholds use. However, this defense fills in holes of other defenses, and those holes are eliminated with partial attacks. 
% \ks{Unclear paragraph}
% \tarun{I think we can move this paragraph to 8.5 along with second last paragraph(that talks about TN)}

%If Alice receives a sufficiently large number of key updates simultaneously, the attack can be easily detected using the burst of key updates heuristic. For example, suppose Alice has $10$ contacts and receives fake key updates for $8$ contacts. 


%\subsection{User Enumeration attack in AKR}
%\label{sec:enumeration}

%Currently, Signal users authenticate to the key server before requesting keys. The server can block any user that attempts an enumeration attack---asking for the key bundle of many legitimate Signal users at a very high rate using automated scripts. 
%Since key requests in AKR are anonymous, it is more difficult for the server to determine if an enumeration attack is in progress, and there is no way to block a malicious user. Also, many malicious users could combine to attempt a denial-of-service attack. Client puzzles are a technique that could be used to mitigate this attack.


%\section{Limitations}

%\ks{Here is a quick list of limitations that we can expand on. Maybe place in its own section.}

%\begin{enumerate}
    
%\item We do not address group communication in Signal for this paper. It is an important topic for future work.

%\item Privacy leak to Mutual friends in Trust Network defense. Alice would learn about all the mutual friends Bob talks to.

%\item The lack of access to communication metadata of the messaging systems. We were unable to tune parameters like the regular monitoring time period, isolation monitoring interval, and delays. Tuning these parameters would optimize defenses.

%\end{enumerate}



==> Related_Work.tex <==

\section{Related Work}

\todo{Cite all of Elham's and Justin's papers}

Authentication is an inherent aspect of secure communication over Internet. However, many Internet clients have incomplete mental models about authentication over Internet. Schroder et al. \cite{} in their user study demonstrated that majority of Signal users failed to correctly verify their conversation partner's key due to usability issues like ... and incomplete mental model. Thus, there is a compelling need for more robust easy to comprehend authentication ceremony.

Presently, protocols like Signal resort to manual process (clients manually showing QR codes to each other) for authentication. 
The existing literature which aims to improve the key verification process of Signal is broadly divided into \textit{manual verification} and \textit{automated verification}.

Under manual verification, there exist a large body work that aims to improve the usability of the authentication ceremony, such as displaying hexadecimal blocks~\cite{PEP} as human understandable language (\emph{e.g.,} English). This approach consists of a one-to-one mapping of hexadecimal blocks to words in the user's language. This can, however, make cross-language comparisons prone to errors. Thus, in order to improve comprehension of the fingerprints, some protocols~\cite{whatsappProtocol} display fingerprints as numeric digits instead of hexadecimal or natural language strings.
% \textcolor{blue}{
% Modern messaging applications~\cite{whatsappProtocol} also display fingerprints as QR codes that users can scan off each other's devices.}

Vaziripour et al.~\cite{vaziripour2018action}, rather than focusing on comprehensibility of the fingerprints, modified the authentication ceremony by improving the UI of the Signal Application. 
They reported that participants were able to complete the ceremony more quickly in their new version of Signal. However, despite these improvements, there were significant fraction of participants who were still unsure (or confused) about the purpose of the authentication ceremony.

The manual process to authenticate clients suffers through many weaknesses. First, clients are expected to have reasonably good understanding of what is authentication ceremony and why it is important. Secondly, for clients which are not physically proximus to each other, becomes even harder to follow the authentication ceremony. 

Thus, researchers proposed some alternative approaches in which they aim to lessen the burden of authentication on the naive clients. Keybase is a key directory that links multiple social media accounts of a person to its encryption keys. This increases the confidence in the authenticity of the keys \emph{i.e.,} keys belong to the person associated with social media accounts.
Vaziripour et al.~\cite{vaziripour2019NoBother} attempted to semi-automate the authentication process in Signal app using social media accounts, similar to Keybase. 
They claimed that automating the authentication ceremony and distributing trust with additional service providers is promising, however these third-party actors need to be more trustworthy and accountable than social media companies. 
\textcolor{blue}{Additionally, there are few other concerns as well. Firstly, aforementioned approaches mandate that users must have additional social media account(s) where there public identity keys can be published. Secondly, it must be ensured that different social media platforms must not collude with the instant messaging apps (IMs)) under consideration. For example, WhatsApp a popular IM is owned by Facebook, likely the largest social media platform, can easily collude with each other. Lastly, we believe that onus of authenticating the social media account is on the IM user herself. It becomes necessary for a IM user to verify that the social media account owner is the person the user is trying to authenticate.}


% Recent research has explored the use of certificate transparency in secure email systems. Ryan~\cite{ryan2014enhanced} proposed an extension to certificate transparency that supported efficient revocation. They designed a secure E2EE email system using PKI that did not rely on certificate authorities.  PrivPK~\cite{alsabah2017privipk} is another secure email system that uses key transparency. It combines certificateless cryptography and key transparency to support forward secrecy. Similar to one of our approaches, it uses CONIKS for key transparency to automatically detect impersonation attacks. 
% There has been no research done from the perspective of the messaging application. Email systems differ a lot from the messaging application infrastructure. There are multiple email services providers which operate together whereas there is only one service provider involved in a messaging application. 
% The multiple service providers were used by earlier research to distribute trust.
\textcolor{blue}{Similarly, to automatically detect the authentication failures distributed ledger based approaches have been proposed. For example,}
CONIKS~\cite{melara2015coniks} (and its successor \cite{}) uses blockchain to enable \textit{completely automated} trust establishment with untrusted communication service providers by having the service provider maintain an auditable directory of all of its users' keys.
It was designed to incorporate multiple CONIKS service providers for auditing, but it can be adapted with just one provider as well. \textcolor{blue}{However, how to use such approaches with single provider has not been conceptualized yet. Thus,} in our research, as one of the possible approaches, we modified CONIKS to automate the Signal's authentication ceremony.

==> Results.tex <==
\section{Prototype Implementation Details}
% \label{prototype_implementations}

% We built several proof-of-concept prototypes to demonstrate the feasibility of fake-key attacks and defenses.

% \subsection{Setup}
% We created our own Signal infrastructure in the lab consisting of a server and five clients for performing attacks and experimenting with defenses.
% The lab computers had Intel(R) Core(TM)i7-7700K CPUs @ 4.20 GHz, with 16 GB RAM.
% We used the open-source Signal server \texttt{OWS 1.88} and simulated clients using \texttt{Signal-Android 4.23.4}.

% \subsection{Fake Key Attacks}
% We modified the Signal server to perform fake key attacks (both MITM and impersonation). 
% We added a client module to the server using the Signal client CLI\footnote{https://github.com/AsamK/signal-cli}. 
% It performs the standard ratcheting encryption done in normal Signal clients. 
% We modified the server to hand out fake keys to clients. 
% When the clients send encrypted messages to each other through the server, the server redirects the messages of the victim(s) to the client CLI module where the message is decrypted for the MKS to access it, and then re-encrypted and sent to the victim in the case of a MITM attack.
% Our experiment demonstrates that fake key attacks are possible in the current Signal server implementation.




% We modified Signal Server to implement MitM and impersonation attacks on Signal Server end. The attacker's client should do all the ratcheting encryptions as a client does. We used Signal client CLI (https://github.com/AsamK/signal-cli) for the purpose of attackers client. We incorporated the attacker's module along with the Signal Server. Whenever a Signal server wants to start a MitM attack, it passes the incoming message to the attacker's CLI client, which in turn returns a response. The Signal server than forwards that message to the intended recipients. To execute an impersonation attack the Signal server forwards the incoming message to signal CLI and reads the message through signal-cli. It then generates a new encrypted message using signal-cli and replies to the sender. In our prototype, an attacker can execute pair targeted attacks by specifying the identity (phone numbers) of communicating pairs to attack. To execute a client-targeted attack, an attacker only have to specify a client's identity.

% We set up our modified signal server at "signal.cs.byu.edu" to test our defense prototypes against the attack prototypes. 

% For the Trust Network's prototype, we mostly made changes on the android signal client. All the verifying messages are sent exactly in the same way a normal communication message would be sent. In our verifying message we add 

% In our prototype, we haven't tuned the timing parameters.

% For the AKR prototype, we use the Tor android library (https://github.com/jehy/Tor-Onion-Proxy-Library) at the android Signal client. To anonymously retrieve keys, the client sets up a Tor circuit and retrieves keys using that circuit. To run a tor service with identity key and make it accessible to the world, we used TinyWebServer to set up a local server on an android device and then redirect the Tor service to that local webserver.

% \subsection{Trust Network}

% To test the feasibility of the Trust Network, we set up five lab machines as Signal clients and one machine as the Signal server, modified to launch fake key attacks. 
% We modified the Android Signal client to support the Trust Network defense.
% All of the verification messages for the Trust Network were sent through the Signal server in the same way that current Signal messages are communicated.
% %Our Signal server (using client CLI) launched the various MITM and impersonation attacks shown in the Table \ref{tab:SignalTable}. 
% We demonstrated that clients can prevent or detect fake key attacks when they share mutual contacts and do not share mutual contacts. 

% \subsubsection{Client-side Memory Requirements}

% With the Trust Network, every Signal user maintains a database of hashed identities, \eg phone numbers, and the identity keys of its two-hop contacts. 
% The space to store information for one contact in a database entry requires 72 bytes---32 bytes (identity hash) + 32 bytes (identity key hash) + 8 bytes (timestamp).
% To estimate the storage requirements for the database, we assume a well-established network where the average user has 200 contacts.
% If each of Alice's contacts sends her on average 200 database entries, her database size is 2.88MB ($200*200*72$ bytes).

% \subsubsection{Efficacy of Trust Network: Mutual contacts}
% \label{trust_network_mutual_contacts_efficacy}
% The Trust Network prevents an MKS from launching an attack on Alice and Bob only if they have some mutual contacts. 
% To determine the probability that two Signal users share a mutual contact, we analyzed a Facebook dataset~\cite{nr} of $\approx 1.3$ million users and their friends.
% %The dataset contains a graph G(V,E), where the vertices V represent users and edges E represent the friend relationship between two users. 
% For our analysis, we considered users who had two or more friends, which was a total of 
% 1,279,517 users.
% From our analysis, the average user has at least one mutual friend for 59 percent of their connections, and the average number of mutual friends is 4.46.

%The well-connected users in the dataset had at least one mutual friend for 75 percent of their contacts and an average of 6.25 mutual friends with their contacts.
%\textcolor{red}{In the dataset: 
%\begin{itemize}
%    \item Total nodes in network: 2937611
 %   \item Nodes with only 1 friend: 1658094
 %   \item Nodes with >2 fiends: 1279517
 %   \item Nodes with friends less than 10: 2315228
%    \item So, we did analysis on 2937611- 2315228 = 622383 nodes
%    \item
%\end{itemize}

%\todo{
%Option 1) We can keep the results as it is. we can remove the upper limit of 500 as there were around 3000 nodes in the network with more than 500. After removing upper limit I got almost same results.
%Option 2) Instead of using lower limit as 10, we can use lower limit 2. We can argue that here we are trying to look at mutual friends, so we considered nodes with at least 2 connections to look at mutual friends.
%Option 3) May be we can make a distribution like what is the number of connections with mutual friends if we consider connections greater than1, then greater than 2, then greater than 3......
%}

%\input{Table.tex}


% We explain our analysis with an example. First, for every individual user, we extracted its friend list from the datasets.
% We began by selecting five random friends of Alice from her friend list. Next, we identified that, out of five contacts, Alice had mutual contacts with whom and how many? 
% Let us assume Alice had mutual contacts with only 3 of her selected contacts and with those 3, she had 6 mutual contacts. Thus, \textbf{there exist a probability of (3/5), that Alice has atleast one mutual friend with some randomly selected contact. For the contacts with which she had mutual contacts, the average number of mutual contacts is (6/}. 
% how many mutual friends Alice has with each of her five friends. 
% After this step, we had five numbers, each corresponding to the number of mutual contacts she has with five of her friends.
% We calculated the average number of mutual contacts she has with her five friends ($MC_{Alice}$). 
% \begin{equation}\label{gen_eqn}
% MC_{Alice} = \frac{total \thickspace  mutual \thickspace friends}{total \thickspace Alice's \thickspace friends} * 5
% \end{equation}
% The same process is repeated for all the selected users in the dataset. Our results show that there is 0.75 probability of getting a mutual contact with a random contact from the friend list. For the users we found mutual contacts, the average number of mutual contacts is 6.25.

% Next, we simulated a scenario where a new user, Alice, joins the social network and starts building her friend network. 
% To determine the fraction of Alice's friends with whom she has at least one mutual friend,
% we first isolated an existing user from the given dataset by removing all its edges from the graph. 
% After removing Alice from the graph, we simulated a scenario where she starts building her friend network from the beginning.
% In every iteration, we created an edge between Alice and one of her contacts (Bob) that had not been visited yet. We calculated whether she has a mutual contact(s) with Bob or not. If yes, then we counted the number of mutual contacts. 
% Finally, when Alice ends up having edges with all of her original set of friends, we calculated the fraction of Alice's friends with whom she has mutual contact(s) and also the average number of mutual contacts she has with them.
% %We repeated the same process for all the well-connected users of the dataset and calculated the averages. 
% We found that a user has at least one mutual friend in 64\% of their connections while creating their friend network,
% and an average of 5.7 mutual friends per connections.

% \subsection{Anonymous Key Retrieval}

% We modified the Android Signal clients to support Anonymous Key Retrieval using the Tor Android Library.\footnote{https://github.com/jehy/Tor-Onion-Proxy-Library}.
% %To anonymously retrieve keys, the client sets up a Tor circuit and retrieves keys using that circuit. 
% We used \texttt{TinyWebServer} on the client as a local server where the identity key of the user is available then proxy the server's traffic via a Tor SOCKS proxy to create a hidden service. 
% %redirect the Tor service to that local webserver.
% We used one computer as a Signal server for launching fake key attacks.
% %For AKR, our Signal clients anonymously queried for the identity keys of the other clients. Our requests did not include the sender’s unique identity, and Signal clients sent such key retrieval requests to our Signal server via Tor. 
% We were able to prevent/detect the MITM and impersonation attacks. 

% To examine the effects of delay, we conducted an experiment measuring the cost of accessing keys via Tor. We requested a key bundle through Tor $100$ times per day for ten days using both WiFi and 4G networks. The time includes setting up a Tor circuit and retrieving keys from the server using that circuit. 
% %Figure \ref{fig:Tor_Service_Up} shows the results of our experiment. 
% Over WiFi, it took an average of $10.4s$ to retrieve keys from the server using Tor and an average of $11.88s$ over a 4G network.


% \subsection{Usability Analysis}
% A critical usability factor is whether Alice experiences a delay when she wants to send a message to Bob.
% Some defenses designed to prevent attacks may require time to verify a key before it used, which may cause a user some delay.

% \begin{itemize}
% \item The \textit{Key Transparency defense} only detects attacks. 
% Since it verifies keys after a conversation begins, the users experience no delay.

% \item In the cases where the \textit{Trust Network defense} prevents an attack, it verifies a key before sending the first message. If there is mutual friend, there is negligible delay to verify key from local key database. If there is no mutual friend clients uses contacts as relay. It incurs a delay of $\approx 200$ ms (for a single hop relay) in our lab experiments.
% % \deva{How we got this number? If we have explained this number in some previous section, we should refer that.}
% % \tarun{To calculate delay for contact relay, we used our setup of five clients, We chose two clients such that there is not any mutual friend between them. This delay is the total time taken between the Key verification request sent to one of the contact and the response that client gets from the friend.}

% \item For \textit{Anonymous Key Retrieval}, the basic defense only detects an attack, so it incurs no delay. 
% The advanced defense sends a query through a Tor circuit, which takes an average of 11.14 seconds. 
% \end{itemize}


% \subsection{Performance analysis}
% We evaluate our design implementations with the following parameters based on the assumptions made by CONIKS \cite{melara2015coniks}:
% \begin{itemize}
% \item An IM application supporting N= $2\textsuperscript{32}$ users. 
% \item Monitoring occurs once per hour. 
% \item Up to 1\% of the users change or add keys per day.
% %, meaning n ≈ $2\textsuperscript{21}$ directory updates in an average epoch. 
% \item A 128-bit cryptographic security level (SHA-256, 512 bit EC-Schnorr signatures).
% \item Clients have an average of 100 connections.
% \end{itemize}


% % \deva{\textbf{DEV: Is there any specific reason to select aforementioned parameters? }}

% \subsubsection{Client-side Memory Requirements} 
% With the Trust Network approach, every user maintains a database of hashed identities --- phone numbers and the public keys of its two-hop contacts. 
% The space to store information for one contact in a database entry requires 72 bytes --- 32 bytes (identity hash) + 32 bytes (public key hash) + 8 bytes (timestamp).
% To estimate the storage requirements for the database, we assume a well-established network where the average user has 100 contacts.
% If each of Alice's contacts sends her on average 100 database entries, her database size is 720KB ($100*100*72$ bytes).

% The Key Transparency approach requires storing the previous STR at the client. The total size of the STR size is 104 bytes (64 for the signature, 32 for the root, and 8 for a timestamp).

% \subsubsection{Client-side Network Traffic}
% In the Trust Network approach, when two clients start communicating, they share their contact's verification bundle. For every contact, they share identity hash (32 bytes) + identity key hash (32 bytes) + timestamp (8 bytes) + EC-Schnorr signature of these three tuples (64bytes). Assuming a client has 100 contacts on average, the contact's verification bundle is 13.6KB ($100*136$ bytes). The total network traffic to exchange verification bundles whenever there is a new connection is 27.2 KB.
% Whenever there is a key update, clients are required to push the key updates to all their contacts. From our assumption, 1\% of the clients in the system update keys every day. Therefore, a client would send one contact's key update to their 100 contacts and receive one key update from every contact. Total network traffic for this process is 27.2 KB ($100*136 + 136*100$).

% When two clients start communications, Key Transparency uses $32.(lg_2(N)+1)+96$ \emph{i.e.,} 1.216 KB ($lg_2(N) + 1$ hashes
% and one 96-byte verifiable random function proof) for a new key lookup~\cite{melara2015coniks}.
% For monitoring, Key Transparency approach requires downloading of $64+lg_2(n).32 = 736$ bytes every epoch and for auditing it requires 104 bytes every epoch (64 for the signature, 32 for the root and 8 for a
% timestamp). Therefore key transparency with multiple-providers requires a total of 20.1 KB per day (17.6 KB for monitoring and 2.5 KB for auditing) ~\cite{melara2015coniks}. In the case of Key Transparency with a single provider, the monitoring cost would be the same, i.e., 17.6 KB. Clients audit the provider by verifying STR with their friends. They only need to check STR when there is a key update. From our assumption of 1\% key updates, every client's only single contact's key would be updated every day. In such a case, the client uses 104 bytes (64 for the signature, 32 for the root, and 8 for a timestamp) to verify STR with one contact. If a client confirms the STR with ten randomly chosen contacts, %bandwidth would be
% it requires exchanging of 
% 1.04 KB data. The client also might have to answer to STR verification request if someone asks for it. The probability of getting selected by one of the contacts is 0.1; therefore, the number of verification request a client would receive are 10 KB ($0.1*100$ bytes). The total network traffic used for monitoring is 11.44 KB ($1.04 + 10*1.04$ bytes) per day. The total network traffic by single provider key transparency is 29.04 KB ($17.6 + 11.44$) per day.

% In AKR, a client retrieves keys from the server using the TOR circuit. There is no straightforward approach to find data usage for the Tor circuit theoretically. So, we implemented an Android app that 1) creates a TOR circuit, and 2) retrieves the key bundle of a user from our implementation of the Signal server. We used the packet capture android app to capture pcap for this app and analyzed it in Wireshark. One key retrieval using the Tor circuit uses ~32 KB of data (15KB sent + 17KB received). 
% The basic AKR doesn't store anything on the client-side i.e., no client-side requirement. The advanced AKR stores the TOR service URL of every friend. One TOR URL is of 16 bytes (16 char). From our assumption of 100 friends, the total client-side memory usage is 1.6KB. In basic AKR, after a client starts a new communication, it monitors a new connection's key until it has confidence that the key she received is correct. Assuming that a client wants to detect an attack within 10 hours with probability 0.999,  as explained in Section 5.1, it would take ~320KB (32KB x 10times) for every new connection. Also, every client monitors their key regularly. From our assumption that every client monitors their key every hour, the daily network traffic is 768KB (32x24 times).
% In advanced AKR, when a client starts a new communication, it retrieves other client's keys from the MKS through the Tor circuit, and it costs the client ~32KB data. If there is a key update, it retrieves the key from the corresponding client's TOR service, which requires ~40KB. Also, a user monitors the new/updated key for some interval, like in basic AKR. So, the total data usage for a new connection is 320 KB (32Kb x 10 times monitoring), and for a key update is 328KB (40KB for first-time key verification + 32KB x 9 times). The total daily network traffic is the same as basic AKR i.e., 768KB(32x24 times).



%\begin{figure}[h!]
%\vspace{-0.5cm}
%\centerline{\includegraphics[width=0.5\textwidth]{images/BoxPlot2.pdf}}
%\caption{Time taken to a) retrieve keys through Tor circuit b) bring online the Tor service on a client }
%\vspace{-0.5cm}
%\label{fig:Tor_Service_Up}
%\end{figure}

%Moreover, to defend against attacks on existing connections, a client is required to host a Tor onion service on its mobile device to aid the key verification process. A client’s Tor service is offline most of the time, and it is brought online during a particular time of the day. To measure the average time required to bring a hidden service online on an Android device, we brought up a Tor service $100$ times a day for ten days (both on 4G and WiFi). The time in bringing a Tor service online includes a) setting up a local server, b) setting up a Tor circuit, c) publish the Tor service’s identity in the Tor network, such that some Tor relay could act as an introduction point to the Tor service. Figure \ref{fig:Tor_Service_Up} shows the results. The average time taken to make Tor service accessible is 8.4 seconds on WiFi (\textit{TorServiceUP\_WiFi}) and $8.5$ s on 4G (\textit{TorServiceUP\_4G}).


==> Reviews/CCS_Reviews.tex <==
% \section{CCS reviews}

% Move these to their own document per instructions. See todo list in main document.

\section{Review \#A}


\subsection{Overall merit}

1. Reject

\subsection{Paper summary}
The paper addresses a problem in the context of usable security: If the initial Diffie-Hellman share for key agreement in an end-to-end-encrypted instant messaging scheme (SIGNAL, WhatsApp, Telegram) is sent transparently (i.e. without user interaction) to the client applications, a malicious key server may deliver fake initial shares to become a man-in-the-middle. Such attacks normally would be detected by manual comparison of the key shares, which however would significantly reduce the usability of the solution. The authors therefore define an attacker model and propose three solutions on how to automatically detect such attack without user involvement.

\subsection{Strengths}
The paper addresses an important problem, and is well written. It presents three generic solutions to the general problem, which all seem to be applicable in practice.

\subsection{Weaknesses}
The threat model is not clear enough on the capabilities of the adversary. This leads to inconsistencies in the security analysis, which is either correct or wrong. The countermeasures also do not take into account special security properties of IM cryptographic schemes, e.g. SIGNAL's ratcheting scheme.

\subsection{Comments for author}
\begin{itemize}
    \item Section 3: The threat model is no clear enough. What does 'malicious key server' and 'hacked key server' mean? Is this the same threat model? What about long-lived public keys to authenticate the key shares: Does a malicious/hacked key server know the private keys for these public keys? Similarly unclear are the network capabilities of the adversary: Does he control all communications, or only some? Does he control the central communication server in an IM scheme, or only those requests that are directed to the key update server?
    
    \tarun{We updated the threat model to make the attackers capability more clearer.}
    
    \item Section 4: The security of this countermeasure depends on the question above. In this section you assume that 'To ensure that Alice’s contacts cannot falsify keys for Bob, the key server must sign each key that it distributes to clients. Thus the key server generates a long-term asymmetric key pair and sends the public key to clients at the time of registration.' But if the malicious/hacked key server knows the private key, he can forge all these verification bundles. And if he controls all network connections, he can deliver these forged verification bundles instead of the real ones.
    \tarun{
    This is along the lines of our primary attack that we described in our threat model i.e the key server distributing fake keys. The signatures in verification bundle's purpose is to defend against malicious contacts not to prevent this attack. To defend against the attack described, we use mutual contact, contact relay and monitoring heuristics. 
}
    
     
    \item Moreover, the exact meaning of 'client targeted attack' remains unclear: In Section 3 you write that 'a client-targeted ... is also more easily detected, since it involves many pairs of fake keys'. So if the key server delivers different keys to different people, section 4 is wrong since it is required that 'Now Alice compares the hash of the key from Bob’s verification bundle that was sent by Carol with the hash of the key provided by key server. If they match, Alice trusts the key, otherwise the attack is prevented.' This only works if the server delivers the SAME key to all contacts.
    \tarun{ Every user in the system have a unique public private key pair. So in ideal scenario, the key server delivers same public key for a user to everyone in the system. Section 4 talks about detection of pair targeted detection in that part, by using the fact that every contact should have the same public key for a contact. 
    Section 3 talks about client targeted MITM, where the MKS intercepts all the connections to a client C. So, to execute this attack the MKS need to a fake key for C to all C's contacts and provide fake public keys to C for their contact. As every user in the system has unique key pair, the MKS provide different fake keys to C for their contact to make the attack undetectable, that's what we mean by different key pair in section 4.
    TODO: Make the sentence more clearer in Section 3?}
    
    \item Inconsistencies like the ones mentioned above must be clarified before the paper can be accepted.
    \tarun{updated.}
    
    \item As an additional idea: If the IM scheme uses ratcheting, both parties share a common state. Can this common state be used to detect a fake 'key update' message? Such a message should only be necessary if one of the two parties has lost its internal state, however, there must be a previous state which both parties still shared.
    \tarun{This line of reasoning works if we are only handling the case when a user does not lose their phone or re-install the messaging app. In both of these cases, prior conversation state is lost and the app generates a new public key for the user. If we were only handling the case where the user’s phone is not lost, then no key updates are possible, so the user simply has to reject any key update messages. But this is not how Signal and related secure messaging protocols work. They handle key updates for reinstalled apps or lost phones. So we need some other mechanism to distinguish valid key updates from malicious key updates.}
\end{itemize}

\subsection{Required improvements}
Formalize the three model, and show formally how the proposed countermeasures would help to prevent the described attacks.
\tarun{TODO: (update this) For AKR, we did a probability based security analysis in section 4.1. For Trust network, we individually evaluated the modules. For key transparency, we build upon the security properties of a well known system CONIKS.}



\section{Review \#B}

\subsection{Overall merit}
3. Neutral

\subsection{Paper summary}
The paper revolves around fake key attacks in secure messaging applications like Signal and WhatsApp.
The main motivation is how to prevent/detect instances where a compromised server is providing fake
keys to either impersonate specific users or MITM the communication between users. To that end, the
authors present 3 different approaches, including several extensions, and detail how each defense fares
against the different attacks. The first proposal (Trust Network) relies on other trusted contacts
for verifying a user's key, e.g., a common contact between 2 users trying to communicate. In the absence
of common contacts, contacts can be used as relays for obtaining the keys from the server for verification.
The 2nd proposal (Anonymous Key Retrieval) provides additional security by abstracting away identities and also incorporating Tor hidden services for hiding users' IP addresses. The final proposal "modifies" CONIKS
for a single provider scenario where clients also play the role of auditors.

\subsection{Strengths}
\begin{itemize}
    \item Secure messaging is a timely and important topic.
    \item Provides prototype implementations.
    \item Provides extensive discussion on how each attack is affected by each proposed countermeasure.
    \item The paper is well written.
\end{itemize}

\subsection{Weaknesses}
\begin{itemize}
    \item Narrow scope: focuses on very specific, and unlikely, attack.
    \item Some of the proposed defenses or arguments/claims are unrealistic in the context of a real-world deployment and core use cases of these apps, and also introduce privacy risks.
    \item Several of the concepts here have been explored to some extent in prior work.
    \item AKR, which is the most novel/strong countermeasure, relies on a third-party infrastructure which may not be available to many users.
\end{itemize}



\subsection{Comments for author}
\begin{itemize}
    \item In general, the paper was easy to read and focuses on secure messaging apps, which is an important topic. However, the paper focuses on a class of attacks that is extremely (to say the least) uncommon -- even the motivating example provided in the intro (IronChat) is unlikely an example of such an attack given what is publicly known. As such, the paper has a very narrow scope. 
    \tarun{We have updated the motivation of our research in the Introduction section.}
    
    \item Given the analysis and proposed defenses in [17], the contributions become somewhat incremental 2 of the 3 approaches are not really that novel. 
    \tarun{[17]] evaluation included the addition of auditable logs like CONIKS to a key directory to detect attacks. Our work builds on their evaluation in several ways. First, we provide an in-depth discussion on how to adopt CONIKS to a single operator. We also provide two additional approaches to prevent or detect attacks automatically. Their SoK focuses entirely on manually approaches to comparing fingerprints. They considered web of trust solutions, but only manual key signing parties in PGP instead of an automated trust network solution like we propose.}
    
    \item To make matters worse, apart form the lack of novelty, the Trust Network approach also has several other issues and is extremely weak proposal overall with several assumptions that don't cover common/critical uses of secure messaging apps. \item First of all, the strong security properties should when Alice and Bob have a mutual contact. However, that would not be the case in many important scenarios (e.g., an informant communicating with a journalist) where such applications are used. While I understand that obtaining such data is hard, the numbers provided from Facebook obviously bear no semblance to what user's messaging app social circles look like. 
    \tarun{That's true stronger security property using mutual friends might be not be possible in every case. But even in the cases of non-mutual friends TN makes significant progress in detection of attacks as compared to current authentication ceremony.}
    
    \item Furthermore, the privacy leakage that occurs where users' social graph data are exposed would prevent the deployment of such a countermeasure in practice. 
    \tarun{This approach does have the limitation of mutual friends' information leakage therefore could not be used in every scenario. But this approach could be the right fit in some scenarios like LinkedIn. There is no way on LinkedIn to hide the mutual connection. If they would want to incorporate E2EE for their messaging platform, Trust network could be a good fit for them. }
    
    \item Next, the arguments in 4.4.7 are unconvincing given the wide deployment of IPv6 by mobile providers (e.g., see https://blogs.akamai.com/2016/06/preparing-for-ipv6-only-mobile-networks-why-and-how.html) --  arguing that "many users NAT are likely behind the same NAT device" is not really a sufficient countermeasure against sophisticated timing attacks.
    \textcolor{blue}{
    In this section we discussed about possibility of traffic correlation attack \textit{solely based on the IP address} --- what if Alice has a fixed IP address; MKS could identify Alice based on source IP address (an not timing analysis).
    }
    
    
    \item Given these limitations, the Trust Network defense should not be presented so prominently and extensively in the paper since it weakens the overall presentation. The other 2 proposals should be presented in more depth (E.g., the presentation of the CONIKS-style defense is extremely concise and "superficial"). More weight should be given to section 6 and more details should be provided, and the authors should better clarify how novel this proposal is based on the original CONIKS proposal -- since the authors explicitly state that "Clients serve as auditors for their own identity provider" in the original proposal, it's not clear how different their current design is.
    \tarun{We have restructured the paper to focus on AKR approach. In the original CONIKS proposal, clients could audit their own identity provider because there are multiple providers. Clients randomly query a few other providers to verify that they give the same STR as their identity provider. In our proposal, we have to design a new auditing process that works even when there is a single identity provider.}

\item A similar issue is the vagueness of claims in the AKR defense where attacks will *eventually* be detected. 
\tarun{We have explained this in AKR defense with an example, the detection period depends on the monitoring interval. The probability of detecting an attack increases as the monitoring interval passes.}

\item Given that this is the most novel of the 3 proposals (given [17]), the fact that it relies on a third party infrastructure that is commonly blocked in many countries, while also only guaranteeing that attacks will be detected *eventually* significantly limits the benefits of this proposal when considering the challenges of deploying it. 
\tarun{The basic AKR only detects attacks, and advanced AKR prevents attacks. For the basic AKR, given the monitoring interval of an hour, the basic AKR detects an attack within 7 hours with a probability of 0.992.  }

\item Furthermore, attack detection inherently relies on multiple contacts communicating over time and the communication being attacked, which may result in significantly delayed detection in critical scenarios.
\tarun{The detection depends on the user monitoring their keys regularly. 
}

    \item Similarly, the AKR defense requires the mass update key monitoring approach to detect client-targeted existing connection attacks, which if done in a stealthy manner will only be detected *eventually*.
    
    \item Next, in 6.4.5 the paper states that an exchange of conflicting STRs will occur eventually unless there is a complete partitioning of the network. However, no additional details are provided. What does that mean? How would this happen? How hard is it for the attacker to do that? Would that completely bypass all your defenses? Again, in 6.4.6 the stealthier attacks can only be detected when all 3 heuristics are included.
    \tarun{This attack is possible when all the new contacts of a user and the user are on completely different sub-networks. The server in theory can do it breaking/not allowing connection between two subnetworks where the server is executing the attack. It bypasses the CONIKS defense. Although, the KS needs to break a lot of connections to create two disjoint networks.}
    
    \item Overall, there seems to be a lot of room for stealthier attacks to take place before they are actually detected. Given that such applications are commonly used by high-value targets with non-overlapping social graphs, it is not immediately obvious how effective these mechanisms will be in practice. In fact, by removing/reducing the key change notifications, the end result might be an increased false sense of security in certain scenarios.
    \tarun{The AKR and CONIKS don't depend on overlapping social graphs. Even, the Trust network doesn't entirely depend on overlapping sub-graphs. If there are no mutual friends, we use contact as a relay.}
    
    \item It is not clear from section 8.6 if the proposed approach is actually applicable to Signal due to its pull-based model. If that is the case, the authors need to be upfront about this significant limitation and explicitly mention it in the introduction/background as well.
    \tarun{The pull-based approach is needed by the Trust network approach only. Other approaches work on both pull and push-based}

    \item It would also be nice if the authors obtained feedback from vendors (e.g., Signal) regarding fake key attacks and the proposed countermeasures (e.g., to see whether they are concerned with such attacks and willing to adopt the proposed defenses or are independently exploring other approaches).
    \item The authors have overlooked a relevant paper (Vasile et al., IWSP '19)
\end{itemize}


\subsection{Required improvements}
---------------------
\begin{itemize}
    \item Provide more concrete measurements/statements about the security limitations of the proposed defenses instead of stating that attackers will *eventually* be detected. The critical nature of many communications that take place over such apps necessitate concrete data instead of vague quantifiers (e.g., through simulations).

    \item Better emphasize novelty of proposed solutions, especially for CONIKS-based countermeasure.

    \item Provide more details for the CONIKS-based countermeasure.

    \item Provide missing details mentioned in my review for section 6.4
    \item Obtain and provide data that accurately quantifies the feasibility of the Trust Network approach and better highlight all the limitations of this approach in a realistic setting. Furthermore, this countermeasure should be less prominently featured that the other 2, given the significant limitations.
    \item Better motivate proposed countermeasures (e.g., using feedback from vendors regarding their concerns/view
on fake key attacks)
\end{itemize}



\section{Review \#C}

\subsection{Overall merit}
4. Weak Accept

\subsection{Paper summary}
This paper studies defenses against man-in-the-middle (MitM) attacks and impersonation attacks in end-to-end encryption systems. The paper carefully analyzes three defenses and their security properties, together with implementations and evaluation

\subsection{Strengths}
\begin{itemize}
    \item Highly important topic
    \item Solid and detailed analysis
\end{itemize}

\subsection{Weaknesses}
"Unconventional" novelty

\subsection{Comments for author}
\begin{itemize}
    \item I am a bit torn by this paper. I very much enjoyed reading this paper and I felt I learned a lot from the paper. The discussion on monitoring heuristics, anonymized key retrievals and defense comparisons are helpful and thought-provoking. The experimental results can serve as useful references to the community.

    \item On the other hand, it is difficult to get super excited about this paper. Even though I find the discussions and observations well thought out and well-articulated, at the end of the day, they are quite natural. In fact, I have thought about a small subset of these nuances in casual hallway discussions with colleagues. I suspect different small pieces of this paper have appeared at some point in everyday encounters and meetings in different institutions and tech teams. Of course, the paper is much more comprehensive and systematic.

    \item The implementation section is quite terse in the main body. I would like to see some of the more important details in the main body. To make space, I find several points unimportant. The distinction between single-provider and multi-provider is superficial once you ask clients to be auditors. The contact relay details feel too low-level to me.

\end{itemize}

\section{Review \#D}
==========================================

\subsection{Overall merit}
2. Weak reject

\subsection{Paper summary}
The paper recalls that people do not use eg QR codes in messaging, which leads to possible fake key insertion attacks. The paper discusses three strategies for coping with this problem (without user input) and analyses their effectiveness.

\subsection{Strengths}
Very topical real-world problem that would be great to solve.

\subsection{Weaknesses}
\begin{itemize}
    \item Extremely informal security analysis means that effectiveness of defenses is not convincing -- these proposals really need a detailed security and privacy analysis.
    \item Trust network suggestion completely breaks privacy of peer-to-peer connection, as it reveals intended communication partners to others.
    \item Unclear how to deal with out-of-sync behaviour and offline contacts selected for trustnetwork/relaying.
\end{itemize}

\subsection{Comments for author}
\begin{itemize}
    \item I like the problem that this paper tackles, but at the moment the security analysis is way too informal, and therefore entirely unconvincing. I highly recommend the authors to continue working on this, but find a way to do a more rigorous analysis of both the security and privacy aspects.

    \item Looking at the contributions:
     - Contribution 1: I don't agree the designs are detailed enough yet, e.g., when it comes to the intervals in the anonymous retrieval (see below), but this should be fixable; I would actually rephrase the contribution to "we propose" -- but since the third proposal is basic key transparency, this needs to be carefully quantified.
     - Contribution 2: This is the core problem for me, and would need a good methodology to work from.
     - Contribution 3 I would remove. It is not hard to see that these attacks work.
     - Contribution 4 is part "analysis" and part "feasibility".
     I feel the paper and its contributions are written in the vein of "this is what we did" instead of the more helpful "this is how we advance the state-of-the-art". I would recommend rewriting these parts in the style of the latter, while being self criticial. I think this would really bring out the unique contributions better.

    \item In Table 2, it is suggested that e.g. trust network prevents certain attacks, but this only can be true if the network is 100\% reliable, the required peers are online, and the checking agent does not "accept" or "receive" the first message until it has confirmation of the key from the trust network. I don't think these are realistic assumptions that would make the system unusable in practice.
    \tarun{The Trust network prevents attacks either by using the keys in the dataset (no network reliability needed) or through contact relay using a sealed sender, where it can use any friend. In our test, it took approx 200 ms to do that, I think users can wait for that much?}

    \item In Section 5.2 there is not enough detail about the intervals, which is crucial. If these are not done the right way, then the Server can trivially tell the self-requests from the other requests. The analysis of the authors assumes the Server does not know about the regular intervals and/or is not able to infer anything about the intervals. This makes the analysis unconvincing.

    \item I found it interesting that in Table 1, the Anonymous Key Retrieval (basic) has 0 verification delay and 0 client side memory. I never knew running a TOR client required 0 memory ;-) A similar comment can be made for the advanced variant.
    \tarun{The verification delay is the time a user needs to wait before they can start sending/receiving messages. As in the basic AKR, we are not waiting for the verification to be completed before allowing the user to send/receive a message so the delay incurred is 0. By "memory" we mean to say disk space. We'll update the term to make it clear. The AKR doesn't store any additional things for verification.}

    \item While the lost of privacy for the trust network solution is vaguely hinted at, I think this is actually a no-go for most application scenarios. This is too hidden for me in, e.g., the conclusion.

    \item The prototype is nice, and shows that the naive fake key insertion attacks don't work. However, it of course cannot show that there is not a slightly more clever version of the attack that does still work.

    \item For the trust network, what happens if clients run out of sync? E.g. Bob has pkB1, and Alice receives it. Now Bob gets a new key (maybe changes phone) and starts with pkB2. Alice is offline, but Charlie obtains pkB2. Now Charlie asks Alice, who is just coming online, and before Alice obtains pkB2 from the server, she responds with pkB1 to Charlie. This leads Charlie to conclude that there is an attack, right? If so, how can this be dealt with.

\end{itemize}


\subsection{Required improvements}
\begin{itemize}
    \item Find a more accurate/formal way to analyse the security and privacy of the proposals. There are many methods used in the literature. This also requires making the threat model more concrete in terms of the capabilities of the adversary.
    \item Better separate between "this is what we did" versus "this is the state of the art and these are our contributions that advance the state of the art".
    \item Clarify details e.g. of interval scheduling for anonymous key retrieval suggestion.
    \item Clarify trade-off between prevention/wait for response in the asynchronous settings where some phones may be off for longer, or lost, broken, etc.
\end{itemize}



\section{Review \#E}

\subsection{Overall merit}
2. Weak reject

\subsection{Paper summary}
The paper presents a method to detect and prevent so-called "fake key" attacks in secure messaging systems (e.g., WhatsApp), whereby a malicious key server can distribute fake keys to users to perform impersonation or man-in-the-middle attacks. The paper presents an implementation of these
attacks to demonstrate feasibility, and implements various defenses. The defenses include a range of approaches, including: (1) a trust network
(similar to a web of trust); (2) anonymous key retrieval, which makes it more
difficult for a malicious server to target a specific user; (3) key transparency (e.g., certificate transparency).

\subsection{Strengths}
The paper explores the potential weaknesses of fake keys in a secure messaging
system and explores a range of defenses against these attacks.

The paper performs a proof-of-concept demonstration of both the attacks and
defenses.

The performance numbers (latency, memory) show that the proposed approach can
be practical.

\subsection{Weaknesses}
The paper's delta beyond past work on certificate transparency and CONIKS is
not clear. The attack has not been observed in practice and is a general weakness of any
centralized system.

\subsection{Comments for author}
\begin{itemize}
    \item  The paper takes existing technologies (certificate transparency, web of trust, etc.) and applies it to a hypothetical problem in secure messaging systems (attacks of fake keys at the server). But there is no innovation here in design, and the attack is hypothetical.

    \item The attack depends on a strong assumption: that the message key server itself is hacked.  The authors themselves indicate that this scenario is unlikely and has not been observed in practice, indicating that this is mostly a
    hypothetical attack.

    \item Beyond past work on CONIKS and CT, which explicitly list secure messaging as a use case, the contributions to key security are not clear from reading the paper. In fact, secure messaging was a motivation for the CONIKS design in the
    first place, and so the paper might want to offer some qualitative and
    quantitative comparisons to CONIKS: (1) explain why previous approaches are
    inadequate for solving the fake key attack; (2) compare the performance and
    effectiveness of the proposed approach to past approaches, including CONIKS.
\end{itemize}


==> Security_analysis.tex <==
\subsection{KT Security Analysis}

We now analyze how well Key Transparency protects users from the attacks we have identified. For pair-targeted attacks, we assume a connection between Alice and Bob. For client-targeted attacks, we assume the targeted user is Alice.

For the {\em multi-provider scenario}, we can detect all pair-targeted and client-targeted attacks. The target of the attack can always contact an auditor, independent of its communication with its identity provider, and thus obtain proof of equivocation. We rate these attacks as detected rather than prevented because of the delay imposed by epochs. \ahc{did you discuss multi-providers at all? or auditors?? and, this isn't sufficient as analysis. when are auditors contacted? being to contact isn't enough if you don't contact! }

However, in the {\em single-provider scenario}, all communication occurs through a central key server, which makes its MITM attacks more powerful. We discuss each attack for the single-provider scenario below: \ahc{this looks like a list of specific attacks, but security should be wrt security goals and attacker capabilities, not of specific attack strategies. This will require more careful arguments but is doable. }


\subsubsection{MITM, pair-targeted} Since this attack is pair-targeted, there must exist an STR with the fake keys and another with the real keys. Alice can query any random contact for the latest (real) STR they have received from the central server and compare it to the (fake) STR she receives. She discovers the equivocation and detects this attack.

\subsubsection{MITM, client-targeted, new connections} In launching a MITM attack on Alice, the key server may choose to attack only new connections Alice makes. In this case, (1) the MKS creates a forked history for Alice containing fake keys for her new contacts, (2) a forked history for Alice's new contacts containing Alice's fake key, and (3) keeps all of Alice's existing clients on the original history. Alice can detect this attack by obtaining the latest STR from an existing contact. 
Alice's new contacts may not detect this attack if the MKS gives every client except Alice's existing clients a forked history unless a new contact shares an existing contact with Alice. However, this allows Alice's existing contacts to detect this attack when seeing exchanged STRs from other clients.

\subsubsection{MITM, client-targeted, existing connections} 
The MKS can instead choose to conduct a MITM attack on all of Alice's existing contacts by sending Alice and her contacts fake key updates. The MKS issues a consistent, linear history with the fake key for Alice to all of Alice's contacts while giving Alice a history that includes her real key but fake keys for all of her contacts. 
Key Transparency cannot detect this attack with the MKS performing an active man-in-the-middle attack because any time Alice asks for the latest STR a contact has seen, the MKS can intercept the request and falsify the response. Meanwhile, all of Alice's contacts see the same, consistent history.
To defend against this attack, we use mass key update monitoring heuristic \S\ref{subsec:MassKeyUpdate} from Trust Network defense. It \emph{prevents} naive attacks and \emph{detects} stealthy attacks.

\subsubsection{Impersonation, pair-targeted} Since this attack is pair-targeted, the target of the attack, either Alice or her contact, can query a random contact for the latest STR they have received, compare, and find the equivocation, detecting the attack. 

\subsubsection{Impersonation, client-targeted, new connections} When impersonating new clients to Alice, the MKS creates a forked history for Alice containing fake keys for her new contacts and keeps all existing contacts of Alice on the original history. Alice can detect this attack by obtaining the latest STR from an existing contact. When impersonating as Alice to new contacts, the MKS creates a forked history for her new contacts containing fake keys and keeps Alice on the original history. New contacts can detect this attack by obtaining the latest STR from a mutual contact with Alice (if they have one) or from a random contact if the MKS only gives the forked history to new contacts of Alice. Thus to have a chance of maintaining the attack, the MKS must give the forked history to all of Alice's contacts. 
This forked history allows Alice, her existing contacts, and potentially other clients to identify conflicting STRs since an exchange of conflicting STRs eventually occurs unless there is a complete partitioning of the network.

\subsubsection{Impersonation, client-targeted, existing connections} The MKS can impersonate all of Alice's existing contacts to Alice by giving Alice a history that includes her real key but fake keys for all of her contacts. This attack cannot be detected, because any time Alice asks for the latest STR a contact has seen, the MKS can intercept the request and falsify the response. Alternatively, the MKS can impersonate as Alice to her existing contacts by giving them a history that includes her fake key. This attack cannot be detected by Key Transparency alone because the MKS presents a consistent history to everyone except Alice, who can no longer communicate with anyone.
To defend against this attack, we use some Trust Network monitoring heuristics (\S\ref{sec:heuristics}).
When the MKS impersonates all of Alice's existing connections to Alice, mass key update monitoring prevents naive attacks and detects stealthy attacks. When the MKS impersonates Alice to all of her existing connections, isolation monitoring detects this attack.

% \dev{Dev:Presently, we are referring to monitoring heuristics of \S\ref{sec:heuristics}. Later in next section also we refer to heuristics of the same \S\ref{sec:heuristics}? Thus a question arises, why monitoring heuristics are part of TN, if all solutions require them in detection (or prevention) of some attacks. 
% }
% \ks{I think I noticed that and struck out that text now. Does my strikeout resolve your concern here?}

%Key transparency detects both MitM and impersonation attacks. If an MKS presents a fake key, it is detected at the next epoch through auditing or key monitoring. 
%There are two approaches to auditing. In a multi-provider scenario, the providers perform the auditing, whereas, in a single-provider scenario, the clients perform the auditing. When clients receive an STR from the key server, they request an STR from an auditor (i.e., a provider or another client) to compare with the STR they received. If there is ever a mismatch, then the server has equivocated by giving two entities inconsistent STRs for a given epoch.
%In a single-provider scenario, clients can monitor their own key to detect if a fake key ever appears in the transparency log. There is no evidence to convince third parties that the server has misbehaved, but clients can protect themselves by abandoning the service.

%All pair-targeted and client targeted attacks can be detected by auditing, assuming the key server equivocates to conduct these attacks.
%If an MKS launches a client-targeted impersonation attack on new and existing connections without equivocating by placing a fake key in the log for everyone to see, the client under attack can detect this at the next epoch. The client would have to alert the contacts of the attack out of band. This is not possible for new connections that were established after the attack commenced.



\subsection{AKM Security Analysis}

\ks{Do we need this detailed discussion about how each attack is thwarted? Move to an appendix? Perhaps these detailed descriptions of how individual attacks are handled should become the basis for comparing the defenses? This is what led to Table II after all.}

We now analyze how well Anonymous Key Retrieval protects users from fake key attacks, described in our threat model, using the basic and advanced defenses. We present the results of the security analysis in Table ~\ref{tab:compare}. For pair-targeted attacks, we assume the connection is between Alice and Bob. For client-targeted attacks, we assume the targeted user is Alice.

\tarun{IN PROGRESS: Basic AKM: The users monitor the new or updated key for n consecutive intervals regularly after key retrieval. To give a fake key to a user, the server has to distinguish the key verification request from monitoring request in all n intervals. The probability to successfully execute it is (0.5)n.}

\tarun{IN PROGRESS: Advanced AKM: The regular anonymous monitoring from the key owners prevents the server from presenting fake key for every key retrieval request for a user. The probability of distinguishing the key retrieval requests from monitoring requests is (probability of finding the intervals in which key retrieval query was made)x (probability of finding the key retrieval request within any one of the interval) = (n/I)0.5}

\subsubsection{MITM, pair-targeted} The basic defense detects this attack because both Alice and Bob monitor each other's key anonymously. The advanced defense prevents the attack against new connections because both Alice and Bob retrieve each other's keys anonymously. It's improbable for the MKS to successfully predict the time of a new communication as explained in ~\ref{subsec:AdvancedAKR}. The advanced defense prevents the attack on existing connections because Alice and Bob will first confirm key updates using an out-of-band third party channel.

\subsubsection{MITM, client-targeted} The basic defense detects this attack because Alice and her contacts monitor her key anonymously. The advanced defense prevents the attack against new connection because it's improbable for the MKS to successfully predict the time of a new communication as explained in ~\ref{subsec:AdvancedAKR}. The advanced defense prevents the attack on existing connections because Alice and her existing contacts will first confirm key updates using an out-of-band third party channel.


\subsubsection{Impersonation, pair-targeted} The basic defense detects impersonation attacks on new and existing connections because multiple monitors of a key will (eventually) detect any equivocation.
If the MKS impersonates as Alice to Bob or vice versa, the attack is detected because both of them will monitor the key of the target.
The advanced defense prevents the attack against new connections because the key server cannot reliably determine who is requesting Alice's key in order to impersonate as Alice or to Alice.
The advanced defense prevents the attack against existing connections because Alice (when the MKS impersonates to Alice) or Bob (when the MKS impersonates as Alice) first confirm the fake key update using an out-of-band third party channel.

\subsubsection{Impersonation, client-targeted, new connections} The basic defense detects attacks on new connections because multiple monitors of a key will (eventually) detect any equivocation.
If the MKS impersonates as Alice to new connections, Alice and all her new connections monitor her key. 
If the MKS impersonates to Alice for new connections, Alice and each new connection monitor the new connection's key.
The advanced defense prevents the attack against new connection because it's improbable for the MKS to successfully predict the time of a new communication as explained in ~\ref{subsec:AdvancedAKR}.

\subsubsection{Impersonation, client-targeted, existing connections} 
The basic defense detects attacks on existing connections because multiple monitors of a key will (eventually) detect any equivocation.
If the MKS impersonates as Alice to existing connections, Alice and all her new connections monitor her key. 
If the MKS impersonates to Alice for existing connections, Alice and each new connection Bob monitor Bob's key.
The advanced defense prevents the attack against existing connections because Alice (when the MKS impersonates to Alice) or Bob (when the MKS impersonates as Alice) can detect the fake key update using an out-of-band channel.


\subsubsection{All rapid attacks that end with the MKS restoring valid keys}
Key history monitoring from ~\ref{subsec:KeyHist} can detect these attacks.

% \dev{ToDo:  Simulation of X axis: Number of new friends (per day)  Y axis: Number of clients with new connections (per day). Simulate for say 1 year. Corresponding to each value on X axis we will have a box plot describing the max variation in MIs.}







% \subsection{TN Security Analysis}

% We now consider how the Trust Network defends against fake key attacks.
% For pair-targeted attacks, we assume a connection between Alice and Bob. For client-targeted attacks, we assume the targeted user is Alice.

% \subsubsection{MITM, pair-targeted}
% This attack, for both new and existing connections, can be prevented if Alice and Bob share a mutual contact.
% Alice's client will retrieve the correct key from her verification bundle database and compare it with one provided by the MKS. If the keys do not match, Alice's client will refrain from communicating with Bob, thus preventing the attack. In the absence of mutual contacts, Alice can detect the attack using a contact relay. Detection depends on Alice being able to retrieve the correct key for Bob from a relay. This in turn depends on the MKS being unable to detect that a relay is asking on behalf of Alice and then expanding its attack by also presenting a fake key to the relay. For new connections, the relay asks for Bob's key before Alice; the MKS would need to expand its attack to a client-targeted attack to avoid detection. For existing connections, using relays obscures both who is asking for Bob's key and who is sending Alice the key. This makes it difficult for the MKS to mount a timing attack so it can present a fake key to the relay. Again, the MKS would need to expand its attack to a client-targeted attack to avoid detection.


% %The attack on new connections can be prevented using pre-key retrieval, as Alice's client would first ask her contact Carol (using sealed sender) to retrieve Bob's keys on her behalf. MKS would provide correct keys to Carol, which would relay this correct key bundle to Alice, preventing the attack. But, for existing connections, this can be easily detected using post-key retrieval. Since the request is relayed through multiple hops (ref. Subsection \ref{subsec:MultipleRelays}) to avoid correlation based attacks, some extra delay would be incurred before obtaining the correct keys from some Signal user.
% %Meanwhile, she could continue her communication with Bob using the key obtained from the MKS without waiting for response from a Signal user. Once some Signal user responds, Alice can detect whether or not she was under attack.
% %Moreover, if the the additional delay is not a concern for Alice, she could wait for some Signal user to reply with the correct key, before communicating with Bob. This prevents such attacks.

% \subsubsection{MITM, client-targeted}
% For new connections this attack can be prevented if Alice and Bob share a mutual contact, as above. In the absence of a mutual contact, Alice can detect the attack using a contact relay.
% Since the attack is targeting Alice, any other contact of Alice, such as Carol, can retrieve Bob's true key from the MKS. It can be argued that the MKS could expand its attack and give every client a fake key for Bob. This results in a client-targeted impersonation attack on Bob; see below for how this defense rates.
% When the MKS uses a client-targeted/MITM attack on Alice’s existing connections, mass key update monitoring prevents naive attacks and detects stealthy attacks.


% %It can be argued tat if other Signal user would ask for Alice's key bundle. MKS can easily provide them all with fake key bundle and they would not be able to detect the fake keys. However, for a successful MITM, both communicating parties must get fake keys; in our case Alice would identify the fake keys apriori the communication, preventing such attacks..

% \subsubsection{Impersonation, pair-targeted}
% This scenario is similar to MITM pair targeted attacks; both for new and existing connections the attack can be prevented, and the same explanation applies.

% \subsubsection{Impersonation, client-targeted, new connections}
% If the MKS impersonates new connections to Alice, this is prevented using mutual contacts or detected using contact relays, similar to MITM client-targeted attacks on new connections. If the MKS impersonates as Alice to new connections, the attack is prevented if any of these clients has a mutual contact with Alice. The impersonation as Alice may also be detected with contact relays; this forces the MKS to provide the fake key for every request of Alice's key. Eventually this could mean that a mutual contact with Alice detects the attack.

% \subsubsection{Impersonation, client-targeted, existing connections}
% When the MKS impersonates all of Alice's existing connections to Alice,
% mass key update monitoring \emph{prevents} naive attacks and \emph{detects} stealthy attacks. When the MKS impersonates Alice to all of her existing connections, isolation monitoring \emph{detects} this attack.

% \subsubsection{All attacks that end with the MKS restoring valid keys}
% An MKS may be motivated to execute a short-lived attack to avoid detection, especially for client-targeted attacks.
% 	Key history monitoring detects short-lived attacks, as explained above.




% \subsection{Simulation}
% \label{simulation_setup}
% We cannot directly validate the effectiveness of the TN in practice, as there is no public sample dataset for the messaging networks and their traffic pattern. Instead, we analyze a Facebook's subnetwork~\cite{nr} of $\approx 1.3$ million users and perform simulations based on generalized but realistic assumptions on message patterns. We do not claim that the results from this simulation are exact value for the messaging networks. However, it gives a sense of feasibility and the parameters' values that could be used for the TN. 


% For our analysis, we considered users who had two or more friends (one of the assumption of TN), which was a total of 1,279,517 users. In our simulation 1) 1\% of the users updates keys per day, 2) 1\% of the users makes a new friend per day

% \subsection{Isolation monitoring}
% \label{appendix_isolation_monitoring}
% To make the isolation monitoring process efficient, the client divides an epoch into $x$ subintervals, where $x$ is the client's number of contacts. During each sub-interval, the client selects a random contact and sends them an isolation monitoring query. Upon receiving a response from a query sent during a previous sub-interval, the client considers itself as non-isolated, stops monitoring, and resumes monitoring at the next epoch. In case no response is received throughout all sub-intervals of an epoch, the client assumes it is isolated from its contacts by the server.

% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.48\textwidth]{images/percent_change.png}
% 	\caption{percentage of key change vs number of neighbors}
% 	\label{fig:percentKeyChange}
% \end{figure}

% Results[In progress]: 49\% of the new connections are prevented, 9.47\% threshold parameter for mass key monitoring.. 

% need to put threshold graph for mass key monitoring.




% \subsubsection{Limitations of Contact Relay approach}
% \label{contact_relay_attacks}
% \paragraph{Packets correlation at Network layer}
% \st{An MKS (acting as a global adversary) may try to correlate traffic patterns at the network layer based on IP addresses.For example, it is easy to identify Alice if she has a fixed IP address.
% Currently analysis based solely on IP addresses may lead to inaccurate inferences because many ISPs across the globe have deployed Carrier-grade NAT (CGN) devices~\cite{livadariu2018inferring, rytilahtiusing}.
% Ritchter et al.[] reported that CGN deployment is ubiquitous in cellular networks with more than $90\%$ of all cellular ASes deploying CGNs.
% Thus, in a well-established social network, many users are likely behind the same NAT device, making it hard for the MKS to identify Alice among other NAT clients accurately.
% However, deployment of IPv6 by mobile providers in the near future may make it easier for the MKS to correlate traffic pattern based on network layer. In that case, it would be easier for clients to communicate with each other directly for key verification as they would have unique IP addresses.}

% \paragraph{Timing Correlation on a (inactive/unbusy/dull?) network}
% \st{To prevent timing correlation on the verification requests, the client adds a random delay to obfuscate the verification request.
% The effectiveness of the delay depends on the number of messages flowing through the network. If the network traffic is high, even a small delay makes it harder for the MKS to identify the request accurately. But if the network traffic is too low, then a high delay would be needed to prevent the timing correlation. Morever, we couldn't find co-relation between the network traffic and the delay because of lack of data available for research.}



% The trust network detects a short duration attack by key history monitoring and detects a long duration attack by contact relay.




%% DZ: deleted below because I don't understand/agree with it. Alice CAN make connections -- they are impersonated by the MKS. Now, other users won't be able to make connetions to Alice, so maybe THEY will notice. This is true for ANY impersonation attack and all defenses.
%It must be noted that, if MKS launches this attack for prolong period of time, it would lead to detection by Alice. This is because, for the entire attack duration, Alice would not be able to create any E2EE connection with other Signal users (and vice-versa) raising suspicion. Moreover, this would lead to usability issues as Alice would isolated from all the upcoming connections. On the other hand, if the attack is for short duration, it can be detected with our Key monitoring heuristic (ref. Subsection \ref{subsec:KeyHist}).



%For existing connections, if MKS impersonates to Alice as each of her contact, it needs to send the fake key updates of all the clients. This can be detected using our additional heuristic mass key monitoring (ref. Subsection \ref{subsec:MassKeyUpdate}). However, if it impersonates as Alice to all her contacts, MKS would provide fake key of Alice to all, disconnecting Alice from her contacts. This attack can be detected using isolation monitoring heuristic (ref. Subsection \ref{subsec:Isolation}).

% The TN prevents all pair-targeted attacks (Rows 1, 2, 5, 6) and client-targeted attacks for new connections (Rows 3 and 7) when Alice has a mutual contact with Bob that has previously sent her his correct keys.

% If Alice does not share a mutual contact with Bob, using contact as a relay she can request one of her contacts Carol (as a first point of contact) to obtain Bob's key from the MKS. Based on RealyCount parameter

% If Connor queries the MKS for Bob's key immediately after Alice asks him, the MKS might suspect that Connor is asking for Bob's key on behalf of Alice by correlating Connor's request with Alice's message to Connor. To prevent the correlation, Connor can pause for a random period of time before querying the MKS for Bob's key.
% Contact as a relay could incur delay.
% Thus, Alice has two options --- (1) if she opts for \textit{prevention}, she must wait for some Signal user to reply with the correct key, or (2) she can opt for \textit{detection} and continue her communication with Bob using the key obtained from the MKS without waiting for response from a Signal user. Once some Signal user responds, Alice can detect whether or not she was under attack.

% \ks{The server gives any of Alice's contacts Bob's fake key under the assumption that this is a key request since the contact has not communicated with Bob in the past. I don't think this is an effective defense even with the delayed request.}

% Suppose an MKS launches a client-targeted MitM attack against all of Alice's existing connections (Row 4).
% If Alice receives all the key updates for her contacts within a very short duration of time, she may have no contact remaining to act as a relay to query the key server.
% The heuristic for mass key update monitoring detects this attack (see \ref{subsec:heuristics}).


% \ks {What happens when a legitimate key change occurs, and how do we avoid false positives? Suppose Alice receives a key update for Bob, has a prior key from a mutual contact that is old. Does she first confirm the key change with the other contact? A valid key change will be sent to all the mutual contacts, but when do we assume we can learn about it? What if that single mutual contact is offline?}


==> Simulation.tex <==

\subsection{Simulation} 
% \ahc{this subsection seems way too early; I think all simulations etc. should appear separately later. But if you guys prefer to evaluate separately here the justification for this basic mechanisms, at least clarify that's all we do here. }
\subsubsection{Assumptions:}
There are no public datasets that accurately reflect the size, connectivity, and communication patterns of existing secure messaging systems. To validate the effectiveness of our proposed defenses, we conduct simulations based on a Facebook sub-network of $\approx 1.3$ million users~\cite{nr}. Even though the results are based on assumptions about existing networks instead of real-world data, the results provide an initial comparison of the effectiveness and performance of the defenses. The simulations also provide a way to understand the impact of different parameter choices for some of the defenses.

The simulations are based on the following assumptions. We considered only those users in the dataset that have two or more friends, a total of 1,279,517 users in the network. We simulate each defense to analyze its security and performance using the following parameters inspired from the assumptions in CONIKS \cite{melara2015coniks}:

\begin{itemize}
\item Up to 1\% of the clients 
\begin{itemize}
    \item Change or add keys per day.
    \item Make a new friend per day.
    \item Disconnect per day for a certain period. We use disconnection time distribution from ~\cite{bradthesis} to assign a disconnection period for each client in the disconnected population.  
\end{itemize}
% \item Up to 1\% of the clients 
% \item Up to 1\% of the clients 
% \item Monitoring occurs once per hour. \ks{Does this apply for each defense? Does monitoring mean anything to the reader at this point?}
\item Clients have an average of 100 connections.
%\item A 128-bit cryptographic security level (SHA-256, 512-bit EC-Schnorr signatures).
\end{itemize}
We present a feasibility and security analysis for each defense based on the simulations in the relevant sections of the paper. The performance analysis of the simulation data is summarized in Table ~\ref{tab:performance}.
\vspace{2mm}

\subsubsection{Mass key update monitoring analysis:}
Based on our network simulation, Fig.~\ref{fig:percentKeyChange} presents the percentage of a client's contacts ($max$, $mean$, and $median$) that update their key per day depending on the total number of contacts. The maximum percentage can guide the determination of a threshold value dynamically based on the total number of contacts. If a client observes a higher percentage of contacts' key updates than the threshold, it assumes an attack is in progress. \dev{Graph needs a little more elaboration, it could be confusing. Can we give one example of what could be the threshold based on our simulation?}
Future research is needed to determine how well these threshold values hold in different messaging networks.
\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{images/percent_change.png}
	\caption{The percentage of contacts ($max$, $mean$, and $median$) that update their key per day based on the total number of contacts for a client, where \textit{max} is the highest percentage of contacts with a key update across all clients with a given number of contacts.\tarun{Remove mean, median and vary epochs duration.}}
	\label{fig:percentKeyChange}
\end{figure}

\subsubsection{Isolation monitoring analysis:}
To analyze this heuristic, we utilized a recent study of $440$ different Android devices, with an average of 1.6 years of data for each device \cite{bradthesis}. The study reports that the probability that a disconnected interval ($DI_{time}$) for a device lasts for \textit{less than} one minute is $0.68$, less than one hour is $0.96$, and less than one day is $0.998$.  

Suppose the time period for isolation monitoring is $t$. In that case, the probability that a single contact might not respond is $1-DI_{t}$, and the probability that  $n$ contacts might not respond is $(1-DI_{t})\textsuperscript{n}$.
For example, assuming the time period for isolation monitoring is 1 hour, and Alice sends a verification message to 3 of her friends every interval, the probability that none of the contacts reply to Alice during that interval is $(1-0.96)\textsuperscript{3} = 0.00006$. 
As more contacts are added, the probability approaches zero.
%If no response arrives at Alice from any of her contacts during a monitoring period, it is considered an attack. But, this might happen due to some network connectivity issues, and our approach would incorrectly classify this as attack. 
%However, the probability of falsely determining isolation monitoring as an attack is negligible. Even with only two contacts selected for verifying isolation, the attack can be detected in an hour with probability $0.9984$.

Fig.~\ref{fig:isolationMonitoringFig} shows that with an increase in monitoring interval's duration or the number of contacts, the probability of a false positive decreases. However, even for two contacts with a monitoring interval of 10 minutes, the likelihood of a false-positive is 0.0052. The false positive rate decreases exponentially with an increase in the number of contacts or duration of the monitoring interval. In our simulation, a client makes an average of only $1.01$ isolation verification requests per monitoring interval.
\dev{How the graph has been created? I guess some intuition of the process would also suffice.}

\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{images/isolation_monitoring.png}
	\caption{Probability of falsely classifying disconnection of all contacts as an attack based on number of contacts of a client. Different lines represents different monitoring intervals (in mins).
	\ahc{I think the x-axis should be the monitoring-intervals, not # of friends, just show three or four lines for numbers of friends, and base this on some data on typical numbers of friends (so have one very low and two-three more typical numbers of friends). Also: use also different lines, not just colors, some people are color blind and some use black-and-white printouts. }
	}
	\label{fig:isolationMonitoringFig}
\end{figure}

==> Table.tex <==
\newcommand*{\tilt}[1]{\adjustbox{angle=90,lap=\width-0.5em}{\em #1}}
\newcommand*{\prevents}{{\tiny \CIRCLE}}
\newcommand*{\detects}{{\tiny \Circle}}
\newcommand*{\preventsAKR}{{\tiny \CIRCLE^{*}$}}
\newcommand*{\preventsTor}{{\tiny \CIRCLE^{+}$}}
\newcommand*{\preventsTorHistory}{{\tiny \CIRCLE^{a}$}}
\newcommand{\no}{}
\newcommand{\partiald}{{\tiny \Leftcircle}}
\newcommand{\partialNotNew}{{\tiny \Rightcircle}}
\newcommand{\partialp}{{\tiny \LEFTcircle}}

\begin{table*}
  \centering
  \caption{Taxonomy of fake key attacks and analysis of defenses}
  \label{tab:compare}
  \begin{tabular}{l|cccc|cccc|}
    & \multicolumn{4}{c|}{MITM} & \multicolumn{4}{c|}{Impersonation} \\
    & \multicolumn{2}{c}{Pair Targeted} & \multicolumn{2}{c|}{Client Targeted} & \multicolumn{2}{c}{Pair Targeted} & \multicolumn{2}{c|}{Client Targeted} \\
    \textit{Defense}  & New & Existing & New & Existing & New & Existing & New & Existing\\
    \midrule
    Key Transparency (multiple-provider) & \detects & \detects & \detects & \detects & \detects & \detects & \detects & \detects \\
    Key Transparency (single-provider) & \detects & \detects & \detects & \no & \detects & \detects & \detects & \no \\
    Trust Network (mutual contact) & \prevents & \prevents & \prevents &  & \prevents &
                                                                            \prevents & \prevents &  \\
    Trust Network (contact relay) & \detects & \detects & \detects &  & \detects &
                                                                            \detects & \partiald &  \\
    Anonymous Key Retrieval (basic) & \detects & \detects & \detects & \detects & \detects & \detects & \detects & \detects\\
    Anonymous Key Retrieval (advanced) & \prevents & \prevents & \prevents & \prevents & \prevents & \prevents & \partialp & \prevents\\
    Mass key update monitoring (naive) &&&& \prevents &&&& \prevents\\
    Mass key update monitoring (stealthy) &&&& \detects &&&& \detects$^\dag$\\
    Isolation monitoring &&&& &&&& \detects$^\ddag$ \\
    Key history monitoring & \partiald & \partiald & \partiald & \partiald & \partiald & \partiald & \partiald & \partiald\\
    \end{tabular}
    \vspace{3mm}\\
    \prevents~prevents the attack, \detects~detects the attack, \partialp~sometimes prevents the attack, \partiald~sometimes detects the attack, (blank) susceptible\\
 %   $*$ anonymous key retrieval, $+$ Tor hidden service \\
    $\dag$ impersonating to Alice, $\ddag$ impersonating as Alice\\
\end{table*}

==> Table_2.tex <==
\newcommand*{\tilt}[1]{\adjustbox{angle=90,lap=\width-0.5em}{\em #1}}
\newcommand*{\prevents}{{\tiny \CIRCLE}}
\newcommand*{\detects}{{\tiny \Circle}}
\newcommand*{\preventsAKR}{{\tiny \CIRCLE^{*}$}}
\newcommand*{\preventsTor}{{\tiny \CIRCLE^{+}$}}
\newcommand*{\preventsTorHistory}{{\tiny \CIRCLE^{a}$}}
\newcommand{\no}{}
\newcommand{\partiald}{{\tiny \Leftcircle}}
\newcommand{\partialdright}{{\tiny \Rightcircle}}
\newcommand{\partialponly}{{\tiny \LEFTCIRCLE}}
\newcommand{\partialNotNew}{{\tiny \Rightcircle}}
\newcommand{\partialp}{{\tiny \LEFTcircle}}
\newcommand{\shortlived}{{ \Square}}



\begin{table*}
	\centering
	\caption{Taxonomy of fake key attacks and analysis of defenses}
	\label{tab:compare}
	\begin{center}
		\begin{tabular}{l|cccc|cccc|cc}
			                                     & \multicolumn{4}{c|}{MITM}          & \multicolumn{4}{c|}{Impersonation}                                                                                                                              \\
			% & \multicolumn{2}{c|}{Resources} \\
			                                     & \multicolumn{2}{c}{Pair-Targeted } & \multicolumn{2}{c|}{Client-Targeted} & \multicolumn{2}{c}{Pair-Targeted} & \multicolumn{2}{c|}{Client-Targeted}                                                 \\
			\textit{Defense}                     & New                                & Existing                             & New                               & Existing                             & New       & Existing  & New       & Existing  \\
			\midrule
			
% 			Key Transparency (multiple-provider) & \detects                           & \detects                             & \detects                          & \partialp                            & \detects  & \detects  & \detects  & \partialp \\
% 			Key Transparency (single-provider)   & \detects                           & \detects                             & \detects                          & \partialp                            & \detects  & \detects  & \detects  & \partialp \\
			
			Key Transparency   & \detects                           & \detects                             & \detects                          &                             & \detects  & \detects  & \detects  &  \\
			
			Anonymous Key Monitoring (basic)      & \detects                           & \detects                             & \detects                          & \detects                            & \detects  & \detects  & \detects  & \detects \\
			Anonymous Key Monitoring (advanced)   & \prevents                          & \prevents                            & \prevents                         & \prevents                            & \prevents & \prevents & \partialp & \prevents \\
			
			
% 			Trust Network                        & \prevents                          & \partialp                            & \prevents                         & \partialp                            & \prevents & \partialp & \partialp & \partialp \\
			
			Trust Network                      & \prevents                          & \partialp                            & \partialp                &                             & \prevents & \partialp & \partialp &  \\
			
			Mass key update monitoring                      &                           &                             &                          & \detects                            &  &  &  & \partiald \\
			Isolation monitoring         & & & & & & & & \partialdright \\

			Short-lived attack monitoring       &
			\shortlived &              \shortlived &              \shortlived &      			\shortlived &              \shortlived &              \shortlived &      			\shortlived &               \shortlived \\
		\end{tabular}
	\end{center}
	\vspace{3mm}
	\prevents~prevents the attack~~ \detects~detects the attack~~  \partialp~sometimes prevents the attack~~ \shortlived~detects short-lived attack~~ \\
\end{table*}


==> Table_3.tex <==
\begin{table*}
	\centering
	\caption{Performance analysis}
	\label{tab:performance}
	\begin{tabular}{l|c|c|c|c|c}
		                                     &  & \multicolumn{4}{c}{Resources}                                                                    \\
		% & \multicolumn{2}{c|}{Resources} \\
		% & \multicolumn{2}{c}{Pair Targeted } & \multicolumn{2}{c|}{Client Targeted} & \multicolumn{2}{c}{Pair Targeted} & \multicolumn{2}{c|}{Client Targeted} \\
		\textit{Defense}                     & Detection/Waiting time \textsuperscript{\textdagger}   $^\ddagger$        & Client side memory & \multicolumn{3}{c}{Network Traffic (per client)}                        \\
		                                     &                            &                               & (per epoch)                 & (per new connection) & (per key update) \\
		\midrule

% 		Key Transparency (multiple-provider) & $0$                            & $104 B$                       & $20.1 KB$                                 & $1.216 KB$           \\
		

    	KT- detection  & $2\cdot(diam(G) +1)\cdot\delta$ (<1 epoch)                           & $104 B$                       & $7.136 KB$                                & $1.056 KB$     & $1.056 KB$      \\
    	
    	KT- prevention  & $2\cdot(diam(G) +1)\cdot\delta$, $2\cdot\delta$                            & $4.9 KB$                       & $29.04 KB$                                & $1.216 KB$ & $40 KB^{*}$           \\


		AKM-detection      & $m$ epochs ($\approx10^{**}$)                            & $0$                           & $~32 KB$                                 & $~320 KB$  & $~320 KB$            \\
		AKM-prevention   & $m$ epochs, $2\cdot\delta$                    & $4.8 KB$                      & $~32 KB$                                 & $~320 KB$ & $40 KB^{*}$           \\

		
		KTAM-detection                        & $\Delta$ (<1 epoch)                       & $104 B$                     & $33.96 KB$                                 & $1.06 KB$ & $1.06 KB$            \\
		
		KTAM-prevention                      & $\Delta$, $2\cdot\delta$ & $4.9 KB$                     & $33.96 KB$                                 & $1.06 KB$    & $40 KB^{*}$        \\
		



	\end{tabular}
	
	
	
	\vspace{3mm}
    $\ddagger$~ = the delay is after the beginning of the next epoch in which the contact starts communication.\\
    \textdagger~= Detection time is for detection mode, and waiting time is for prevention mode. The waiting time in prevention mode is presented as <new connections, existing connections>.\\
	*~ = Using TOR service as the out-of-band channel, the actual data exchanged is 64 bytes.~~~~~~~
	**~= detects with $0.999$ probability.\\
    


% 	\detects~detects the attack, \partialp~sometimes prevents the attack \\
\end{table*}


==> detailed_analysis.tex <==
\section{Security proofs}
\label{section:detailed_analysis}


% \subsection{KTCA}



% \subsection{AKM}




% \subsection{KTACA}





% \subsection{Short-lived attack monitoring}

